Planetary Candidates Observed by Kepler. VIII. A Fully Automated Catalog With Measured Completeness and Reliability Based on Data Release 25

We present the Kepler Object of Interest (KOI) catalog of transiting exoplanets based on searching four years of Kepler time series photometry (Data Release 25, Q1-Q17). The catalog contains 8054 KOIs of which 4034 are planet candidates with periods between 0.25 and 632 days. Of these candidates, 219 are new and include two in multi-planet systems (KOI-82.06 and KOI-2926.05), and ten high-reliability, terrestrial-size, habitable zone candidates. This catalog was created using a tool called the Robovetter which automatically vets the DR25 Threshold Crossing Events (TCEs, Twicken et al. 2016). The Robovetter also vetted simulated data sets and measured how well it was able to separate TCEs caused by noise from those caused by low signal-to-noise transits. We discusses the Robovetter and the metrics it uses to sort TCEs. For orbital periods less than 100 days the Robovetter completeness (the fraction of simulated transits that are determined to be planet candidates) across all observed stars is greater than 85%. For the same period range, the catalog reliability (the fraction of candidates that are not due to instrumental or stellar noise) is greater than 98%. However, for low signal-to-noise candidates between 200 and 500 days around FGK dwarf stars, the Robovetter is 76.7% complete and the catalog is 50.5% reliable. The KOI catalog, the transit fits and all of the simulated data used to characterize this catalog are available at the NASA Exoplanet Archive.

==> RV-minorFlags.tex <==
\section{Robovetter Mnemonic Flags}
\label{minorflagsec}
\red{This needs to be updated with DR25 mnemonic flags.}
In Table~\ref{robodispstab} we list mnemonic flags that describe the results of individual robovetter tests in the comments column. Here we describe the meaning of each flag.

\begin{itemize}
\item[] \textbf{ALT\_ROBO\_ODD\_EVEN\_TEST\_FAIL}: The TCE failed the robovetter's odd-even depth test on the alternate detrending, and thus is marked as a FP due to a significant secondary.
\item[] \textbf{ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET}: A significant secondary eclipse was detected in the alternate detrending, but it was determined to possibly be due to planetary reflection and/or thermal emission. While the significant secondary major flag remains set, the TCE is dispositioned as a PC.
\item[] \textbf{ALT\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD}: A significant secondary eclipse was detected in the alternate detrending, but it was determined to be the same depth as the primary within the uncertainties. Thus, the TCE is possibly a PC that was detected at twice the true orbital period. When this flag is set, it acts as an override to other flags such that the significant secondary major flag is not set, and thus the TCE is dispositioned as a PC if no other major flags are set.
\item[] \textbf{ALT\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW}: The difference of the primary and positive event significances, computed by the model-shift test using the alternate detrending, is below the threshold $\sigma'_{\rm FA}$. This indicates the primary event is not unique in the phased light curve, and thus the TCE is dispositioned as a FP with the not transit-like major flag set.
\item[] \textbf{ALT\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW}: The difference of the primary and tertiary event significances, computed by the model-shift test using the alternate detrending, is below the threshold $\sigma'_{\rm FA}$. This indicates the primary event is not unique in the phased light curve, and thus the TCE is dispositioned as a FP with the not transit-like major flag set.
\item[] \textbf{ALT\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW}: The significance of the primary event divided by the ratio of red noise to white noise in the light curve, computed by the model-shift test using the alternate detrending, is below the threshold $\sigma_{\rm FA}$. This indicates the primary event is not significant compared to the amount of systematic noise in the light curve, and thus the TCE is dispositioned as a FP with the not transit-like major flag set.
\item[] \textbf{CENTROID\_SIGNIF\_UNCERTAIN}: The significance of the centroid offset cannot be measured to high enough precision, and thus the centroid module can not confidently disposition the TCE as a FP. This is typically due to having only a very small number (3 or 4) of offset measurements, all with low SNR.
\item[] \textbf{CLEAR\_APO}: The TCE was marked as a FP due to a centroid offset because the transit occurs on a star that is spatially resolved from the target.
\item[] \textbf{CROWDED\_DIFF}: More than one potential stellar image was found in the difference image. The EYEBALL flag is always set when the CROWDED\_DIFF flag is set.
\item[] \textbf{DV\_ROBO\_ODD\_EVEN\_TEST\_FAIL}: The TCE failed the robovetter's odd-even depth test on the DV detrending, and thus is marked as a FP due to a significant secondary.
\item[] \textbf{DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET}: A significant secondary eclipse was detected in the DV detrending, but it was determined to possibly be due to planetary reflection and/or thermal emission. While the significant secondary major flag remains set, the TCE is dispositioned as a PC.  
\item[] \textbf{DV\_SEC\_SAME\_DEPTH\_AS\_PRI\_COULD\_BE\_TWICE\_TRUE\_PERIOD}: A significant secondary eclipse was detected in the DV detrending, but it was determined to be the same depth as the primary within the uncertainties. Thus, the TCE is possibly a PC that was detected at twice the true orbital period. When this flag is set, it acts as an override to other flags such that the significant secondary major flag is not set, and thus the TCE is dispositioned as a PC if no other major flags are set.
\item[] \textbf{DV\_SIG\_PRI\_MINUS\_SIG\_POS\_TOO\_LOW}: The difference of the primary and positive event significances, computed by the model-shift test using the DV detrending, is below the threshold $\sigma'_{\rm FA}$. This indicates the primary event is not unique in the phased light curve, and thus the TCE is dispositioned as a FP with the not transit-like major flag set.
\item[] \textbf{DV\_SIG\_PRI\_MINUS\_SIG\_TER\_TOO\_LOW}: The difference of the primary and tertiary event significances, computed by the model-shift test using the DV detrending, is below the threshold $\sigma'_{\rm FA}$. This indicates the primary event is not unique in the phased light curve, and thus the TCE is dispositioned as a FP with the not transit-like major flag set.  
\item[] \textbf{DV\_SIG\_PRI\_OVER\_FRED\_TOO\_LOW}: The significance of the primary event divided by the ratio of red noise to white noise in the light curve, computed by the model-shift test using the DV detrending, is below the threshold $\sigma_{\rm FA}$. This indicates the primary event is not significant compared to the amount of systematic noise in the light curve, and thus the TCE is dispositioned as a FP with the not transit-like major flag set.  
\item[] \textbf{EYEBALL}: The metrics used by the centroid module are very close to the decision boundaries, and thus the centroid disposition of this TCE is uncertain and warrants further scrutiny. No TCEs are marked as a FP due to a centroid offset if this flag is set.
\item[] \textbf{FIT\_FAILED}: The transit was not fit by a model in DV and thus no difference images were created for use by the centroid module. Thus, the TCE is not failed due to a centroid offset by default. This flag is typically set for very deep transits due to eclipsing binaries.
\item[] \textbf{INVERT\_DIFF}: One or more difference images were inverted, meaning the difference image claims the star got brighter during transit. This is usually due to variability of the target star and suggests the difference image should not be trusted. When this flag is set, the TCE is marked as a candidate that requires further scrutiny, i.e., the EYEBALL flag is set and the TCE is not marked as a FP due to a centroid offset.
\item[] \textbf{KIC\_OFFSET}: The centroid module measured the offset distance relative to the star's recorded position in the Kepler Input Catalog (KIC), not the out of transit centroid. The KIC position is less accurate in sparse fields, but more accurate in crowded fields. If this is the only flag set, there is no reason to believe a statistically significant centroid shift is present \citep{Mullally2015c}.
\item[] \textbf{LPP\_ALT\_TOO\_HIGH}: The LPP value \citep{Thompson2015b}, as computed using the alternate detrending, is above the robovetter threshold. This indicates the TCE is not transit-shaped, and thus is dispositioned as a FP with the not transit-like major flag set.
\item[] \textbf{LPP\_DV\_TOO\_HIGH}: The LPP value, as computed using the DV detrending, is above the robovetter threshold. This indicates the TCE is not transit-shaped, and thus is dispositioned as a FP with the not transit-like major flag set.  
\item[] \textbf{MARSHALL\_FAIL}: The TCE failed the Marshall metric \citep{Mullally2015b}, which indicates that the TCE's individual transits are not transit-shaped and more likely due to instrumental artifacts. Thus, the TCE is dispositioned as a FP with the not transit-like major flag set.
\item[] \textbf{OTHER\_TCE\_AT\_SAME\_PERIOD\_DIFF\_EPOCH}: Another TCE on the same target with a higher planet number was found to have the same period as the current TCE, but a significantly different epoch. This indicates the current TCE is an eclipsing binary with the other TCE representing the secondary eclipse. If the ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET and DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET flags are not set, the TCE is dispositioned as a FP with the significant secondary major flag set.
\item[] \textbf{PARENT\_IS\_X}: The TCE has been identified as a FP due to an ephemeris match. This flag indicates the most likely parent, or true physical source of the signal, where X will be substituted for the parent's name. Note that X is not guaranteed to be the true parent, but simply is the most likely source given the information available.
\item[] \textbf{PERIOD\_ALIAS\_IN\_ALT\_DATA\_SEEN\_AT\_X:1}: Using the results of the model-shift test (specifically the phases of the primary, secondary, and tertiary events) a possible period alias is seen at X:1, where X is an integer. This indicates the TCE has likely been detected at a period that is X times longer than the true orbital period. This flag is currently informational only and not used to declare any TCE a FP.
\item[] \textbf{RESID\_OF\_PREV\_TCE}: The TCE has the same period and epoch as a previous transit-like TCE. This indicates the current TCE is simply a residual artifact of the previous TCE after it was removed from the light curve. Thus, the current TCE is dispositioned as a FP with the not transit-like major flag set.
\item[] \textbf{SAME\_P\_AS\_PREV\_NTL\_TCE}: The current TCE has the same period as a previous TCE that was dispositioned as FP with the not transit-like major flag set. This indicates that the current TCE is due to the same not transit-like signal. Thus, the current TCE is dispositioned as a FP with the not transit-like major flag set.
\item[] \textbf{SATURATED}: The star is saturated. The assumptions employed by the centroid robovetter module break down for saturated stars, so the TCE is marked as a candidate requiring further scrutiny, i.e., the EYEBALL flag is set and the TCE is not marked as a FP due to a centroid offset.
\item[] \textbf{SEASONAL\_DEPTH\_DIFFS\_IN\_ALT}: There appears to be a significant difference in the computed TCE depth when using the alternate detrending light curves from different seasons. This indicates significant light contamination is present, usually due to a bright star at the edge of the image, which may or may not be the source of the signal. As it is impossible to determine whether or not the TCE is on-target from this flag alone, it is currently informational only and not used to declare any TCE a FP.
\item[] \textbf{SEASONAL\_DEPTH\_DIFFS\_IN\_DV}: There appears to be a significant difference in the computed TCE depth when using the DV detrending light curves from different seasons. This indicates significant light contamination is present, usually due to a bright star at the edge of the image, which may or may not be the source of the signal. As it is impossible to determine whether or not the TCE is on-target from this flag alone, it is currently informational only and not used to declare any TCE a FP.  
\item[] \textbf{SIG\_SEC\_IN\_ALT\_MODEL\_SHIFT}: The significance of the secondary event divided by the ratio of red noise to white noise in the light curve, computed by the model-shift test using the alternate detrending, is above the threshold $\sigma_{\rm FA}$. Also, the difference between the secondary and tertiary event significances, and the difference between the secondary and positive event significances, both computed by the model-shift test using the alternate detrending, is above the threshold $\sigma'_{\rm FA}$. This indicates that there is a unique and significant secondary event in the light curve, i.e., a secondary eclipse. Thus, assuming the ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET flag is not set, the TCE is dispositioned as a FP with the significant secondary flag set.
\item[] \textbf{SIG\_SEC\_IN\_DV\_MODEL\_SHIFT}: The significance of the secondary event divided by the ratio of red noise to white noise in the light curve, computed by the model-shift test using the DV detrending, is above the threshold $\sigma_{\rm FA}$. Also, the difference between the secondary and tertiary event significances, and the difference between the secondary and positive event significances, both computed by the model-shift test using the DV detrending, is above the threshold $\sigma'_{\rm FA}$. This indicates that there is a unique and significant secondary event in the light curve, i.e., a secondary eclipse. Thus, assuming the DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET flag is not set, the TCE is dispositioned as a FP with the significant secondary flag set.
\item[] \textbf{SIGNIF\_OFFSET}: There is a statistically significant shift in the centroid during transit. This indicates the variability is not due to the target star. Thus, the TCE is dispositioned as a FP with the centroid offset major flag set.
\item[] \textbf{THIS\_TCE\_IS\_A\_SEC}: The TCE is determined to have the same period, but different epoch, as a previous transit-like TCE. This indicates that the current TCE corresponds to the secondary eclipse of an eclipsing binary (or planet if the ALT\_SEC\_COULD\_BE\_DUE\_TO\_PLANET or DV\_SEC\_COULD\_BE\_DUE\_TO\_PLANET flags are set.) Thus, the current TCE is dispositioned as a FP with both the not transit-like and significant secondary major flags set.
\item[] \textbf{TOO\_FEW\_CENTROIDS}: The PRF centroid fit used by the centroid module does not always converge, even in high SNR difference images. This flag is set if centroid offsets are recorded for fewer than 3 high SNR difference images.
\item[] \textbf{TOO\_FEW\_QUARTERS}: Fewer than 3 difference images of sufficiently high SNR are available, and thus very few tests in the centroid module are applicable to the TCE. If this flag is set in conjunction with the CLEAR\_APO flag, the source of the transit may be on a star clearly resolved from the target.
\item[] \textbf{TRANSITS\_NOT\_CONSISTENT}: The TCE had a max\_ses\_in\_mes / mes ratio of greater than 0.9, and a period greater than 90 days. This indicates that the TCE is dominated by a single large event, and thus is due to a systematic feature such as a sudden pixel sensitivity dropout. Thus, the TCE is dispositioned as a FP with the not transit-like major flag set.
\end{itemize}


==> Table-hz2.tex <==
\clearpage
\LongTables
\begin{deluxetable*}{rrrrrlr|lrrlr}
\tablecolumns{12}
\tabletypesize{\scriptsize}
\tablewidth{\linewidth}
\tablecaption{Habitable Zone Planet Candidates}
\tablehead{
\colhead{} & \colhead{} & \colhead{} & \multicolumn{4}{c}{CatalogValues} & \colhead{} & \multicolumn{4}{c}{Confirmed Values} \\ 
\\ 
\colhead{KOI} &
\colhead{SNR} &
\colhead{Score} &
\colhead{\rp} &
\colhead{$F_{\rm p}$} &
\colhead{\tstar} &
\colhead{\rstar} &
\colhead{Confirmed} &
\colhead{\rp} &
\colhead{$S_{\rm p}$} &
\colhead{\tstar} &
\colhead{\rstar} \\ 
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{[\re]} &
\colhead{[$S_{\rm \oplus}$]} &
\colhead{[K]} &
\colhead{[\rsun]} &
\colhead{Name} &
\colhead{[\re]} &
\colhead{[$S_{\rm \oplus}$]} &
\colhead{[K]} &
\colhead{[\rsun]} 
}
\startdata
172.02 & 18.0 & 0.7 & 1.7$^{+0.21}_{-0.22}$ & 1.6$^{+0.59}_{-0.45}$ & 5637$^{+113}_{-101}$ & 0.9$^{+0.1}_{-0.1}$ & Kepler-69 c & 1.7$^{+0.33}_{-0.23}$ & 1.9$^{+0.81}_{-0.57}$ & 5638$^{+168}_{-168}$ & 0.9$^{+0.2}_{-0.1}$  \\ 
238.03 & 11.9 & 0.8 & 2.0$^{+0.33}_{-0.29}$ & 1.8$^{+0.87}_{-0.60}$ & 6086$^{+133}_{-133}$ & 1.2$^{+0.2}_{-0.2}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
438.02 & 30.6 & 1.0 & 1.9$^{+0.11}_{-0.12}$ & 1.3$^{+0.26}_{-0.25}$ & 3984$^{+71}_{-86}$ & 0.5$^{+0.0}_{-0.0}$ & Kepler-155 c & 1.9$^{+0.11}_{-0.12}$ & 1.3$^{+0.26}_{-0.25}$ & 3984$^{+71}_{-86}$ & 0.5$^{+0.0}_{-0.0}$  \\ 
463.01 & 78.0 & 0.0 & 1.6$^{+0.32}_{-0.29}$ & 1.2$^{+0.72}_{-0.47}$ & 3395$^{+74}_{-67}$ & 0.3$^{+0.1}_{-0.1}$ & Kepler-560 b & 1.6$^{+0.32}_{-0.29}$ & 1.2$^{+0.72}_{-0.47}$ & 3395$^{+74}_{-67}$ & 0.3$^{+0.1}_{-0.1}$  \\ 
494.01 & 35.9 & 1.0 & 1.7$^{+0.21}_{-0.33}$ & 2.3$^{+1.17}_{-1.10}$ & 3787$^{+163}_{-204}$ & 0.5$^{+0.1}_{-0.1}$ & Kepler-577 b & 1.7$^{+0.21}_{-0.33}$ & 2.3$^{+1.17}_{-1.10}$ & 3787$^{+163}_{-204}$ & 0.5$^{+0.1}_{-0.1}$  \\ 
571.05 & 7.7 & 0.7 & 1.2$^{+0.11}_{-0.14}$ & 0.2$^{+0.07}_{-0.06}$ & 3751$^{+75}_{-84}$ & 0.4$^{+0.0}_{-0.1}$ & Kepler-186 f & 1.1$^{+0.08}_{-0.08}$ & 0.3$^{+0.06}_{-0.04}$ & 3755$^{+90}_{-90}$ & 0.5$^{+0.0}_{-0.0}$  \\ 
701.03 & 35.9 & 1.0 & 1.7$^{+0.10}_{-0.07}$ & 1.2$^{+0.27}_{-0.19}$ & 4926$^{+98}_{-98}$ & 0.7$^{+0.0}_{-0.0}$ & Kepler-62 e & 1.6$^{+0.04}_{-0.04}$ & 1.2$^{+0.10}_{-0.10}$ & 4925$^{+70}_{-70}$ & 0.6$^{+0.0}_{-0.0}$  \\ 
812.03 & 18.0 & 1.0 & 1.8$^{+0.12}_{-0.15}$ & 1.3$^{+0.29}_{-0.30}$ & 3950$^{+70}_{-86}$ & 0.5$^{+0.0}_{-0.0}$ & Kepler-235 e & 1.8$^{+0.12}_{-0.15}$ & 1.3$^{+0.29}_{-0.30}$ & 3950$^{+70}_{-86}$ & 0.5$^{+0.0}_{-0.0}$  \\ 
854.01 & 19.3 & 1.0 & 1.9$^{+0.12}_{-0.22}$ & 0.7$^{+0.15}_{-0.19}$ & 3593$^{+71}_{-86}$ & 0.5$^{+0.0}_{-0.1}$ & Kepler-705 b & 1.9$^{+0.12}_{-0.22}$ & 0.7$^{+0.15}_{-0.19}$ & 3593$^{+71}_{-86}$ & 0.5$^{+0.0}_{-0.1}$  \\ 
947.01 & 45.7 & 1.0 & 1.8$^{+0.16}_{-0.21}$ & 1.9$^{+0.52}_{-0.53}$ & 3755$^{+75}_{-84}$ & 0.5$^{+0.0}_{-0.1}$ & Kepler-737 b & 1.8$^{+0.16}_{-0.21}$ & 1.9$^{+0.52}_{-0.53}$ & 3755$^{+75}_{-84}$ & 0.5$^{+0.0}_{-0.1}$  \\ 
1078.03 & 22.2 & 1.0 & 1.9$^{+0.14}_{-0.22}$ & 1.9$^{+0.49}_{-0.55}$ & 3789$^{+75}_{-82}$ & 0.5$^{+0.0}_{-0.1}$ & Kepler-267 d & 1.9$^{+0.14}_{-0.22}$ & 1.9$^{+0.49}_{-0.55}$ & 3789$^{+75}_{-82}$ & 0.5$^{+0.0}_{-0.1}$  \\ 
1404.02 & 10.1 & 1.0 & 0.9$^{+0.16}_{-0.21}$ & 3.0$^{+2.29}_{-1.67}$ & 3751$^{+219}_{-219}$ & 0.5$^{+0.1}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
1422.04 & 9.1 & 0.9 & 1.2$^{+0.15}_{-0.18}$ & 0.4$^{+0.15}_{-0.13}$ & 3526$^{+71}_{-78}$ & 0.4$^{+0.0}_{-0.1}$ & Kepler-296 f & 1.8$^{+0.31}_{-0.30}$ & 0.6$^{+0.21}_{-0.25}$ & 3740$^{+130}_{-130}$ & 0.5$^{+0.1}_{-0.1}$  \\ 
1422.05 & 10.5 & 1.0 & 1.1$^{+0.13}_{-0.16}$ & 0.9$^{+0.33}_{-0.30}$ & 3526$^{+71}_{-78}$ & 0.4$^{+0.0}_{-0.1}$ & Kepler-296 e & 1.5$^{+0.26}_{-0.24}$ & 1.4$^{+0.47}_{-0.58}$ & 3740$^{+130}_{-130}$ & 0.5$^{+0.1}_{-0.1}$  \\ 
1596.02 & 16.5 & 0.7 & 1.9$^{+0.13}_{-0.17}$ & 0.4$^{+0.09}_{-0.10}$ & 3883$^{+69}_{-93}$ & 0.5$^{+0.0}_{-0.0}$ & Kepler-309 c & 1.9$^{+0.13}_{-0.17}$ & 0.4$^{+0.09}_{-0.10}$ & 3883$^{+69}_{-93}$ & 0.5$^{+0.0}_{-0.0}$  \\ 
2162.02 & 11.1 & 0.9 & 1.4$^{+0.18}_{-0.18}$ & 2.1$^{+0.76}_{-0.59}$ & 5678$^{+113}_{-102}$ & 0.9$^{+0.1}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
2194.03 & 7.9 & 0.5 & 1.4$^{+0.18}_{-0.18}$ & 0.7$^{+0.29}_{-0.22}$ & 5670$^{+113}_{-102}$ & 0.9$^{+0.1}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
2418.01 & 11.7 & 0.9 & 1.7$^{+0.12}_{-0.21}$ & 0.3$^{+0.08}_{-0.11}$ & 3576$^{+71}_{-85}$ & 0.5$^{+0.0}_{-0.1}$ & Kepler-1229 b & 1.7$^{+0.12}_{-0.21}$ & 0.3$^{+0.08}_{-0.11}$ & 3576$^{+71}_{-85}$ & 0.5$^{+0.0}_{-0.1}$  \\ 
2626.01 & 14.6 & 1.0 & 1.6$^{+0.20}_{-0.21}$ & 0.8$^{+0.30}_{-0.25}$ & 3554$^{+71}_{-80}$ & 0.4$^{+0.0}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
2650.01 & 10.1 & 1.0 & 1.1$^{+0.07}_{-0.10}$ & 1.7$^{+0.35}_{-0.42}$ & 3765$^{+75}_{-83}$ & 0.5$^{+0.0}_{-0.0}$ & Kepler-395 c & 1.1$^{+0.07}_{-0.10}$ & 1.7$^{+0.35}_{-0.42}$ & 3765$^{+75}_{-83}$ & 0.5$^{+0.0}_{-0.0}$  \\ 
2719.02 & 10.0 & 1.0 & 1.5$^{+0.10}_{-0.16}$ & 2.0$^{+0.53}_{-0.58}$ & 4827$^{+129}_{-144}$ & 0.8$^{+0.1}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
3010.01 & 12.7 & 1.0 & 1.4$^{+0.07}_{-0.10}$ & 0.8$^{+0.17}_{-0.16}$ & 3808$^{+69}_{-76}$ & 0.5$^{+0.0}_{-0.0}$ & Kepler-1410 b & 1.4$^{+0.07}_{-0.10}$ & 0.8$^{+0.17}_{-0.16}$ & 3808$^{+69}_{-76}$ & 0.5$^{+0.0}_{-0.0}$  \\ 
3034.01 & 11.9 & 1.0 & 1.7$^{+0.12}_{-0.17}$ & 1.7$^{+0.40}_{-0.45}$ & 3720$^{+73}_{-81}$ & 0.5$^{+0.0}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
3282.01 & 14.7 & 1.0 & 1.8$^{+0.09}_{-0.13}$ & 1.3$^{+0.26}_{-0.26}$ & 3899$^{+78}_{-78}$ & 0.5$^{+0.0}_{-0.0}$ & Kepler-1455 b & 1.8$^{+0.09}_{-0.13}$ & 1.3$^{+0.26}_{-0.26}$ & 3899$^{+78}_{-78}$ & 0.5$^{+0.0}_{-0.0}$  \\ 
3284.01 & 11.9 & 1.0 & 1.0$^{+0.06}_{-0.07}$ & 1.6$^{+0.37}_{-0.34}$ & 3749$^{+75}_{-84}$ & 0.5$^{+0.0}_{-0.0}$ & Kepler-438 b & 1.1$^{+0.11}_{-0.22}$ & 1.7$^{+0.43}_{-0.50}$ & 3748$^{+112}_{-112}$ & 0.5$^{+0.0}_{-0.1}$  \\ 
3497.01 & 19.6 & 1.0 & 0.8$^{+0.12}_{-0.16}$ & 1.4$^{+0.58}_{-0.58}$ & 3419$^{+67}_{-76}$ & 0.3$^{+0.1}_{-0.1}$ & Kepler-1512 b & 0.8$^{+0.12}_{-0.16}$ & 1.4$^{+0.58}_{-0.58}$ & 3419$^{+67}_{-76}$ & 0.3$^{+0.1}_{-0.1}$  \\ 
4005.01 & 17.8 & 1.0 & 2.2$^{+0.22}_{-0.16}$ & 1.7$^{+0.47}_{-0.31}$ & 5431$^{+81}_{-81}$ & 0.9$^{+0.1}_{-0.1}$ & Kepler-439 b & 2.2$^{+0.11}_{-0.44}$ & 1.9$^{+0.46}_{-0.26}$ & 5431$^{+100}_{-100}$ & 0.9$^{+0.1}_{-0.0}$  \\ 
4036.01 & 14.8 & 1.0 & 1.7$^{+0.10}_{-0.06}$ & 0.8$^{+0.17}_{-0.12}$ & 4798$^{+95}_{-95}$ & 0.7$^{+0.0}_{-0.0}$ & Kepler-1544 b & 1.7$^{+0.10}_{-0.06}$ & 0.8$^{+0.17}_{-0.12}$ & 4798$^{+95}_{-95}$ & 0.7$^{+0.0}_{-0.0}$  \\ 
4087.01 & 15.7 & 1.0 & 1.6$^{+0.10}_{-0.08}$ & 0.7$^{+0.14}_{-0.11}$ & 4133$^{+74}_{-82}$ & 0.6$^{+0.0}_{-0.0}$ & Kepler-440 b & 1.9$^{+0.22}_{-0.22}$ & 1.4$^{+0.32}_{-0.35}$ & 4134$^{+154}_{-154}$ & 0.6$^{+0.0}_{-0.1}$  \\ 
4356.01 & 11.0 & 1.0 & 1.7$^{+0.14}_{-0.20}$ & 0.3$^{+0.09}_{-0.09}$ & 4367$^{+124}_{-155}$ & 0.5$^{+0.0}_{-0.1}$ & Kepler-1593 b & 1.7$^{+0.14}_{-0.20}$ & 0.3$^{+0.09}_{-0.09}$ & 4367$^{+124}_{-155}$ & 0.5$^{+0.0}_{-0.1}$  \\ 
4427.01 & 10.8 & 1.0 & 1.6$^{+0.12}_{-0.14}$ & 0.2$^{+0.06}_{-0.05}$ & 3788$^{+76}_{-84}$ & 0.5$^{+0.0}_{-0.0}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
4460.01 & 10.7 & 1.0 & 2.0$^{+0.30}_{-0.29}$ & 1.4$^{+0.55}_{-0.44}$ & 5497$^{+82}_{-74}$ & 1.1$^{+0.2}_{-0.2}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
4550.01 & 9.6 & 0.9 & 1.8$^{+0.05}_{-0.12}$ & 1.3$^{+0.17}_{-0.24}$ & 4821$^{+76}_{-86}$ & 0.8$^{+0.0}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
4622.01 & 9.7 & 1.0 & 1.6$^{+0.09}_{-0.06}$ & 0.3$^{+0.06}_{-0.05}$ & 4339$^{+78}_{-87}$ & 0.6$^{+0.0}_{-0.0}$ & Kepler-441 b & 1.6$^{+0.22}_{-0.22}$ & 0.2$^{+0.08}_{-0.06}$ & 4340$^{+177}_{-177}$ & 0.6$^{+0.0}_{-0.1}$  \\ 
4742.01 & 12.9 & 1.0 & 1.3$^{+0.07}_{-0.05}$ & 0.8$^{+0.15}_{-0.11}$ & 4401$^{+78}_{-78}$ & 0.6$^{+0.0}_{-0.0}$ & Kepler-442 b & 1.3$^{+0.11}_{-0.22}$ & 0.7$^{+0.20}_{-0.10}$ & 4402$^{+100}_{-100}$ & 0.6$^{+0.0}_{-0.0}$  \\ 
5375.01 & 7.2 & 0.2 & 5.9$^{+3.64}_{-4.46}$ & 7.5$^{+14.00}_{-7.13}$ & 5142$^{+120}_{-180}$ & 2.8$^{+1.7}_{-2.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
7016.01 & 7.6 & 0.8 & 1.1$^{+0.20}_{-0.10}$ & 0.6$^{+0.32}_{-0.15}$ & 5579$^{+150}_{-150}$ & 0.8$^{+0.1}_{-0.1}$ & Kepler-452 b & 1.6$^{+0.23}_{-0.20}$ & 1.1$^{+0.31}_{-0.19}$ & 5757$^{+85}_{-85}$ & 1.1$^{+0.1}_{-0.1}$  \\ 
7223.01 & 10.3 & 0.9 & 1.6$^{+0.27}_{-0.12}$ & 0.5$^{+0.29}_{-0.13}$ & 5366$^{+160}_{-144}$ & 0.7$^{+0.1}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
7703.01 & 7.4 & 0.3 & 2.0$^{+0.61}_{-0.22}$ & 1.0$^{+0.92}_{-0.30}$ & 6031$^{+180}_{-198}$ & 1.0$^{+0.3}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
7706.01 & 7.5 & 0.8 & 1.2$^{+0.08}_{-0.16}$ & 2.0$^{+0.55}_{-0.68}$ & 4281$^{+115}_{-140}$ & 0.5$^{+0.0}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
7711.01 & 8.5 & 1.0 & 1.3$^{+0.34}_{-0.12}$ & 0.9$^{+0.66}_{-0.22}$ & 5734$^{+154}_{-154}$ & 0.8$^{+0.2}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
7716.01 & 7.1 & 0.2 & 1.3$^{+0.25}_{-0.10}$ & 0.4$^{+0.24}_{-0.09}$ & 5700$^{+171}_{-153}$ & 0.7$^{+0.1}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
7880.01 & 7.2 & 0.1 & 1.8$^{+0.48}_{-0.26}$ & 1.1$^{+0.80}_{-0.37}$ & 6626$^{+158}_{-217}$ & 1.1$^{+0.3}_{-0.2}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
7882.01 & 7.2 & 0.5 & 1.3$^{+0.08}_{-0.12}$ & 1.8$^{+0.49}_{-0.47}$ & 4348$^{+130}_{-130}$ & 0.6$^{+0.0}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
7894.01 & 8.5 & 0.8 & 1.6$^{+0.49}_{-0.15}$ & 1.0$^{+0.87}_{-0.27}$ & 5995$^{+163}_{-181}$ & 0.9$^{+0.3}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
7915.01 & 7.2 & 0.3 & 2.1$^{+0.65}_{-0.43}$ & 2.0$^{+1.81}_{-0.91}$ & 6337$^{+176}_{-220}$ & 1.2$^{+0.4}_{-0.2}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
7923.01 & 10.0 & 0.8 & 1.0$^{+0.12}_{-0.10}$ & 0.4$^{+0.20}_{-0.13}$ & 5060$^{+192}_{-174}$ & 0.9$^{+0.1}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
7930.01 & 8.0 & 0.5 & 1.4$^{+0.11}_{-0.11}$ & 0.3$^{+0.08}_{-0.07}$ & 5031$^{+135}_{-150}$ & 0.6$^{+0.0}_{-0.0}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
7931.01 & 7.5 & 0.5 & 2.1$^{+0.64}_{-0.35}$ & 2.6$^{+2.40}_{-1.01}$ & 6086$^{+193}_{-214}$ & 1.1$^{+0.3}_{-0.2}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
7932.01 & 7.2 & 0.2 & 1.0$^{+0.22}_{-0.15}$ & 0.5$^{+0.33}_{-0.18}$ & 5637$^{+169}_{-152}$ & 0.8$^{+0.2}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
7938.01 & 7.5 & 0.5 & 2.3$^{+0.53}_{-1.32}$ & 8.6$^{+6.29}_{-7.18}$ & 5989$^{+213}_{-192}$ & 2.5$^{+0.6}_{-1.4}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
7953.01 & 7.3 & 0.3 & 1.4$^{+0.33}_{-0.12}$ & 0.6$^{+0.37}_{-0.14}$ & 5580$^{+150}_{-166}$ & 0.9$^{+0.2}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
7954.01 & 8.9 & 0.8 & 1.7$^{+0.46}_{-0.14}$ & 0.7$^{+0.52}_{-0.18}$ & 5769$^{+155}_{-172}$ & 0.8$^{+0.2}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
7992.01 & 8.7 & 0.1 & 1.8$^{+0.56}_{-0.18}$ & 2.1$^{+1.81}_{-0.61}$ & 6461$^{+155}_{-213}$ & 1.0$^{+0.3}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
8000.01 & 8.7 & 1.0 & 1.7$^{+0.43}_{-0.14}$ & 1.2$^{+0.90}_{-0.30}$ & 5663$^{+169}_{-152}$ & 0.8$^{+0.2}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
8012.01 & 7.7 & 1.0 & 0.4$^{+0.17}_{-0.12}$ & 0.4$^{+0.47}_{-0.19}$ & 3374$^{+112}_{-82}$ & 0.2$^{+0.1}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
8048.01 & 7.2 & 0.3 & 1.3$^{+0.36}_{-0.11}$ & 0.9$^{+0.70}_{-0.23}$ & 6156$^{+167}_{-186}$ & 0.8$^{+0.2}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
8085.01 & 7.9 & 0.4 & 1.7$^{+0.46}_{-0.31}$ & 1.0$^{+0.82}_{-0.41}$ & 5979$^{+161}_{-179}$ & 1.0$^{+0.3}_{-0.2}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
8107.01 & 7.6 & 0.4 & 1.7$^{+0.45}_{-0.67}$ & 2.3$^{+1.88}_{-1.60}$ & 6180$^{+195}_{-238}$ & 1.9$^{+0.5}_{-0.8}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
8174.01 & 7.4 & 0.7 & 0.6$^{+0.07}_{-0.07}$ & 0.7$^{+0.28}_{-0.21}$ & 5332$^{+160}_{-144}$ & 0.8$^{+0.1}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
8242.01 & 7.1 & 0.2 & 1.4$^{+0.32}_{-0.11}$ & 0.8$^{+0.56}_{-0.19}$ & 5762$^{+155}_{-155}$ & 0.8$^{+0.2}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
8246.01 & 7.2 & 0.2 & 1.6$^{+0.45}_{-0.37}$ & 1.5$^{+1.27}_{-0.71}$ & 6067$^{+182}_{-182}$ & 1.2$^{+0.3}_{-0.3}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
8253.01 & 7.9 & 0.1 & 0.9$^{+0.13}_{-0.04}$ & 0.6$^{+0.22}_{-0.08}$ & 5547$^{+74}_{-83}$ & 0.9$^{+0.1}_{-0.0}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
8259.01 & 7.5 & 0.3 & 1.7$^{+0.52}_{-0.18}$ & 1.1$^{+1.00}_{-0.34}$ & 6299$^{+170}_{-226}$ & 0.9$^{+0.3}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
8272.01 & 7.6 & 0.1 & 1.1$^{+0.37}_{-0.13}$ & 1.1$^{+1.04}_{-0.32}$ & 6263$^{+169}_{-188}$ & 1.0$^{+0.3}_{-0.1}$ & \nodata & \nodata & \nodata & \nodata & \nodata  \\ 
\enddata
\tablecomments{KOIs with confirmed planet numbers have been confirmed as planetary in nature either via ground-based follow-up observations or statistical analyses. In these cases we list the confirmed \kepler{} planet number, confirmed values for the planet radius, insolation flux, and stellar effective temperature and radius, and reference for the confirmation study.}
\label{t:hz}
\end{deluxetable*}



==> Table-hz3.tex <==
\clearpage
\LongTables
\begin{deluxetable*}{rr1rrrrrrr}
\tablecolumns{10}
\tabletypesize{\scriptsize}
\tablewidth{\linewidth}
\tablecaption{Habitable Zone Planet Candidates}
\tablehead{
\colhead{KOI} &
\colhead{KIC} &
\colhead{Kepler} &
\colhead{Period} &
\colhead{\rp} &
\colhead{$F_{\rm p}$} &
\colhead{\tstar} &
\colhead{\rstar} &
\colhead{MES} &
\colhead{Score} \\ 
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{[days]} &
\colhead{[\re]} &
\colhead{[$F_{\rm e}$]} &
\colhead{[K]} &
\colhead{[\rsun]} 
}
\startdata
172.02 & 8692861 & Kepler-69 c & 242.46130 & 1.7$^{+0.21}_{-0.22}$ & 1.6$^{+0.59}_{-0.45}$ & 5637$^{+113}_{-101}$ & 0.9$^{+0.1}_{-0.1}$ & 18.0 & 0.7 \\ 
238.03 & 7219825 & \nodata & 362.97828 & 2.0$^{+0.33}_{-0.29}$ & 1.8$^{+0.87}_{-0.60}$ & 6086$^{+133}_{-133}$ & 1.2$^{+0.2}_{-0.2}$ & 11.9 & 0.8 \\ 
438.02 & 12302530 & Kepler-155 c & 52.66153 & 1.9$^{+0.11}_{-0.12}$ & 1.3$^{+0.26}_{-0.25}$ & 3984$^{+71}_{-86}$ & 0.5$^{+0.0}_{-0.0}$ & 30.6 & 1.0 \\ 
463.01 & 8845205 & Kepler-560 b & 18.47763 & 1.6$^{+0.32}_{-0.29}$ & 1.2$^{+0.72}_{-0.47}$ & 3395$^{+74}_{-67}$ & 0.3$^{+0.1}_{-0.1}$ & 78.0 & 0.0 \\ 
494.01 & 3966801 & Kepler-577 b & 25.69581 & 1.7$^{+0.21}_{-0.33}$ & 2.3$^{+1.17}_{-1.10}$ & 3787$^{+163}_{-204}$ & 0.5$^{+0.1}_{-0.1}$ & 35.9 & 1.0 \\ 
571.05 & 8120608 & Kepler-186 f & 129.94410 & 1.2$^{+0.11}_{-0.14}$ & 0.2$^{+0.07}_{-0.06}$ & 3751$^{+75}_{-84}$ & 0.4$^{+0.0}_{-0.1}$ & 7.7 & 0.7 \\ 
701.03 & 9002278 & Kepler-62 e & 122.38740 & 1.7$^{+0.10}_{-0.07}$ & 1.2$^{+0.27}_{-0.19}$ & 4926$^{+98}_{-98}$ & 0.7$^{+0.0}_{-0.0}$ & 35.9 & 1.0 \\ 
701.04 & 9002278 & Kepler-62 f & 267.29100 & 1.4$^{+0.08}_{-0.06}$ & 0.4$^{+0.09}_{-0.07}$ & 4926$^{+98}_{-98}$ & 0.7$^{+0.0}_{-0.0}$ & 14.3 & 0.0 \\ 
812.03 & 4139816 & Kepler-235 e & 46.18420 & 1.8$^{+0.12}_{-0.15}$ & 1.3$^{+0.29}_{-0.30}$ & 3950$^{+70}_{-86}$ & 0.5$^{+0.0}_{-0.0}$ & 18.0 & 1.0 \\ 
854.01 & 6435936 & Kepler-705 b & 56.05608 & 1.9$^{+0.12}_{-0.22}$ & 0.7$^{+0.15}_{-0.19}$ & 3593$^{+71}_{-86}$ & 0.5$^{+0.0}_{-0.1}$ & 19.3 & 1.0 \\ 
947.01 & 9710326 & Kepler-737 b & 28.59914 & 1.8$^{+0.16}_{-0.21}$ & 1.9$^{+0.52}_{-0.53}$ & 3755$^{+75}_{-84}$ & 0.5$^{+0.0}_{-0.1}$ & 45.7 & 1.0 \\ 
1078.03 & 10166274 & Kepler-267 d & 28.46465 & 1.9$^{+0.14}_{-0.22}$ & 1.9$^{+0.49}_{-0.55}$ & 3789$^{+75}_{-82}$ & 0.5$^{+0.0}_{-0.1}$ & 22.2 & 1.0 \\ 
1298.02 & 10604335 & Kepler-283 c & 92.74958 & 1.9$^{+0.08}_{-0.10}$ & 0.8$^{+0.15}_{-0.14}$ & 4141$^{+83}_{-91}$ & 0.6$^{+0.0}_{-0.0}$ & 10.7 & 0.0 \\ 
1404.02 & 8874090 & \nodata & 18.90609 & 0.9$^{+0.16}_{-0.21}$ & 3.0$^{+2.29}_{-1.67}$ & 3751$^{+219}_{-219}$ & 0.5$^{+0.1}_{-0.1}$ & 10.1 & 1.0 \\ 
1422.02 & 11497958 & Kepler-296 d & 19.85029 & 1.5$^{+0.19}_{-0.23}$ & 1.8$^{+0.68}_{-0.62}$ & 3526$^{+71}_{-78}$ & 0.4$^{+0.0}_{-0.1}$ & 25.1 & 1.0 \\ 
1422.04 & 11497958 & Kepler-296 f & 63.33627 & 1.2$^{+0.15}_{-0.18}$ & 0.4$^{+0.15}_{-0.13}$ & 3526$^{+71}_{-78}$ & 0.4$^{+0.0}_{-0.1}$ & 9.1 & 0.9 \\ 
1422.05 & 11497958 & Kepler-296 e & 34.14211 & 1.1$^{+0.13}_{-0.16}$ & 0.9$^{+0.33}_{-0.30}$ & 3526$^{+71}_{-78}$ & 0.4$^{+0.0}_{-0.1}$ & 10.5 & 1.0 \\ 
1596.02 & 10027323 & Kepler-309 c & 105.35823 & 1.9$^{+0.13}_{-0.17}$ & 0.4$^{+0.09}_{-0.10}$ & 3883$^{+69}_{-93}$ & 0.5$^{+0.0}_{-0.0}$ & 16.5 & 0.7 \\ 
2162.02 & 9205938 & \nodata & 199.66876 & 1.4$^{+0.18}_{-0.18}$ & 2.1$^{+0.76}_{-0.59}$ & 5678$^{+113}_{-102}$ & 0.9$^{+0.1}_{-0.1}$ & 11.1 & 0.9 \\ 
2418.01 & 10027247 & Kepler-1229 b & 86.82952 & 1.7$^{+0.12}_{-0.21}$ & 0.3$^{+0.08}_{-0.11}$ & 3576$^{+71}_{-85}$ & 0.5$^{+0.0}_{-0.1}$ & 11.7 & 0.9 \\ 
2626.01 & 11768142 & \nodata & 38.09707 & 1.6$^{+0.20}_{-0.21}$ & 0.8$^{+0.30}_{-0.25}$ & 3554$^{+71}_{-80}$ & 0.4$^{+0.0}_{-0.1}$ & 14.6 & 1.0 \\ 
2650.01 & 8890150 & Kepler-395 c & 34.98978 & 1.1$^{+0.07}_{-0.10}$ & 1.7$^{+0.35}_{-0.42}$ & 3765$^{+75}_{-83}$ & 0.5$^{+0.0}_{-0.0}$ & 10.1 & 1.0 \\ 
2719.02 & 5184911 & \nodata & 106.25976 & 1.5$^{+0.10}_{-0.16}$ & 2.0$^{+0.53}_{-0.58}$ & 4827$^{+129}_{-144}$ & 0.8$^{+0.1}_{-0.1}$ & 10.0 & 1.0 \\ 
3010.01 & 3642335 & Kepler-1410 b & 60.86610 & 1.4$^{+0.07}_{-0.10}$ & 0.8$^{+0.17}_{-0.16}$ & 3808$^{+69}_{-76}$ & 0.5$^{+0.0}_{-0.0}$ & 12.7 & 1.0 \\ 
3034.01 & 2973386 & \nodata & 31.02092 & 1.7$^{+0.12}_{-0.17}$ & 1.7$^{+0.40}_{-0.45}$ & 3720$^{+73}_{-81}$ & 0.5$^{+0.0}_{-0.1}$ & 11.9 & 1.0 \\ 
3138.01 & 6444896 & Kepler-1649 b & 8.68909 & 0.5$^{+0.00}_{-0.00}$ & 0.5$^{+0.00}_{-0.00}$ & 2703$^{+0}_{-0}$ & 0.1$^{+0.0}_{-0.0}$ & 12.0 & 1.0 \\ 
3282.01 & 12066569 & Kepler-1455 b & 49.27684 & 1.8$^{+0.09}_{-0.13}$ & 1.3$^{+0.26}_{-0.26}$ & 3899$^{+78}_{-78}$ & 0.5$^{+0.0}_{-0.0}$ & 14.7 & 1.0 \\ 
3284.01 & 6497146 & Kepler-438 b & 35.23319 & 1.0$^{+0.06}_{-0.07}$ & 1.6$^{+0.37}_{-0.34}$ & 3749$^{+75}_{-84}$ & 0.5$^{+0.0}_{-0.0}$ & 11.9 & 1.0 \\ 
3497.01 & 8424002 & Kepler-1512 b & 20.35972 & 0.8$^{+0.12}_{-0.16}$ & 1.4$^{+0.58}_{-0.58}$ & 3419$^{+67}_{-76}$ & 0.3$^{+0.1}_{-0.1}$ & 19.6 & 1.0 \\ 
4005.01 & 8142787 & Kepler-439 b & 178.13960 & 2.2$^{+0.22}_{-0.16}$ & 1.7$^{+0.47}_{-0.31}$ & 5431$^{+81}_{-81}$ & 0.9$^{+0.1}_{-0.1}$ & 17.8 & 1.0 \\ 
4036.01 & 11415243 & Kepler-1544 b & 168.81133 & 1.7$^{+0.10}_{-0.06}$ & 0.8$^{+0.17}_{-0.12}$ & 4798$^{+95}_{-95}$ & 0.7$^{+0.0}_{-0.0}$ & 14.8 & 1.0 \\ 
4087.01 & 6106282 & Kepler-440 b & 101.11141 & 1.6$^{+0.10}_{-0.08}$ & 0.7$^{+0.14}_{-0.11}$ & 4133$^{+74}_{-82}$ & 0.6$^{+0.0}_{-0.0}$ & 15.7 & 1.0 \\ 
4356.01 & 8459663 & Kepler-1593 b & 174.51028 & 1.7$^{+0.14}_{-0.20}$ & 0.3$^{+0.09}_{-0.09}$ & 4367$^{+124}_{-155}$ & 0.5$^{+0.0}_{-0.1}$ & 11.0 & 1.0 \\ 
4427.01 & 4172805 & \nodata & 147.66173 & 1.6$^{+0.12}_{-0.14}$ & 0.2$^{+0.06}_{-0.05}$ & 3788$^{+76}_{-84}$ & 0.5$^{+0.0}_{-0.0}$ & 10.8 & 1.0 \\ 
4460.01 & 9947389 & \nodata & 284.72721 & 2.0$^{+0.30}_{-0.29}$ & 1.4$^{+0.55}_{-0.44}$ & 5497$^{+82}_{-74}$ & 1.1$^{+0.2}_{-0.2}$ & 10.7 & 1.0 \\ 
4550.01 & 5977470 & \nodata & 140.25194 & 1.8$^{+0.05}_{-0.12}$ & 1.3$^{+0.17}_{-0.24}$ & 4821$^{+76}_{-86}$ & 0.8$^{+0.0}_{-0.1}$ & 9.6 & 0.9 \\ 
4622.01 & 11284772 & Kepler-441 b & 207.24820 & 1.6$^{+0.09}_{-0.06}$ & 0.3$^{+0.06}_{-0.05}$ & 4339$^{+78}_{-87}$ & 0.6$^{+0.0}_{-0.0}$ & 9.7 & 1.0 \\ 
4742.01 & 4138008 & Kepler-442 b & 112.30530 & 1.3$^{+0.07}_{-0.05}$ & 0.8$^{+0.15}_{-0.11}$ & 4401$^{+78}_{-78}$ & 0.6$^{+0.0}_{-0.0}$ & 12.9 & 1.0 \\ 
7016.01 & 8311864 & Kepler-452 b & 384.84300 & 1.1$^{+0.20}_{-0.10}$ & 0.6$^{+0.32}_{-0.15}$ & 5579$^{+150}_{-150}$ & 0.8$^{+0.1}_{-0.1}$ & 7.6 & 0.8 \\ 
7223.01 & 9674320 & \nodata & 317.06242 & 1.6$^{+0.27}_{-0.12}$ & 0.5$^{+0.29}_{-0.13}$ & 5366$^{+160}_{-144}$ & 0.7$^{+0.1}_{-0.1}$ & 10.3 & 0.9 \\ 
7706.01 & 4762283 & \nodata & 42.04952 & 1.2$^{+0.08}_{-0.16}$ & 2.0$^{+0.55}_{-0.68}$ & 4281$^{+115}_{-140}$ & 0.5$^{+0.0}_{-0.1}$ & 7.5 & 0.8 \\ 
7711.01 & 4940203 & \nodata & 302.77982 & 1.3$^{+0.34}_{-0.12}$ & 0.9$^{+0.66}_{-0.22}$ & 5734$^{+154}_{-154}$ & 0.8$^{+0.2}_{-0.1}$ & 8.5 & 1.0 \\ 
7882.01 & 8364232 & \nodata & 65.41518 & 1.3$^{+0.08}_{-0.12}$ & 1.8$^{+0.49}_{-0.47}$ & 4348$^{+130}_{-130}$ & 0.6$^{+0.0}_{-0.1}$ & 7.2 & 0.5 \\ 
7894.01 & 8555967 & \nodata & 347.97611 & 1.6$^{+0.49}_{-0.15}$ & 1.0$^{+0.87}_{-0.27}$ & 5995$^{+163}_{-181}$ & 0.9$^{+0.3}_{-0.1}$ & 8.5 & 0.8 \\ 
7923.01 & 9084569 & \nodata & 395.13138 & 1.0$^{+0.12}_{-0.10}$ & 0.4$^{+0.20}_{-0.13}$ & 5060$^{+192}_{-174}$ & 0.9$^{+0.1}_{-0.1}$ & 10.0 & 0.8 \\ 
7938.01 & 9469494 & \nodata & 275.56030 & 2.3$^{+0.53}_{-1.32}$ & 8.6$^{+6.29}_{-7.18}$ & 5989$^{+213}_{-192}$ & 2.5$^{+0.6}_{-1.4}$ & 7.5 & 0.5 \\ 
7954.01 & 9650762 & \nodata & 372.15035 & 1.7$^{+0.46}_{-0.14}$ & 0.7$^{+0.52}_{-0.18}$ & 5769$^{+155}_{-172}$ & 0.8$^{+0.2}_{-0.1}$ & 8.9 & 0.8 \\ 
8000.01 & 10331279 & \nodata & 225.48805 & 1.7$^{+0.43}_{-0.14}$ & 1.2$^{+0.90}_{-0.30}$ & 5663$^{+169}_{-152}$ & 0.8$^{+0.2}_{-0.1}$ & 8.7 & 1.0 \\ 
8012.01 & 10452252 & \nodata & 34.57372 & 0.4$^{+0.17}_{-0.12}$ & 0.4$^{+0.47}_{-0.19}$ & 3374$^{+112}_{-82}$ & 0.2$^{+0.1}_{-0.1}$ & 7.7 & 1.0 \\ 
8174.01 & 8873873 & \nodata & 295.06066 & 0.6$^{+0.07}_{-0.07}$ & 0.7$^{+0.28}_{-0.21}$ & 5332$^{+160}_{-144}$ & 0.8$^{+0.1}_{-0.1}$ & 7.4 & 0.7 \\ 
\enddata
\label{hzearthstab}
\end{deluxetable*}


==> ephemmatch-full.tex <==
001433962-01 & 3924.01 & 1:1 & 13.5 & 3 & -2 & 14.91 & 0.56 & 4.7434E+02 & Direct-PRF & 0\\
001724961-01 & 001724968-01 & 1:1 & 4.7 & 1 & -1 & 13.39 & -2.96 & 2.1190E+00 & Direct-PRF & 0\\
002166206-01 & 3735.01 & 1:1 & 8.3 & -1 & -2 & 17.64 & -4.34 & 5.6706E+02 & Direct-PRF & 0\\
002309585-01 & 5982.01 & 1:1 & 11.7 & -2 & 1 & 13.93 & 1.45 & 2.0011E+02 & Direct-PRF & 0\\
002437112-01 & 3598.01 & 1:1 & 19.7 & -5 & 1 & 17.63 & -1.48 & 1.0525E+03 & Direct-PRF & 0\\
002437112-02 & 002437149-02 & 2:1 & 19.7 & -5 & 1 & 17.63 & -1.48 & 6.9253E+02 & Direct-PRF & 0\\
002437488-01 & 6268.01 & 1:1 & 10.6 & 0 & 3 & 16.98 & -2.02 & 2.5330E+02 & Direct-PRF & 0\\
002437804-01 & 002437783-01 & 1:1 & 14.4 & 4 & -1 & 17.30 & -3.14 & 1.4225E+02 & Direct-PRF & 0\\
002438062-01 & 6270.01 & 1:1 & 3.5 & -1 & 1 & \nodata & \nodata & 2.6640E+00 & Direct-PRF & 0\\
002438070-01 & 6270.01 & 1:1 & 6.3 & 2 & 0 & \nodata & \nodata & 6.0790E+01 & Direct-PRF & 0\\
002438513-02 & 1003.01 & 1:1 & 13.3 & 3 & -1 & 16.21 & -2.23 & 2.2624E+02 & Direct-PRF & 0\\
002438517-01 & 3699.01 & 1:1 & 12.5 & -1 & 3 & 17.77 & -2.23 & 6.4113E+02 & Direct-PRF & 0\\
002441151-01 & 3642.01 & 1:1 & 10.6 & 2 & 1 & 16.65 & -1.97 & 9.3570E+01 & Direct-PRF & 0\\
002445154-01 & 5983.01 & 1:1 & 16.7 & 1 & 4 & 13.55 & 1.61 & 2.3290E+02 & Direct-PRF & 0\\
002449053-01 & 002449084-pri & 1:1 & 18.4 & 4 & 2 & 15.02 & 0.12 & 7.7040E+03 & Direct-PRF & 0\\
002449074-01 & 002449090-pri & 1:1 & 10.6 & -1 & 3 & 16.24 & -3.09 & 5.5452E+02 & Direct-PRF & 0\\
002449074-02 & 002449090-sec & 1:1 & 10.6 & -1 & 3 & 16.24 & -3.09 & 4.2150E+02 & Direct-PRF & 0\\
002452450-01 & 3687.01 & 1:1 & 7.4 & 0 & -2 & 16.47 & -3.36 & 1.4148E+02 & Direct-PRF & 0\\
002558363-01 & 3855.01 & 1:1 & 6.9 & -1 & 1 & 18.55 & -2.55 & 1.0683E+03 & Direct-PRF & 0\\
002569488-01 & 3704.01 & 1:1 & 11.4 & -3 & 1 & 17.38 & -3.22 & 4.8743E+02 & Direct-PRF & 0\\
002570505-01 & 6286.01 & 1:1 & 174.2 & 37 & -22 & 10.67 & 2.89 & 2.0675E+04 & Direct-PRF & 0\\
002570767-01 & 6286.01 & 1:1 & 204.1 & 51 & 4 & 10.67 & 2.09 & 2.3737E+04 & Direct-PRF & 0\\
002570773-01 & 6286.01 & 1:1 & 231.8 & 58 & 0 & 10.67 & 6.18 & 6.7181E+02 & Direct-PRF & 0\\
002574543-01 & 002987660-01 & 6:1 & 1094.7 & 116 & -8 & 7.95 & 5.30 & 1.6533E-01 & Direct-PRF & 1\\
002707916-01 & 6286.01 & 1:1 & 168.8 & 0 & -42 & 10.67 & 5.67 & 1.3813E+03 & Direct-PRF & 0\\
002707985-01 & 6286.01 & 1:1 & 100.8 & -6 & -24 & 10.67 & 1.81 & 2.1364E+04 & Direct-PRF & 0\\
002708172-01 & 6286.01 & 1:1 & 161.0 & -32 & 25 & 10.67 & 3.14 & 1.7803E+04 & Direct-PRF & 0\\
002708203-01 & 6286.01 & 1:1 & 105.1 & 25 & -6 & 10.67 & 2.84 & 8.9015E+03 & Direct-PRF & 0\\
002708221-01 & 6286.01 & 1:1 & 64.7 & 16 & 4 & 10.67 & 5.49 & 1.0438E+03 & Direct-PRF & 0\\
002708270-01 & 6286.01 & 1:1 & 87.5 & 2 & 22 & 10.67 & 3.31 & 4.8189E+03 & Direct-PRF & 0\\
002708278-01 & 6286.01 & 1:1 & 169.6 & -20 & 38 & 10.67 & 3.81 & 6.0463E+03 & Direct-PRF & 0\\
002708286-01 & 6286.01 & 1:1 & 127.6 & 31 & 6 & 10.67 & 4.48 & 5.2534E+03 & Direct-PRF & 0\\
002708343-01 & 6286.01 & 1:1 & 160.5 & 37 & 16 & 10.67 & 4.50 & 3.3911E+03 & Direct-PRF & 0\\
002708420-01 & 6286.01 & 1:1 & 187.9 & 16 & 45 & 10.67 & 3.24 & 8.7796E+03 & Direct-PRF & 0\\
002708445-01 & 6286.01 & 1:1 & 198.1 & 25 & 43 & 10.67 & 4.33 & 1.0682E+04 & Direct-PRF & 0\\
002711123-01 & 6290.01 & 1:1 & 7.6 & 2 & 0 & 12.34 & 0.19 & 1.4908E+01 & Direct-PRF & 0\\
002711131-01 & 6290.01 & 2:1 & 22.1 & -3 & 5 & 12.34 & 1.18 & 5.4815E+01 & Direct-PRF & 0\\
002711606-01 & 003339563-pri & 1:1 & 1990.0 & 501 & 0 & 14.18 & -0.41 & 1.1863E+04 & Col-Anomaly & 0\\
002714803-01 & 002714831-01 & 1:1 & 36.0 & 9 & 1 & 14.65 & -0.31 & 1.0556E+00 & Direct-PRF & 1\\
002714831-01 & 002714803-01 & 1:1 & 36.0 & -9 & -1 & 14.34 & 0.31 & 9.4737E-01 & Direct-PRF & 1\\
002714887-01 & 002714954-01 & 3:1 & 54.5 & 12 & 5 & 14.54 & -0.11 & 5.2727E-01 & Direct-PRF & 1\\
002714947-01 & 002714887-01 & 1:3 & 63.0 & -16 & -1 & 14.43 & -1.18 & 1.7188E+00 & Direct-PRF & 1\\
002714954-01 & 002714887-01 & 1:3 & 54.5 & -12 & -5 & 14.43 & 0.11 & 1.8966E+00 & Direct-PRF & 1\\
002715228-01 & 002715282-01 & 1:1 & 108.0 & 27 & -4 & 15.07 & 0.20 & 8.0000E-01 & Col-Anomaly & 1\\
002715282-01 & 002715228-01 & 1:1 & 108.0 & -27 & 4 & 15.27 & -0.20 & 1.2500E+00 & Col-Anomaly & 1\\
002715398-01 & 002715228-01 & 1:1 & 191.1 & -48 & -3 & 15.27 & 0.35 & 8.1081E-01 & Col-Anomaly & 1\\
002718672-01 & 002718663-02 & 1:1 & 4.8 & 0 & -1 & 13.52 & -2.73 & 1.5833E+01 & Direct-PRF & 0\\
002830919-01 & 6363.01 & 1:1 & 5083.6 & -770 & 6 & 13.76 & 0.99 & 1.0906E+03 & Col-Anomaly & 0\\
002852528-01 & 6294.01 & 1:1 & 17.4 & 0 & -4 & 15.31 & 0.40 & 8.0689E+02 & Direct-PRF & 0\\
002860793-01 & 6297.01 & 1:1 & 20.8 & -5 & 2 & 14.04 & -0.65 & 1.0908E+03 & Direct-PRF & 0\\
002987660-01 & 4947.01 & 1:6 & 1094.7 & -116 & 8 & 13.25 & -5.30 & 6.1042E+00 & Direct-PRF & 1\\
003003992-01 & 6099.01 & 1:1 & 19.8 & -5 & -2 & 13.93 & -2.77 & 2.0422E+03 & Direct-PRF & 0\\
003097346-01 & 003097352-01 & 1:1 & 10.3 & 0 & 3 & 16.94 & -5.38 & 2.0886E+03 & Direct-PRF & 0\\
003098184-01 & 003098194-01 & 1:1 & 8.8 & -2 & 0 & 13.90 & 1.25 & 6.5266E+00 & Direct-PRF & 0\\
003098184-02 & 003098194-02 & 1:1 & 8.8 & -2 & 0 & 13.90 & 1.25 & 6.1069E+00 & Direct-PRF & 0\\
003098197-01 & 003098194-01 & 1:1 & 5.7 & 0 & -1 & 13.90 & 0.94 & 3.0102E+00 & Direct-PRF & 0\\
003098197-02 & 003098194-02 & 1:1 & 5.7 & 0 & -1 & 13.90 & 0.94 & 3.0126E+00 & Direct-PRF & 0\\
003109937-01 & 1112.01 & 1:1 & 4.8 & 1 & 2 & 14.63 & 1.12 & 1.2881E+00 & Direct-PRF & 0\\
003110937-01 & 6286.01 & 1:1 & 1347.3 & -339 & 0 & 10.67 & 4.53 & 1.0337E+04 & Col-Anomaly & 0\\
003114661-01 & 3763.01 & 1:1 & 8.4 & -2 & 1 & 17.38 & -1.63 & 7.0987E+01 & Direct-PRF & 0\\
003114661-02 & 003114667-sec & 1:1 & 8.4 & -2 & 1 & 17.38 & -1.63 & 1.4825E+01 & Direct-PRF & 0\\
003117046-01 & 4479.01 & 1:1 & 1981.8 & 498 & 0 & 15.14 & -0.32 & 2.1404E+00 & Col-Anomaly & 1\\
003120276-01 & 6307.01 & 1:1 & 36.5 & 5 & 8 & 10.88 & 4.33 & 3.8282E+02 & Direct-PRF & 0\\
003120308-01 & 6307.01 & 1:1 & 38.7 & -7 & 7 & 10.88 & 3.77 & 6.0574E+02 & Direct-PRF & 0\\
003120397-01 & 6307.01 & 1:1 & 50.3 & -2 & -13 & 10.88 & 4.79 & 4.9615E+02 & Direct-PRF & 0\\
003124412-01 & 3918.01 & 1:1 & 5.8 & 1 & 0 & 18.24 & -3.33 & 9.5365E+02 & Direct-PRF & 0\\
003221119-01 & 003221207-pri & 2:1 & 82.6 & 15 & 14 & 11.97 & 1.60 & 2.2788E+04 & Direct-PRF & 0\\
003228740-01 & V404-Lyr-pri & 1:1 & 94.1 & -18 & -16 & 11.82 & 1.89 & 2.2668E+04 & Direct-PRF & 0\\
003228804-01 & V404-Lyr-pri & 1:1 & 61.4 & 4 & -14 & 11.82 & 3.19 & 5.8581E+03 & Direct-PRF & 0\\
003228824-01 & 003228804-01 & 1:1 & 11.2 & 3 & 1 & 15.01 & 0.73 & 1.0723E+00 & Direct-PRF & 0\\
003228825-01 & V404-Lyr-pri & 1:1 & 66.0 & -17 & 3 & 11.82 & 0.21 & 2.1724E+04 & Direct-PRF & 0\\
003228918-01 & 003228988-01 & 2:1 & 52.6 & -6 & -12 & 15.31 & -0.12 & 2.4696E-01 & Direct-PRF & 1\\
003228918-02 & V404-Lyr-pri & 1:1 & 31.9 & 2 & 8 & 11.82 & 3.38 & 1.9764E+02 & Direct-PRF & 0\\
003228945-01 & 003228988-01 & 1:1 & 60.1 & -15 & 1 & 15.31 & -0.29 & 7.2619E-01 & Direct-PRF & 1\\
003228986-01 & V404-Lyr-pri & 1:1 & 80.4 & 11 & 17 & 11.82 & 2.37 & 8.1464E+03 & Direct-PRF & 0\\
003228988-01 & 003228945-01 & 1:1 & 60.1 & 15 & -1 & 15.02 & 0.29 & 1.3770E+00 & Direct-PRF & 1\\
003229028-01 & V404-Lyr-pri & 1:1 & 182.9 & 46 & 1 & 11.82 & 1.22 & 2.4827E+04 & Direct-PRF & 0\\
003229073-01 & V404-Lyr-pri & 1:1 & 144.6 & 15 & 34 & 11.82 & 3.11 & 1.3368E+04 & Direct-PRF & 0\\
003230095-01 & 6311.01 & 1:1 & 83.4 & -11 & -18 & 9.00 & 6.13 & 5.0547E+02 & Direct-PRF & 0\\
003230206-01 & 6311.01 & 1:1 & 92.9 & 17 & -16 & 9.00 & 6.58 & 2.3737E+02 & Direct-PRF & 0\\
003230227-02 & 003337351-01 & 1:1 & 17.8 & 2 & -4 & 13.36 & -4.36 & 5.4598E+02 & Direct-PRF & 0\\
003230753-01 & 6101.01 & 1:1 & 23.4 & -1 & -6 & 12.55 & 2.07 & 8.5769E+02 & Direct-PRF & 0\\
003231137-01 & 3643.01 & 1:1 & 8.7 & 1 & 2 & 16.60 & -3.04 & 3.0502E+02 & Direct-PRF & 0\\
003231137-02 & 003231120-02 & 2:1 & 8.7 & 1 & 2 & 16.60 & -3.04 & 1.8475E+02 & Direct-PRF & 0\\
003231410-03 & 003231406-01 & 1:1 & 14.2 & 3 & -1 & 10.46 & 3.20 & 2.0346E+00 & Direct-PRF & 0\\
003235174-01 & 3511.01 & 3:1 & 1700.0 & 427 & 5 & 8.35 & 6.66 & 7.4940E+02 & Col-Anomaly & 0\\
003240141-01 & 003240159-pri & 5:1 & 14.7 & -2 & 3 & 12.26 & 3.13 & 2.3965E+00 & Direct-PRF & 0\\
003241557-01 & 6312.01 & 1:1 & 48.3 & 5 & 11 & 12.52 & 1.25 & 1.1593E+04 & Direct-PRF & 0\\
003241604-02 & 6312.01 & 1:1 & 34.6 & -5 & 7 & 12.52 & 2.75 & 1.9322E+03 & Direct-PRF & 0\\
003241647-01 & 6312.01 & 1:2 & 76.6 & -18 & 6 & 12.52 & 2.73 & 9.1091E+03 & Direct-PRF & 0\\
003241662-01 & 6312.01 & 1:1 & 56.0 & 7 & -13 & 12.52 & 2.67 & 4.8582E+03 & Direct-PRF & 0\\
003245638-01 & 3977.01 & 2:1 & 13.2 & 2 & -3 & 15.04 & -1.91 & 2.2410E+00 & Direct-PRF & 0\\
003245638-02 & 3977.01 & 2:1 & 13.2 & 2 & -3 & 15.04 & -1.91 & 1.8443E+00 & Direct-PRF & 0\\
003247396-01 & 4035.01 & 1:1 & 6.8 & 2 & 0 & 18.53 & -5.77 & 6.2863E+01 & Direct-PRF & 0\\
003248033-01 & 1759.01 & 1:1 & 14.3 & -4 & 0 & 15.39 & -3.23 & 1.3229E+03 & Direct-PRF & 0\\
003324986-01 & 807.01 & 1:1 & 3150.4 & -302 & 1 & 15.97 & -0.98 & 1.0906E+01 & Col-Anomaly & 1\\
003327992-01 & 003327980-pri & 1:2 & 9.1 & -2 & -1 & 12.12 & 3.46 & 1.5594E+01 & Direct-PRF & 0\\
003327993-01 & 003327980-pri & 1:2 & 70.6 & 8 & -16 & 12.12 & 3.78 & 1.2051E+03 & Direct-PRF & 0\\
003328026-01 & 003327980-pri & 1:2 & 38.6 & -7 & -7 & 12.12 & 3.03 & 1.2189E+03 & Direct-PRF & 0\\
003328027-01 & 003327980-pri & 1:2 & 51.7 & -3 & -12 & 12.12 & 3.51 & 2.6588E+03 & Direct-PRF & 0\\
003328052-01 & 003327980-pri & 1:2 & 64.2 & -10 & -12 & 12.12 & 3.42 & 1.9425E+03 & Direct-PRF & 0\\
003329643-01 & 003431321-pri & 1:1 & 20.9 & 4 & -2 & 11.20 & 3.76 & 1.2958E+02 & Direct-PRF & 0\\
003335813-01 & 003335816-pri & 1:2 & 8.3 & -2 & 1 & 12.08 & 1.71 & 2.3643E+00 & Direct-PRF & 0\\
003336476-01 & 6286.01 & 1:1 & 2112.0 & -531 & 1 & 10.67 & 1.74 & 4.0057E+04 & Col-Anomaly & 0\\
003337351-01 & 6311.01 & 1:1 & 17.8 & -2 & 4 & 9.00 & 4.36 & 1.1916E+00 & Direct-PRF & 0\\
003337425-01 & 6311.01 & 1:1 & 64.9 & 5 & 16 & 9.00 & 5.93 & 2.0307E+02 & Direct-PRF & 0\\
003337432-01 & 4980.01 & 1:1 & 82.4 & 19 & -8 & 11.29 & 2.11 & 3.8478E+03 & Direct-PRF & 0\\
003337438-01 & 4980.01 & 1:1 & 75.1 & 18 & -5 & 11.29 & 2.21 & 8.1155E+03 & Direct-PRF & 0\\
003337548-01 & 4980.01 & 1:1 & 164.1 & 41 & 1 & 11.29 & 4.38 & 5.0152E+03 & Direct-PRF & 0\\
003338674-01 & 3795.01 & 1:1 & 8.5 & 2 & 1 & 14.81 & -2.10 & 1.6073E+02 & Direct-PRF & 0\\
003338674-02 & 3795.01 & 1:2 & 8.5 & 2 & 1 & 14.81 & -2.10 & 6.4797E+02 & Direct-PRF & 0\\
003340312-01 & 3677.01 & 1:1 & 11.0 & -2 & 1 & 16.25 & -1.71 & 8.9282E+01 & Direct-PRF & 0\\
003344419-01 & 003344427-pri & 2:1 & 11.4 & -3 & 0 & 15.83 & -0.84 & 8.5050E+02 & Direct-PRF & 0\\
003344419-02 & 3764.01 & 1:1 & 11.4 & -3 & 0 & 15.83 & -0.84 & 1.0028E+03 & Direct-PRF & 0\\
003348082-01 & 003348093-pri & 1:2 & 15.2 & -2 & 3 & 16.20 & -1.16 & 8.9795E+02 & Direct-PRF & 0\\
003437739-01 & 6286.01 & 1:1 & 2553.8 & -643 & 0 & 10.67 & 4.67 & 1.0014E+04 & Col-Anomaly & 0\\
003438975-01 & 4980.01 & 1:1 & 38.3 & -2 & -10 & 11.29 & 1.01 & 3.7826E+03 & Direct-PRF & 0\\
003438976-01 & 4980.01 & 1:1 & 83.8 & -21 & 3 & 11.29 & 2.82 & 9.4968E+03 & Direct-PRF & 0\\
003439096-01 & 4980.01 & 1:1 & 45.4 & 6 & 9 & 11.29 & 2.51 & 2.1154E+03 & Direct-PRF & 0\\
003439126-03 & 4980.01 & 1:1 & 79.1 & 1 & 20 & 11.29 & 3.82 & 2.2657E+03 & Direct-PRF & 0\\
003446451-01 & 3736.01 & 2:1 & 10.6 & 3 & 1 & 16.64 & -4.33 & 7.1637E+02 & Direct-PRF & 0\\
003446451-02 & 3736.01 & 2:1 & 10.6 & 3 & 1 & 16.64 & -4.33 & 1.2690E+03 & Direct-PRF & 0\\
003448132-01 & 003448245-pri & 1:1 & 86.5 & 11 & 20 & 11.86 & 2.38 & 1.1811E+04 & Direct-PRF & 0\\
003448230-01 & 003448245-pri & 2:1 & 72.5 & -13 & 13 & 11.86 & 1.99 & 1.6535E+04 & Direct-PRF & 0\\
003448323-01 & 003448245-pri & 1:1 & 73.0 & -16 & -7 & 11.86 & 3.77 & 4.0827E+03 & Direct-PRF & 0\\
003542542-01 & 003542574-01 & 1:1 & 33.2 & 0 & -8 & 19.03 & -3.24 & 2.5485E+03 & Direct-PRF & 0\\
003542573-01 & 003542574-01 & 1:1 & 10.0 & 2 & -1 & 19.03 & -6.87 & 3.1958E+00 & Direct-PRF & 1\\
003542574-01 & 6338.01 & 1:1 & 10.0 & -2 & 1 & 12.16 & 6.87 & 3.1695E-01 & Direct-PRF & 0\\
003542588-01 & 003542574-01 & 1:1 & 17.4 & -3 & 4 & 19.03 & -5.43 & 3.1514E+03 & Direct-PRF & 0\\
003544689-01 & 3629.01 & 1:1 & 9.8 & 2 & 2 & 15.93 & -0.98 & 8.1108E+01 & Direct-PRF & 0\\
003549993-01 & 003549994-pri & 2:1 & 8.6 & 2 & -1 & 16.10 & -1.36 & 1.9895E+02 & Direct-PRF & 0\\
003556220-01 & 3899.01 & 1:1 & 10.1 & -2 & -2 & 17.66 & -4.28 & 5.3867E+03 & Direct-PRF & 0\\
003557293-01 & 003557421-pri & 2:1 & 85.4 & 16 & -15 & 10.03 & 4.41 & 2.3056E+03 & Direct-PRF & 0\\
003557293-02 & 003557421-pri & 2:1 & 85.4 & 16 & -15 & 10.03 & 4.41 & 3.1439E+03 & Direct-PRF & 0\\
003557341-01 & 003557293-02 & 1:1 & 87.8 & -22 & -2 & 14.44 & 1.42 & 3.9286E-01 & Direct-PRF & 1\\
003558803-01 & 003558822-pri & 1:1 & 22.7 & 6 & 0 & 12.25 & 0.07 & 1.3341E+03 & Direct-PRF & 0\\
003644071-01 & 3511.01 & 3:1 & 447.0 & -6 & -1 & 8.35 & 5.86 & 5.2689E+01 & Direct-PRF & 0\\
003644071-02 & 003644542-sec & 3:1 & 447.0 & -6 & -1 & 8.35 & 5.86 & 5.8303E+01 & Direct-PRF & 0\\
003644399-01 & 3511.01 & 1:1 & 146.5 & 3 & 36 & 8.35 & 7.14 & 7.5508E+02 & Direct-PRF & 0\\
003644505-01 & 3511.01 & 1:1 & 198.3 & 38 & 32 & 8.35 & 5.24 & 2.6938E+03 & Direct-PRF & 0\\
003644523-01 & 3511.01 & 1:1 & 55.0 & -13 & -5 & 8.35 & 7.58 & 8.4442E+01 & Direct-PRF & 0\\
003644523-02 & 003644542-sec & 3:1 & 55.0 & -13 & -5 & 8.35 & 7.58 & 4.5143E+01 & Direct-PRF & 0\\
003644523-03 & 003644542-sec & 1:1 & 55.0 & -13 & -5 & 8.35 & 7.58 & 9.8242E+01 & Direct-PRF & 0\\
003644601-01 & 3511.01 & 3:1 & 71.5 & 17 & -4 & 8.35 & 6.81 & 1.1136E+02 & Direct-PRF & 0\\
003644601-02 & 003644542-sec & 3:1 & 71.5 & 17 & -4 & 8.35 & 6.81 & 1.3641E+02 & Direct-PRF & 0\\
003644601-03 & 3511.01 & 1:1 & 71.5 & 17 & -4 & 8.35 & 6.81 & 3.9656E+02 & Direct-PRF & 0\\
003644601-04 & 003644542-sec & 1:1 & 71.5 & 17 & -4 & 8.35 & 6.81 & 5.0690E+02 & Direct-PRF & 0\\
003644602-01 & 3511.01 & 3:1 & 133.3 & 33 & 5 & 8.35 & 6.79 & 4.9918E+02 & Direct-PRF & 0\\
003644602-02 & 003644601-01 & 1:1 & 72.4 & 16 & 9 & 15.16 & -0.02 & 5.5705E+00 & Direct-PRF & 1\\
003644649-01 & 3511.01 & 3:1 & 210.5 & 52 & 9 & 8.35 & 6.06 & 7.1193E+02 & Direct-PRF & 0\\
003644653-01 & 3511.01 & 1:1 & 105.4 & 25 & -10 & 8.35 & 7.55 & 1.9582E+02 & Direct-PRF & 0\\
003644653-02 & 003644542-sec & 1:1 & 105.4 & 25 & -10 & 8.35 & 7.55 & 2.0429E+02 & Direct-PRF & 0\\
003644738-02 & 003644542-sec & 3:1 & 161.6 & 17 & -37 & 8.35 & 7.01 & 4.1993E+02 & Direct-PRF & 0\\
003655332-01 & 6348.01 & 1:1 & 4.2 & -1 & 0 & 14.21 & -0.36 & 3.7206E+00 & Direct-PRF & 0\\
003732894-01 & 6364.01 & 1:1 & 155.0 & 24 & -31 & 7.57 & 6.73 & 1.1229E+03 & Direct-PRF & 0\\
003732972-01 & 6364.01 & 1:1 & 133.6 & -1 & -33 & 7.57 & 5.68 & 1.1410E+03 & Direct-PRF & 0\\
003735634-01 & 3544.01 & 1:1 & 6.8 & 0 & -2 & 16.14 & -2.23 & 8.6147E+01 & Direct-PRF & 0\\
003834360-01 & 6362.01 & 1:1 & 11.4 & 0 & -3 & 14.66 & 0.06 & 1.8761E+02 & Direct-PRF & 0\\
003836375-01 & 6363.01 & 1:1 & 40.3 & 9 & 5 & 13.76 & 2.21 & 1.2258E+02 & Direct-PRF & 0\\
003836399-01 & 6363.01 & 1:1 & 13.0 & 2 & 3 & 13.76 & 0.69 & 1.3314E+02 & Direct-PRF & 0\\
003836413-01 & 6364.01 & 1:1 & 27.2 & 7 & 0 & 7.57 & 6.19 & 1.6274E+00 & Direct-PRF & 0\\
003836413-02 & 6364.01 & 1:2 & 27.2 & 7 & 0 & 7.57 & 6.19 & 4.0676E+00 & Direct-PRF & 0\\
003836439-01 & 6363.01 & 1:1 & 27.2 & -7 & 0 & 13.76 & -6.19 & 1.0533E+00 & Direct-PRF & 1\\
003836439-02 & 6363.01 & 1:2 & 27.2 & -7 & 0 & 13.76 & -6.19 & 1.4627E+02 & Direct-PRF & 1\\
003836450-01 & 6364.01 & 1:1 & 118.2 & -19 & 23 & 7.57 & 5.76 & 1.4437E+03 & Direct-PRF & 0\\
003836453-01 & 6363.01 & 1:1 & 38.9 & -4 & -9 & 13.76 & -1.70 & 5.5758E+02 & Direct-PRF & 0\\
003836453-02 & 6363.01 & 1:2 & 38.9 & -4 & -9 & 13.76 & -1.70 & 3.9031E+03 & Direct-PRF & 0\\
003836509-01 & 6363.01 & 1:1 & 98.7 & -25 & -3 & 13.76 & -0.20 & 2.0043E+02 & Direct-PRF & 0\\
003836522-01 & 6363.01 & 1:1 & 110.5 & -16 & -23 & 13.76 & 1.08 & 2.0715E+02 & Direct-PRF & 0\\
003836558-01 & 6364.01 & 1:1 & 126.6 & -18 & -26 & 7.57 & 7.04 & 5.9445E+02 & Direct-PRF & 0\\
003838486-01 & 3700.01 & 1:1 & 10.1 & 2 & 1 & 17.90 & -2.06 & 7.2595E+02 & Direct-PRF & 0\\
003848665-01 & 003644542-sec & 3:1 & 993.1 & -250 & 2 & 8.35 & 6.61 & 6.5746E+01 & Direct-PRF & 0\\
003848665-02 & 3511.01 & 1:1 & 993.1 & -250 & 2 & 8.35 & 6.61 & 1.6277E+02 & Direct-PRF & 0\\
003851134-01 & 003954798-pri & 1:1 & 221.1 & 56 & -1 & 13.61 & -0.13 & 3.3850E+04 & Col-Anomaly & 0\\
003851194-01 & 003954798-pri & 1:1 & 317.7 & 80 & 1 & 13.61 & 0.21 & 2.9788E+04 & Col-Anomaly & 0\\
003858804-01 & 003858884-01 & 1:1 & 65.2 & 11 & -12 & 9.28 & 4.50 & 6.8013E+02 & Direct-PRF & 0\\
003858804-02 & 003858884-02 & 1:1 & 65.2 & 11 & -12 & 9.28 & 4.50 & 7.0975E+02 & Direct-PRF & 0\\
003858824-01 & 003858884-01 & 1:1 & 61.1 & 14 & -7 & 9.28 & 6.07 & 2.0544E+02 & Direct-PRF & 0\\
003858824-02 & 003858884-02 & 1:1 & 61.1 & 14 & -7 & 9.28 & 6.07 & 2.1405E+02 & Direct-PRF & 0\\
003858851-01 & 003858884-01 & 1:1 & 54.6 & 14 & -1 & 9.28 & 6.49 & 7.8704E+01 & Direct-PRF & 0\\
003858851-02 & 003858884-02 & 1:1 & 54.6 & 14 & -1 & 9.28 & 6.49 & 8.8463E+01 & Direct-PRF & 0\\
003858879-01 & 003858884-01 & 1:1 & 46.4 & 11 & 6 & 9.28 & 5.84 & 1.4014E+02 & Direct-PRF & 0\\
003858879-02 & 003858884-02 & 1:1 & 46.4 & 11 & 6 & 9.28 & 5.84 & 1.4944E+02 & Direct-PRF & 0\\
003858917-01 & 003858884-01 & 1:1 & 33.0 & -8 & 1 & 9.28 & 5.41 & 1.2026E+02 & Direct-PRF & 0\\
003858917-02 & 003858884-02 & 1:1 & 33.0 & -8 & 1 & 9.28 & 5.41 & 1.2496E+02 & Direct-PRF & 0\\
003858919-01 & 003858884-02 & 1:1 & 97.7 & -23 & -7 & 9.28 & 6.72 & 6.9512E+02 & Direct-PRF & 0\\
003858919-02 & 003858884-01 & 1:1 & 97.7 & -23 & -7 & 9.28 & 6.72 & 7.8149E+02 & Direct-PRF & 0\\
003858943-01 & 003858884-01 & 1:1 & 96.4 & -24 & -3 & 9.28 & 4.54 & 3.1383E+03 & Direct-PRF & 0\\
003858949-01 & 003858884-01 & 1:1 & 43.0 & -5 & 10 & 9.28 & 5.30 & 4.1560E+02 & Direct-PRF & 0\\
003858949-02 & 003858884-02 & 1:1 & 43.0 & -5 & 10 & 9.28 & 5.30 & 4.2675E+02 & Direct-PRF & 0\\
003858988-01 & 003858884-01 & 1:1 & 90.4 & -20 & 11 & 9.28 & 5.72 & 2.5241E+02 & Direct-PRF & 0\\
003858988-02 & 003858884-02 & 1:1 & 90.4 & -20 & 11 & 9.28 & 5.72 & 2.4844E+02 & Direct-PRF & 0\\
003859042-01 & 003858884-02 & 1:1 & 191.4 & -48 & 5 & 9.28 & 6.63 & 1.0875E+03 & Direct-PRF & 0\\
003859151-01 & 003858884-01 & 1:1 & 194.1 & -11 & 48 & 9.28 & 5.60 & 2.6930E+03 & Direct-PRF & 0\\
003859151-02 & 003858884-02 & 1:1 & 194.1 & -11 & 48 & 9.28 & 5.60 & 2.4430E+03 & Direct-PRF & 0\\
003861611-01 & 003861595-pri & 1:1 & 11.7 & -1 & 3 & 11.43 & 4.42 & 2.6071E+00 & Direct-PRF & 0\\
003954211-01 & 3766.01 & 1:1 & 8.6 & 1 & 2 & 15.98 & -0.31 & 3.7287E+02 & Direct-PRF & 0\\
003955866-03 & 003955867-02 & 12:1 & 17.9 & 3 & 3 & 13.55 & 1.34 & 4.9364E+00 & Direct-PRF & 0\\
003962684-01 & 003858884-01 & 1:1 & 108.6 & 27 & 6 & 9.28 & 4.68 & 2.9743E+03 & Direct-PRF & 0\\
003962728-01 & 003858884-01 & 1:1 & 141.9 & 32 & 17 & 9.28 & 6.47 & 1.3154E+03 & Direct-PRF & 0\\
003962728-02 & 003858884-02 & 1:1 & 141.9 & 32 & 17 & 9.28 & 6.47 & 1.5394E+03 & Direct-PRF & 0\\
003962872-01 & 003858884-01 & 1:1 & 213.5 & 31 & 45 & 9.28 & 4.87 & 4.5811E+03 & Direct-PRF & 0\\
003962872-02 & 003858884-02 & 1:1 & 213.5 & 31 & 45 & 9.28 & 4.87 & 3.9662E+03 & Direct-PRF & 0\\
003964562-01 & 3542.01 & 1:1 & 9.4 & -2 & 2 & 14.78 & -2.37 & 1.8818E+02 & Direct-PRF & 0\\
003964562-02 & 003964545-02 & 1:1 & 9.4 & -2 & 2 & 14.78 & -2.37 & 1.6824E+02 & Direct-PRF & 0\\
004035667-01 & 6107.01 & 1:1 & 13.7 & 1 & -3 & 12.70 & -2.67 & 2.7059E+02 & Direct-PRF & 0\\
004037164-01 & 004037163-pri & 1:1 & 6.4 & -1 & 2 & 16.68 & -1.24 & 2.2796E+02 & Direct-PRF & 0\\
004037164-02 & 3793.01 & 1:1 & 6.4 & -1 & 2 & 16.68 & -1.24 & 3.4531E+02 & Direct-PRF & 0\\
004049108-01 & 5994.01 & 1:1 & 11.7 & 2 & -2 & 14.65 & 0.22 & 1.9398E+02 & Direct-PRF & 0\\
004055774-01 & 5025.01 & 1:1 & 19.6 & -4 & -3 & 14.04 & 1.54 & 6.5618E+02 & Direct-PRF & 0\\
004059887-01 & 5045.01 & 1:1 & 459.4 & 115 & 1 & 14.30 & -1.39 & 2.3604E+04 & Col-Anomaly & 0\\
004076976-01 & 6385.01 & 1:2 & 19.5 & -3 & -3 & 13.77 & 0.43 & 2.2617E+03 & Direct-PRF & 0\\
004079535-01 & 3594.01 & 1:1 & 6.2 & 1 & -1 & 15.56 & -0.48 & 8.9777E+00 & Direct-PRF & 0\\
004144231-01 & 6109.01 & 1:1 & 15.7 & -2 & 3 & 11.86 & 3.61 & 4.3377E+01 & Direct-PRF & 0\\
004144238-01 & 6109.01 & 1:1 & 25.2 & 3 & -6 & 11.86 & 1.90 & 7.2816E+02 & Direct-PRF & 0\\
004150496-01 & 004150611-01 & 1:1 & 98.0 & 24 & -7 & 7.90 & 7.64 & 1.4164E+02 & Direct-PRF & 0\\
004150496-02 & 004150611-02 & 1:1 & 98.0 & 24 & -7 & 7.90 & 7.64 & 1.3436E+02 & Direct-PRF & 0\\
004150496-03 & 3156.04 & 1:1 & 98.0 & 24 & -7 & 7.90 & 7.64 & 1.1258E+02 & Direct-PRF & 0\\
004150539-01 & 004150611-01 & 1:1 & 50.1 & 11 & -6 & 7.90 & 7.80 & 5.4684E+01 & Direct-PRF & 0\\
004150539-02 & 004150611-02 & 1:1 & 50.1 & 11 & -6 & 7.90 & 7.80 & 5.3930E+01 & Direct-PRF & 0\\
004150539-03 & 3156.04 & 1:1 & 50.1 & 11 & -6 & 7.90 & 7.80 & 5.0114E+01 & Direct-PRF & 0\\
004150624-01 & 004150611-02 & 1:1 & 69.4 & 14 & 11 & 7.90 & 7.56 & 8.5404E+01 & Direct-PRF & 0\\
004150624-02 & 004150611-01 & 1:1 & 69.4 & 14 & 11 & 7.90 & 7.56 & 9.0599E+01 & Direct-PRF & 0\\
004150624-03 & 3156.04 & 1:1 & 69.4 & 14 & 11 & 7.90 & 7.56 & 8.5571E+01 & Direct-PRF & 0\\
004150701-01 & 004150611-02 & 1:1 & 97.5 & -24 & 1 & 7.90 & 7.96 & 1.2086E+02 & Direct-PRF & 0\\
004150701-02 & 004150611-01 & 1:1 & 97.5 & -24 & 1 & 7.90 & 7.96 & 1.4446E+02 & Direct-PRF & 0\\
004150703-01 & 004150611-02 & 1:1 & 96.6 & -24 & 3 & 7.90 & 6.92 & 4.7083E+02 & Direct-PRF & 0\\
004169315-02 & 004847832-02 & 12:1 & 3147.8 & -7 & 2 & 12.45 & 2.30 & 4.0671E+02 & Cross-Talk & 0\\
004245861-01 & 004245897-pri & 1:1 & 59.0 & 6 & -13 & 12.54 & 3.36 & 2.6651E+03 & Direct-PRF & 0\\
004245933-01 & 004245897-pri & 1:1 & 34.7 & -9 & 1 & 12.54 & 3.29 & 1.1957E+03 & Direct-PRF & 0\\
004245945-01 & 004245897-pri & 1:1 & 47.3 & -6 & 11 & 12.54 & 2.67 & 3.2072E+03 & Direct-PRF & 0\\
004247807-01 & 28.01 & 1:2 & 13.9 & -4 & -1 & 11.26 & 3.55 & 1.6614E+01 & Direct-PRF & 0\\
004247811-01 & 28.01 & 1:2 & 44.7 & -10 & -6 & 11.26 & 3.09 & 2.3473E+03 & Direct-PRF & 0\\
004284980-01 & 6112.01 & 1:1 & 53.4 & 13 & 6 & 12.79 & 2.81 & 2.9492E+03 & Direct-PRF & 0\\
004285107-01 & 6112.01 & 1:1 & 19.0 & 2 & -4 & 12.79 & 1.20 & 1.0644E+03 & Direct-PRF & 0\\
004349442-02 & 244.01 & 1:1 & 8.4 & 1 & -1 & 10.73 & 2.53 & 4.3077E+00 & Direct-PRF & 0\\
004349442-03 & 244.02 & 1:1 & 8.4 & 1 & -1 & 10.73 & 2.53 & 3.7315E+00 & Direct-PRF & 0\\
004356621-01 & 004356766-01 & 1:1 & 251.7 & 63 & 1 & 15.45 & -0.43 & 1.1192E+03 & Col-Anomaly & 0\\
004357985-01 & 004150611-01 & 1:1 & 712.6 & 180 & 0 & 7.90 & 7.52 & 1.7705E+02 & Direct-PRF & 0\\
004365442-01 & 5058.01 & 1:1 & 19.0 & -5 & 1 & 13.31 & -0.01 & 2.2547E+03 & Direct-PRF & 0\\
004372768-01 & 3698.01 & 1:1 & 9.1 & -1 & 1 & 18.23 & -2.32 & 4.7775E+02 & Direct-PRF & 0\\
004373195-01 & V1130-Cyg-pri & 1:1 & 1112.4 & 280 & 0 & 12.32 & -3.20 & 2.0063E+05 & Col-Anomaly & 0\\
004376629-01 & 397.01 & 1:1 & 9.5 & 1 & -2 & 13.77 & -0.09 & 4.6789E+01 & Direct-PRF & 0\\
004380560-01 & 004380558-01 & 1:1 & 4.3 & -1 & 0 & 14.42 & 0.64 & 1.2444E+00 & Direct-PRF & 0\\
004386059-01 & 3659.01 & 1:1 & 10.6 & -1 & -3 & 16.94 & -3.06 & 1.7086E+03 & Direct-PRF & 0\\
004458984-01 & 004458989-pri & 1:1 & 23.1 & -4 & -4 & 12.95 & 3.02 & 1.7779E+03 & Direct-PRF & 0\\
004474645-01 & 3829.01 & 1:1 & 4.6 & 1 & 1 & 16.81 & -2.61 & 1.1343E+02 & Direct-PRF & 0\\
004482738-01 & 004579598-02 & 1:1 & 136.2 & -34 & -2 & 13.79 & -0.84 & 3.0233E-01 & Direct-PRF & 1\\
004482738-02 & 4414.01 & 1:1 & 136.2 & -34 & -2 & 13.79 & -0.84 & 1.4524E+00 & Direct-PRF & 1\\
004484312-01 & 6112.01 & 1:1 & 1125.9 & 284 & 1 & 12.79 & 0.40 & 8.8475E+03 & Col-Anomaly & 0\\
004544571-01 & 004544587-pri & 1:1 & 28.2 & 4 & -5 & 10.80 & 4.95 & 5.6482E+02 & Direct-PRF & 0\\
004544571-02 & 004544587-sec & 1:1 & 28.2 & 4 & -5 & 10.80 & 4.95 & 8.5714E+02 & Direct-PRF & 0\\
004544572-01 & 004544587-pri & 1:1 & 36.6 & 1 & -9 & 10.80 & 4.94 & 1.0203E+03 & Direct-PRF & 0\\
004544572-02 & 004544587-sec & 1:1 & 36.6 & 1 & -9 & 10.80 & 4.94 & 1.9401E+03 & Direct-PRF & 0\\
004544572-03 & 004544571-03 & 1:1 & 17.1 & -3 & -4 & 15.75 & -0.01 & 1.0314E+00 & Direct-PRF & 0\\
004544620-01 & 004544587-pri & 1:1 & 52.0 & -1 & 13 & 10.80 & 5.07 & 9.7795E+02 & Direct-PRF & 0\\
004544620-02 & 004544587-sec & 1:1 & 52.0 & -1 & 13 & 10.80 & 5.07 & 1.2510E+03 & Direct-PRF & 0\\
004544623-01 & 004544587-pri & 1:1 & 43.7 & -11 & 0 & 10.80 & 5.20 & 3.6623E+02 & Direct-PRF & 0\\
004544623-02 & 004544587-sec & 1:1 & 43.7 & -11 & 0 & 10.80 & 5.20 & 8.2046E+01 & Direct-PRF & 0\\
004544684-01 & 004544587-pri & 1:1 & 120.9 & -15 & 27 & 10.80 & 4.12 & 5.1483E+03 & Direct-PRF & 0\\
004568117-01 & V1130-Cyg-pri & 1:1 & 88.9 & 2 & -22 & 12.32 & 1.22 & 2.4076E+04 & Direct-PRF & 0\\
004568298-01 & V1130-Cyg-pri & 1:1 & 99.0 & 25 & 3 & 12.32 & 3.63 & 4.5598E+03 & Direct-PRF & 0\\
004570931-01 & 1658.01 & 1:1 & 9.6 & 0 & -2 & 13.31 & 0.34 & 5.9150E+01 & Direct-PRF & 0\\
004570949-02 & 1343.01 & 1:2 & 9.6 & 0 & 2 & 13.64 & -0.34 & 1.7432E+00 & Direct-PRF & 0\\
004570949-03 & 1343.01 & 1:1 & 9.6 & 0 & 2 & 13.64 & -0.34 & 2.8043E+00 & Direct-PRF & 0\\
004574319-01 & 6427.01 & 1:1 & 47.1 & -11 & 4 & 13.24 & 2.52 & 5.1912E+03 & Direct-PRF & 0\\
004579313-01 & 3657.01 & 1:1 & 7.3 & -1 & 2 & 17.39 & -2.58 & 5.1174E+02 & Direct-PRF & 0\\
004579313-02 & 3657.01 & 1:2 & 7.3 & -1 & 2 & 17.39 & -2.58 & 1.2909E+03 & Direct-PRF & 0\\
004579598-01 & 004482738-02 & 1:1 & 136.2 & 34 & 2 & 12.95 & 0.84 & 2.1538E+00 & Direct-PRF & 1\\
004579598-02 & 004482738-01 & 1:1 & 136.2 & 34 & 2 & 12.95 & 0.84 & 3.3077E+00 & Direct-PRF & 1\\
004586468-01 & 004586482-01 & 1:1 & 6.0 & 1 & 0 & 14.02 & 0.48 & 2.4832E+00 & Direct-PRF & 0\\
004586468-02 & 5073.01 & 1:1 & 6.0 & 1 & 0 & 14.02 & 0.48 & 2.6867E+00 & Direct-PRF & 0\\
004636565-01 & 004445630-01 & 1:1 & 1217.5 & 306 & 0 & 13.86 & -1.35 & 1.1296E+04 & Col-Anomaly & 0\\
004647662-01 & 004647652-pri & 1:1 & 47.3 & 9 & 8 & 11.81 & 2.96 & 3.0771E+03 & Direct-PRF & 0\\
004659405-01 & 3691.01 & 1:1 & 9.9 & 2 & -1 & 16.03 & -2.10 & 1.8632E+02 & Direct-PRF & 0\\
004659405-02 & 004751083-02 & 1:1 & 9.9 & 2 & -1 & 16.03 & -2.10 & 1.4663E+02 & Direct-PRF & 0\\
004665991-01 & 004665989-pri & 1:2 & 35.6 & -8 & -4 & 13.02 & 1.65 & 7.2025E+03 & Direct-PRF & 0\\
004666008-01 & 004665989-pri & 1:1 & 19.3 & 4 & -3 & 13.02 & 1.42 & 1.0180E+03 & Direct-PRF & 0\\
004666008-02 & 6433.01 & 2:1 & 19.3 & 4 & -3 & 13.02 & 1.42 & 2.0391E+03 & Direct-PRF & 0\\
004677282-01 & 004677321-pri & 1:1 & 19.3 & 4 & -3 & 13.48 & -0.32 & 1.2909E+03 & Direct-PRF & 0\\
004678873-01 & 004678875-01 & 1:1 & 4.9 & -1 & -1 & 13.24 & -0.52 & 9.6042E+00 & Direct-PRF & 0\\
004678919-01 & 004678875-01 & 1:1 & 29.3 & 2 & 7 & 13.24 & 0.45 & 6.0264E+03 & Direct-PRF & 0\\
004739565-01 & 004739791-pri & 1:1 & 353.3 & 89 & 0 & 14.70 & -0.53 & 5.7643E+03 & Col-Anomaly & 0\\
004740688-01 & 004740676-pri & 1:1 & 19.3 & 2 & 4 & 13.20 & 2.53 & 6.7000E+02 & Direct-PRF & 0\\
004743513-01 & 3572.01 & 1:1 & 4.3 & 0 & -1 & 14.55 & -1.59 & 1.7207E+01 & Direct-PRF & 0\\
004743513-02 & 004743508-02 & 1:1 & 4.3 & 0 & -1 & 14.55 & -1.59 & 7.7946E+00 & Direct-PRF & 0\\
004756776-05 & 011341164-01 & 6:1 & 39157.3 & 136 & 359 & 12.37 & -1.08 & 4.5238E-01 & Reflection & 1\\
004768756-01 & 6134.01 & 1:1 & 8066.6 & -2 & 11 & 11.94 & 0.69 & 1.6018E+04 & Cross-Talk & 0\\
004769824-01 & 5086.01 & 1:1 & 22.7 & -6 & 1 & 10.95 & 4.46 & 9.1836E+01 & Direct-PRF & 0\\
004769931-01 & 004678875-01 & 1:1 & 448.1 & 112 & 1 & 13.24 & 0.66 & 6.4638E+03 & Col-Anomaly & 0\\
004832175-01 & 004832197-pri & 1:2 & 18.2 & 3 & 4 & 11.51 & 4.25 & 5.5140E+01 & Direct-PRF & 0\\
004832225-02 & 004832197-pri & 1:1 & 39.0 & -10 & -1 & 11.51 & -2.44 & 4.0690E+02 & Direct-PRF & 0\\
004833135-01 & 004150611-01 & 43:1 & 4253.7 & 4 & -1 & 7.90 & 6.76 & 8.7991E+01 & Cross-Talk & 0\\
004833135-02 & 1334.02 & 2:1 & 4212.3 & -10 & -12 & 15.45 & -0.79 & 1.6925E+00 & Col-Anomaly & 1\\
004833135-03 & 1330.01 & 43:1 & 4280.3 & -7 & 5 & 15.70 & -1.04 & 1.5093E+00 & Col-Anomaly & 1\\
004847782-01 & 004847832-01 & 1:1 & 34.8 & -6 & 7 & 12.45 & 2.63 & 1.3376E+03 & Direct-PRF & 0\\
004847782-02 & 004847832-02 & 1:1 & 34.8 & -6 & 7 & 12.45 & 2.63 & 9.6869E+02 & Direct-PRF & 0\\
004847843-01 & 004847832-02 & 1:1 & 17.4 & -2 & -3 & 12.45 & 0.96 & 7.8501E+02 & Direct-PRF & 0\\
004847843-02 & 004847832-01 & 1:1 & 17.4 & -2 & -3 & 12.45 & 0.96 & 8.5001E+02 & Direct-PRF & 0\\
004848321-01 & 004848423-01 & 1:1 & 87.0 & -21 & 5 & 11.82 & 3.20 & 5.5610E+03 & Direct-PRF & 0\\
004848424-01 & 004848423-01 & 1:1 & 83.1 & -18 & -11 & 11.82 & 2.94 & 4.3651E+03 & Direct-PRF & 0\\
004848532-01 & 3560.01 & 1:1 & 80.3 & 2 & -21 & 11.82 & 3.11 & 3.7486E+03 & Direct-PRF & 0\\
004850843-01 & 004938893-01 & 1:1 & 243.4 & -61 & -2 & 15.47 & -0.23 & 1.2955E+00 & Col-Anomaly & 1\\
004851072-01 & 004851217-pri & 1:2 & 124.2 & 31 & 2 & 11.11 & 3.88 & 5.0769E+03 & Direct-PRF & 0\\
004851089-01 & 004851217-01 & 1:1 & 110.0 & 27 & 1 & 11.11 & 4.44 & 1.3219E+02 & Direct-PRF & 0\\
004851145-01 & 004851217-01 & 1:1 & 90.8 & 22 & -2 & 11.11 & 4.53 & 1.0299E+02 & Direct-PRF & 0\\
004851239-01 & 004851217-pri & 1:2 & 77.6 & -19 & 6 & 11.11 & 0.33 & 1.8000E+04 & Direct-PRF & 0\\
004851283-01 & 004851217-01 & 1:1 & 49.2 & -10 & -8 & 11.11 & 0.80 & 5.6057E+01 & Direct-PRF & 0\\
004851338-01 & 004851217-pri & 1:2 & 95.9 & 2 & -24 & 11.11 & 3.90 & 3.6000E+03 & Direct-PRF & 0\\
004851356-01 & 004851217-01 & 1:1 & 97.1 & -2 & -24 & 11.11 & 3.60 & 2.1602E+02 & Direct-PRF & 0\\
004861527-01 & 004773155-01 & 1:1 & 22.2 & 5 & 2 & 13.59 & 0.27 & 1.5719E+03 & Direct-PRF & 0\\
004861527-02 & 004773155-02 & 1:1 & 22.2 & 5 & 2 & 13.59 & 0.27 & 1.6773E+03 & Direct-PRF & 0\\
004861791-01 & 4278.01 & 1:2 & 16.5 & -4 & -1 & 15.99 & -0.04 & 2.1841E+00 & Direct-PRF & 0\\
004913000-01 & 5997.01 & 1:1 & 9.3 & 2 & 0 & 11.30 & 0.37 & 5.0028E+01 & Direct-PRF & 0\\
004914399-01 & 6121.01 & 1:1 & 255.5 & 64 & 0 & 13.82 & 0.64 & 6.6967E+02 & Col-Anomaly & 0\\
004914709-01 & 004150611-01 & 1:1 & 3293.4 & 829 & 0 & 7.90 & 7.74 & 1.3199E+02 & Col-Anomaly & 0\\
004914709-02 & 004150611-02 & 1:1 & 3293.4 & 829 & 0 & 7.90 & 7.74 & 1.9477E+02 & Col-Anomaly & 0\\
004914737-01 & 004150611-02 & 1:1 & 3255.1 & 819 & 0 & 7.90 & 7.21 & 3.8954E+02 & Col-Anomaly & 0\\
004914737-02 & 004150611-01 & 1:1 & 3255.1 & 819 & 0 & 7.90 & 7.21 & 2.5360E+02 & Col-Anomaly & 0\\
004932689-01 & 6474.01 & 1:1 & 16.9 & -4 & 2 & 13.63 & 1.93 & 4.8591E+02 & Direct-PRF & 0\\
004938893-01 & 004850843-01 & 1:1 & 243.4 & 61 & 2 & 15.24 & 0.23 & 7.7193E-01 & Col-Anomaly & 1\\
004946049-01 & 004678875-01 & 1:1 & 1061.1 & 267 & 0 & 13.24 & -0.29 & 2.8625E+04 & Col-Anomaly & 0\\
004949769-01 & 004949770-pri & 1:1 & 13.7 & 3 & 2 & 12.57 & 2.35 & 1.5689E+02 & Direct-PRF & 0\\
004949795-01 & 004949770-pri & 1:1 & 23.9 & -6 & 1 & 12.57 & 2.34 & 2.9435E+03 & Direct-PRF & 0\\
004949801-01 & 004949770-pri & 1:1 & 40.8 & 6 & 8 & 12.57 & 3.04 & 1.7359E+03 & Direct-PRF & 0\\
004949825-01 & 004949770-pri & 1:1 & 30.0 & -4 & 7 & 12.57 & 2.54 & 3.6595E+03 & Direct-PRF & 0\\
005020044-01 & 3688.01 & 1:1 & 6.9 & 0 & -1 & 15.81 & -1.98 & 1.3573E+02 & Direct-PRF & 0\\
005021176-01 & 3679.01 & 1:1 & 7.3 & 1 & 1 & 17.70 & -2.84 & 5.3096E+02 & Direct-PRF & 0\\
005021176-02 & 3679.01 & 1:2 & 7.3 & 1 & 1 & 17.70 & -2.84 & 3.6497E+03 & Direct-PRF & 0\\
005021737-01 & 005021732-01 & 1:1 & 4.5 & 0 & -1 & 13.62 & -1.63 & 1.1667E+01 & Direct-PRF & 0\\
005021737-02 & 005021732-sec & 1:1 & 4.5 & 0 & -1 & 13.62 & -1.63 & 8.6088E+00 & Direct-PRF & 0\\
005023956-01 & 3570.01 & 1:1 & 8.9 & 2 & 0 & 15.05 & -0.44 & 4.4367E+01 & Direct-PRF & 0\\
005024126-01 & 4286.01 & 1:1 & 20.5 & -3 & 4 & 14.96 & 0.66 & 2.8167E+00 & Direct-PRF & 0\\
005024177-01 & 6493.01 & 1:1 & 20.5 & 3 & -4 & 15.63 & -0.66 & 1.0139E+01 & Direct-PRF & 0\\
005024414-01 & 1544.01 & 1:1 & 12.4 & -1 & 3 & 15.06 & -2.36 & 4.9112E+02 & Direct-PRF & 0\\
005024429-01 & 1544.01 & 1:1 & 14.8 & -4 & 1 & 15.06 & -0.12 & 1.6587E+02 & Direct-PRF & 0\\
005024482-01 & 1544.01 & 1:1 & 11.7 & 1 & -2 & 15.06 & -2.86 & 3.7384E+02 & Direct-PRF & 0\\
005036480-01 & 6504.01 & 1:1 & 35.2 & -1 & -8 & 13.35 & 1.86 & 3.0914E+03 & Direct-PRF & 0\\
005036516-01 & 6504.01 & 1:1 & 6.7 & 0 & -1 & 13.35 & 0.99 & 1.0541E+01 & Direct-PRF & 0\\
005036537-01 & 6504.01 & 1:1 & 11.7 & -3 & -1 & 13.35 & 2.21 & 6.3299E+01 & Direct-PRF & 0\\
005041847-02 & 005041843-pri & 2:1 & 6.1 & 1 & -2 & 17.03 & -2.45 & 3.1028E+01 & Direct-PRF & 0\\
005078025-01 & 005077994-sec & 1:1 & 34.3 & 8 & -4 & 12.67 & 2.37 & 2.7361E+03 & Direct-PRF & 0\\
005078025-02 & 005077994-pri & 1:1 & 34.3 & 8 & -4 & 12.67 & 2.37 & 3.2264E+03 & Direct-PRF & 0\\
005088084-05 & 005521373-02 & 1:1 & 2409.4 & 606 & 1 & 12.55 & 2.37 & 5.3724E-02 & Col-Anomaly & 1\\
005088308-03 & 2708.01 & 1:1 & 535.1 & 76 & -111 & 15.90 & -7.21 & 7.9118E+00 & Direct-PRF & 1\\
005097454-01 & 005097446-01 & 1:1 & 9.5 & 0 & -2 & 13.89 & 1.42 & 9.0004E+01 & Direct-PRF & 0\\
005097470-01 & 005097446-01 & 1:1 & 23.2 & -5 & -2 & 13.89 & 0.60 & 5.1792E+03 & Direct-PRF & 0\\
005114623-01 & 6371.01 & 14:1 & 7285.7 & 9 & 0 & 9.28 & 6.08 & 7.5484E+01 & Cross-Talk & 0\\
005114623-02 & 003858884-01 & 14:1 & 7285.7 & 9 & 0 & 9.28 & 6.08 & 7.5959E+01 & Cross-Talk & 0\\
005114623-03 & 6371.01 & 14:1 & 7285.7 & 9 & 0 & 9.28 & 6.08 & 7.7555E+01 & Cross-Talk & 0\\
005114623-04 & 003858884-sec & 15:1 & 7285.7 & 9 & 0 & 9.28 & 6.08 & 8.4592E+01 & Cross-Talk & 0\\
005114623-05 & 003858884-02 & 15:1 & 7285.7 & 9 & 0 & 9.28 & 6.08 & 9.0675E+01 & Cross-Talk & 0\\
005114623-07 & 003858884-sec & 15:1 & 7285.7 & 9 & 0 & 9.28 & 6.08 & 1.0551E+02 & Cross-Talk & 0\\
005128966-01 & 005128972-pri & 1:1 & 4.8 & 2 & 0 & 13.24 & 1.22 & 1.5866E+02 & Direct-PRF & 0\\
005130369-01 & 3707.01 & 1:1 & 5.9 & 0 & 1 & 16.30 & -2.45 & 6.3227E+01 & Direct-PRF & 0\\
005130369-02 & 005130380-02 & 1:1 & 5.9 & 0 & 1 & 16.30 & -2.45 & 3.7250E+01 & Direct-PRF & 0\\
005175986-01 & 005088308-03 & 1:1 & 535.1 & -76 & 111 & 8.69 & 7.21 & 7.3913E-01 & Direct-PRF & 1\\
005181817-01 & 3638.01 & 1:1 & 9.9 & 0 & -2 & 15.93 & -2.72 & 2.9883E+02 & Direct-PRF & 0\\
005193386-01 & 005193384-01 & 1:1 & 8.2 & -1 & 1 & 19.07 & -5.07 & 1.2684E+00 & Direct-PRF & 0\\
005193386-02 & 3637.01 & 1:1 & 8.2 & -1 & 1 & 19.07 & -5.07 & 3.7827E+00 & Direct-PRF & 0\\
005193400-01 & 005193384-01 & 1:1 & 16.6 & 4 & 2 & 19.07 & -3.38 & 7.3593E+02 & Direct-PRF & 0\\
005193400-02 & 3637.01 & 1:1 & 16.6 & 4 & 2 & 19.07 & -3.38 & 1.6602E+03 & Direct-PRF & 0\\
005201115-01 & 005288543-01 & 1:1 & 351.4 & 88 & 0 & 13.59 & -0.72 & 5.7927E+03 & Col-Anomaly & 0\\
005201593-01 & 005201619-pri & 1:1 & 21.3 & 1 & 5 & 13.05 & 0.59 & 1.5708E+04 & Direct-PRF & 0\\
005201596-01 & 005201619-pri & 1:1 & 50.2 & 8 & 9 & 13.05 & 1.98 & 1.4544E+04 & Direct-PRF & 0\\
005201676-01 & 005201619-pri & 1:1 & 57.4 & 14 & -1 & 13.05 & 1.53 & 1.8700E+04 & Direct-PRF & 0\\
005201695-01 & 005201619-pri & 1:1 & 51.7 & 3 & -12 & 13.05 & 2.63 & 6.8895E+03 & Direct-PRF & 0\\
005215980-01 & 005215999-pri & 1:1 & 8.6 & 1 & 1 & 14.11 & 1.10 & 2.4950E+02 & Direct-PRF & 0\\
005217891-01 & 005217733-pri & 1:1 & 98.9 & -18 & -17 & 7.39 & 8.26 & 9.2910E+01 & Direct-PRF & 0\\
005264888-01 & 005264818-pri & 1:1 & 85.1 & 21 & 6 & 8.86 & 6.41 & 6.9211E+02 & Direct-PRF & 0\\
005272571-01 & 005097446-01 & 1:1 & 975.9 & 245 & 1 & 13.89 & -1.41 & 1.8598E+04 & Col-Anomaly & 0\\
005282051-01 & 1545.01 & 1:1 & 8.3 & -2 & 1 & 15.17 & -0.89 & 7.3631E+01 & Direct-PRF & 0\\
005282477-02 & 4560.01 & 1:1 & 37.7 & -4 & 9 & 15.11 & -0.07 & 3.4438E+01 & Direct-PRF & 0\\
005288570-01 & 005288543-01 & 1:1 & 23.9 & -1 & -6 & 13.59 & -0.60 & 1.6464E+03 & Direct-PRF & 0\\
005288577-01 & 005288543-01 & 1:1 & 25.8 & 0 & -7 & 13.59 & 0.01 & 3.5546E+03 & Direct-PRF & 0\\
005298620-01 & V380-Cyg-pri & 1:1 & 396.0 & -82 & -56 & 5.77 & 9.93 & 1.0579E+03 & Direct-PRF & 0\\
005298620-02 & V380-Cyg-sec & 1:1 & 396.0 & -82 & -56 & 5.77 & 9.93 & 9.0870E+02 & Direct-PRF & 0\\
005303551-01 & 3982.01 & 1:1 & 4.8 & 1 & 0 & 16.49 & -1.61 & 2.3276E+01 & Direct-PRF & 0\\
005305225-01 & 005217733-pri & 2:1 & 203.0 & 50 & 7 & 7.39 & 6.62 & 2.7418E+02 & Direct-PRF & 0\\
005305399-01 & 005217733-pri & 2:1 & 99.7 & 24 & -8 & 7.39 & 7.37 & 1.1941E+02 & Direct-PRF & 0\\
005305404-01 & 005217733-pri & 1:1 & 49.4 & 12 & -2 & 7.39 & 7.33 & 3.5169E+01 & Direct-PRF & 0\\
005305404-02 & 005217733-sec & 1:1 & 49.4 & 12 & -2 & 7.39 & 7.33 & 3.4337E+01 & Direct-PRF & 0\\
005305451-01 & 005217733-pri & 1:1 & 100.2 & 21 & -14 & 7.39 & 8.01 & 4.2059E+01 & Direct-PRF & 0\\
005305451-02 & 005217733-sec & 1:1 & 100.2 & 21 & -14 & 7.39 & 8.01 & 5.2407E+01 & Direct-PRF & 0\\
005305471-01 & 005217733-pri & 1:1 & 52.2 & 8 & -10 & 7.39 & 6.79 & 5.0000E+01 & Direct-PRF & 0\\
005305471-02 & 005217733-sec & 1:1 & 52.2 & 8 & -10 & 7.39 & 6.79 & 4.8679E+01 & Direct-PRF & 0\\
005308387-01 & 3887.01 & 1:2 & 13.8 & 4 & 1 & 13.48 & -0.60 & 6.8621E+00 & Direct-PRF & 0\\
005308419-01 & 2724.01 & 2:1 & 13.8 & -4 & -1 & 12.88 & 0.60 & 1.1277E+00 & Direct-PRF & 0\\
005308419-02 & 2724.01 & 1:1 & 13.8 & -4 & -1 & 12.88 & 0.60 & 1.5143E+00 & Direct-PRF & 0\\
005308663-01 & 2718.01 & 1:1 & 13.5 & -3 & 1 & 13.82 & 1.77 & 2.1814E+00 & Direct-PRF & 0\\
005308666-01 & 1562.01 & 1:1 & 13.5 & 3 & -1 & 15.59 & -1.77 & 8.4000E+00 & Direct-PRF & 0\\
005358212-01 & 005358200-pri & 1:1 & 22.8 & 3 & -5 & 15.01 & -0.01 & 1.8874E+04 & Direct-PRF & 0\\
005376642-01 & 005376552-sec & 1:1 & 66.6 & 13 & -11 & 12.86 & 1.50 & 9.4125E+03 & Direct-PRF & 0\\
005384194-01 & 005384183-02 & 1:1 & 5.5 & 0 & 1 & 13.58 & -1.75 & 1.9400E+01 & Direct-PRF & 0\\
005385139-02 & V380-Cyg-sec & 1:1 & 372.1 & 32 & -87 & 5.77 & 10.07 & 7.5460E+02 & Direct-PRF & 0\\
005385150-01 & V380-Cyg-pri & 1:1 & 368.9 & 28 & -88 & 5.77 & 9.70 & 1.0352E+03 & Direct-PRF & 0\\
005385269-01 & V380-Cyg-pri & 1:1 & 323.9 & 0 & -81 & 5.77 & 8.56 & 1.1880E+03 & Direct-PRF & 0\\
005385410-02 & 5172.01 & 1:1 & 370.7 & -93 & 5 & 15.79 & -2.21 & 3.0172E+00 & Col-Anomaly & 1\\
005385410-03 & V380-Cyg-sec & 1:1 & 318.2 & -31 & -74 & 5.77 & 7.81 & 2.5807E+03 & Direct-PRF & 0\\
005385439-01 & V380-Cyg-pri & 1:1 & 200.5 & 4 & -50 & 5.77 & 8.38 & 8.8374E+02 & Direct-PRF & 0\\
005385439-02 & V380-Cyg-sec & 1:1 & 200.5 & 4 & -50 & 5.77 & 8.38 & 8.8990E+02 & Direct-PRF & 0\\
005385469-01 & 6004.01 & 1:1 & 65.3 & 12 & -12 & 15.54 & -2.45 & 9.8511E+00 & Direct-PRF & 1\\
005385471-01 & V380-Cyg-pri & 1:1 & 166.8 & 15 & -39 & 5.77 & 10.22 & 1.6432E+02 & Direct-PRF & 0\\
005385471-02 & V380-Cyg-sec & 1:1 & 166.8 & 15 & -39 & 5.77 & 10.22 & 1.5271E+02 & Direct-PRF & 0\\
005385491-01 & V380-Cyg-pri & 1:1 & 212.2 & -14 & -51 & 5.77 & 7.81 & 1.3176E+03 & Direct-PRF & 0\\
005385491-02 & V380-Cyg-sec & 1:1 & 212.2 & -14 & -51 & 5.77 & 7.81 & 1.2289E+03 & Direct-PRF & 0\\
005385509-01 & V380-Cyg-pri & 1:1 & 278.5 & -37 & -59 & 5.77 & 9.94 & 4.6010E+02 & Direct-PRF & 0\\
005385509-02 & 005471010-02 & 1:1 & 337.1 & -85 & -1 & 15.64 & 0.07 & 8.9063E-01 & Col-Anomaly & 1\\
005385548-01 & V380-Cyg-pri & 1:1 & 126.7 & 2 & -31 & 5.77 & 7.47 & 9.7928E+02 & Direct-PRF & 0\\
005385548-02 & V380-Cyg-sec & 1:1 & 126.7 & 2 & -31 & 5.77 & 7.47 & 9.6296E+02 & Direct-PRF & 0\\
005385566-01 & V380-Cyg-pri & 1:1 & 350.5 & -62 & -62 & 5.77 & 9.77 & 4.9465E+02 & Direct-PRF & 0\\
005385566-02 & V380-Cyg-sec & 1:1 & 350.5 & -62 & -62 & 5.77 & 9.77 & 4.8510E+02 & Direct-PRF & 0\\
005385575-01 & V380-Cyg-pri & 1:1 & 151.6 & -14 & -35 & 5.77 & 8.88 & 2.8757E+02 & Direct-PRF & 0\\
005385575-02 & V380-Cyg-sec & 1:1 & 151.6 & -14 & -35 & 5.77 & 8.88 & 2.2960E+02 & Direct-PRF & 0\\
005385647-01 & V380-Cyg-sec & 1:1 & 269.9 & -52 & -44 & 5.77 & 8.22 & 1.1029E+03 & Direct-PRF & 0\\
005385667-01 & V380-Cyg-pri & 1:1 & 247.5 & -49 & -38 & 5.77 & 7.45 & 2.2297E+03 & Direct-PRF & 0\\
005385667-02 & 005385509-02 & 1:2 & 99.1 & -12 & 21 & 15.71 & -2.49 & 6.4000E+00 & Direct-PRF & 1\\
005385697-01 & V380-Cyg-pri & 1:1 & 229.0 & -48 & -32 & 5.77 & 9.83 & 3.9491E+02 & Direct-PRF & 0\\
005385697-02 & V380-Cyg-sec & 1:1 & 229.0 & -48 & -32 & 5.77 & 9.83 & 4.1625E+02 & Direct-PRF & 0\\
005385750-01 & 6129.01 & 1:1 & 25.7 & -1 & -6 & 12.70 & 1.79 & 4.8381E+00 & Direct-PRF & 0\\
005385750-02 & 005385838-03 & 3:1 & 89.4 & -6 & -22 & 12.97 & 1.52 & 9.1451E-02 & Direct-PRF & 1\\
005385773-01 & V380-Cyg-pri & 1:1 & 309.9 & -72 & -29 & 5.77 & 8.90 & 1.0816E+03 & Direct-PRF & 0\\
005385773-02 & V380-Cyg-sec & 1:1 & 309.9 & -72 & -29 & 5.77 & 8.90 & 8.7186E+02 & Direct-PRF & 0\\
005385778-01 & 005385792-03 & 1:1 & 22.1 & -4 & -5 & 13.60 & -0.90 & 8.2949E-01 & Direct-PRF & 1\\
005385778-03 & V380-Cyg-sec & 1:1 & 77.8 & -20 & -1 & 5.77 & 6.92 & 1.1349E+02 & Direct-PRF & 0\\
005385792-01 & 6129.01 & 1:1 & 22.1 & 4 & 5 & 12.70 & 0.90 & 7.3333E+00 & Direct-PRF & 0\\
005385792-03 & 005385778-01 & 1:1 & 22.1 & 4 & 5 & 12.70 & 0.90 & 1.2056E+00 & Direct-PRF & 1\\
005385838-01 & 6129.01 & 1:1 & 63.8 & 5 & 16 & 12.70 & 0.27 & 1.6985E+01 & Direct-PRF & 1\\
005385838-02 & V380-Cyg-sec & 1:1 & 81.2 & -15 & 15 & 5.77 & 7.20 & 9.4879E+02 & Direct-PRF & 0\\
005385838-03 & 005385750-02 & 1:3 & 89.4 & 6 & 22 & 14.48 & -1.52 & 1.0935E+01 & Direct-PRF & 1\\
005386163-01 & V380-Cyg-pri & 1:1 & 317.3 & -70 & 40 & 5.77 & 7.49 & 3.2939E+03 & Direct-PRF & 0\\
005386163-02 & V380-Cyg-sec & 1:1 & 317.3 & -70 & 40 & 5.77 & 7.49 & 3.2259E+03 & Direct-PRF & 0\\
005386264-01 & V380-Cyg-sec & 1:1 & 323.2 & -47 & 67 & 5.77 & 9.07 & 1.0753E+03 & Direct-PRF & 0\\
005390342-02 & 005390351-pri & 2:1 & 7.2 & -1 & 2 & 16.08 & -0.74 & 1.5418E+01 & Direct-PRF & 0\\
005392871-01 & 3342.01 & 1:1 & 13.3 & 2 & 3 & 15.75 & -2.36 & 4.1070E+02 & Direct-PRF & 0\\
005392871-02 & 005392897-sec & 1:1 & 13.3 & 2 & 3 & 15.75 & -2.36 & 2.8355E+02 & Direct-PRF & 0\\
005428471-01 & 005513861-pri & 1:2 & 87.2 & -15 & -16 & 11.64 & 4.07 & 1.3198E+03 & Direct-PRF & 0\\
005444334-01 & 005529643-01 & 1:1 & 57.3 & -7 & 13 & 15.93 & -0.02 & 1.4026E+00 & Direct-PRF & 1\\
005444384-01 & 005444392-pri & 1:2 & 15.6 & -2 & 4 & 11.38 & 4.17 & 1.0713E+02 & Direct-PRF & 0\\
005444491-01 & 005529738-01 & 1:1 & 76.2 & -19 & -1 & 14.87 & 0.05 & 1.8500E+00 & Direct-PRF & 1\\
005458779-01 & 005458845-01 & 1:1 & 54.0 & -9 & 10 & 13.66 & 2.14 & 5.6250E-01 & Direct-PRF & 1\\
005458795-01 & 005458880-pri & 1:1 & 87.2 & 1 & 22 & 7.82 & 7.32 & 3.1026E+02 & Direct-PRF & 0\\
005458845-01 & 005458779-01 & 1:1 & 54.0 & 9 & -10 & 15.80 & -2.14 & 1.7778E+00 & Direct-PRF & 1\\
005458953-01 & 005458880-pri & 1:1 & 87.3 & 21 & -7 & 7.82 & 6.62 & 3.7812E+02 & Direct-PRF & 0\\
005467102-01 & 3825.01 & 1:1 & 7.5 & -1 & -1 & 15.83 & -0.47 & 2.7415E+01 & Direct-PRF & 0\\
005467124-01 & 3825.01 & 1:1 & 14.6 & -2 & 3 & 15.83 & -2.24 & 7.1585E+03 & Direct-PRF & 0\\
005467126-01 & 3825.01 & 1:1 & 8.4 & 2 & 1 & 15.83 & -3.47 & 2.5148E+02 & Direct-PRF & 0\\
005467126-02 & 005467102-02 & 1:1 & 15.8 & 3 & 2 & 15.36 & -2.99 & 3.5851E+01 & Direct-PRF & 0\\
005470851-01 & V380-Cyg-pri & 1:1 & 400.9 & 62 & -79 & 5.77 & 10.02 & 8.3295E+02 & Direct-PRF & 0\\
005470862-01 & 005385509-02 & 1:1 & 518.6 & 130 & 0 & 15.71 & -0.35 & 2.8444E+00 & Col-Anomaly & 1\\
005470960-01 & V380-Cyg-pri & 1:1 & 383.4 & 82 & -50 & 5.77 & 10.18 & 8.3776E+02 & Direct-PRF & 0\\
005471010-01 & V380-Cyg-pri & 1:1 & 301.9 & 48 & -58 & 5.77 & 9.87 & 7.0356E+02 & Direct-PRF & 0\\
005471010-02 & 005385509-02 & 1:1 & 337.1 & 85 & 1 & 15.71 & -0.07 & 1.1228E+00 & Col-Anomaly & 1\\
005471059-03 & V380-Cyg-pri & 1:1 & 293.2 & 59 & -43 & 5.77 & 8.95 & 9.8594E+02 & Direct-PRF & 0\\
005471059-04 & V380-Cyg-sec & 1:1 & 293.2 & 59 & -43 & 5.77 & 8.95 & 1.0664E+03 & Direct-PRF & 0\\
005471068-01 & V380-Cyg-pri & 1:1 & 298.8 & 63 & -41 & 5.77 & 9.41 & 9.5351E+02 & Direct-PRF & 0\\
005471068-02 & V380-Cyg-sec & 1:1 & 298.8 & 63 & -41 & 5.77 & 9.41 & 1.0081E+03 & Direct-PRF & 0\\
005471108-01 & V380-Cyg-pri & 1:1 & 246.3 & 44 & -43 & 5.77 & 5.83 & 3.2939E+03 & Direct-PRF & 0\\
005471158-01 & V380-Cyg-pri & 1:1 & 207.3 & 27 & -44 & 5.77 & 9.95 & 3.7258E+02 & Direct-PRF & 0\\
005471158-02 & V380-Cyg-sec & 1:1 & 207.3 & 27 & -44 & 5.77 & 9.95 & 3.6973E+02 & Direct-PRF & 0\\
005471170-01 & 6586.01 & 1:1 & 317.6 & 80 & -4 & 12.62 & -0.37 & 4.6750E+01 & Col-Anomaly & 1\\
005471192-01 & V380-Cyg-pri & 1:1 & 218.9 & 48 & -27 & 5.77 & 8.51 & 1.1235E+03 & Direct-PRF & 0\\
005471202-01 & V380-Cyg-pri & 1:1 & 179.6 & 23 & -38 & 5.77 & 9.09 & 5.3878E+02 & Direct-PRF & 0\\
005471202-02 & V380-Cyg-sec & 1:1 & 179.6 & 23 & -38 & 5.77 & 9.09 & 4.8877E+02 & Direct-PRF & 0\\
005471217-01 & V380-Cyg-pri & 1:1 & 274.3 & 68 & -10 & 5.77 & 8.65 & 1.0980E+03 & Direct-PRF & 0\\
005471217-02 & V380-Cyg-sec & 1:1 & 274.3 & 68 & -10 & 5.77 & 8.65 & 9.2832E+02 & Direct-PRF & 0\\
005471271-01 & V380-Cyg-pri & 1:1 & 243.8 & 61 & -5 & 5.77 & 7.83 & 1.2713E+03 & Direct-PRF & 0\\
005471271-02 & V380-Cyg-sec & 1:1 & 243.8 & 61 & -5 & 5.77 & 7.83 & 1.2173E+03 & Direct-PRF & 0\\
005471289-01 & V380-Cyg-pri & 1:1 & 220.1 & 55 & -5 & 5.77 & 9.16 & 6.3014E+02 & Direct-PRF & 0\\
005471289-02 & V380-Cyg-sec & 1:1 & 220.1 & 55 & -5 & 5.77 & 9.16 & 6.5170E+02 & Direct-PRF & 0\\
005471328-01 & V380-Cyg-pri & 1:1 & 93.6 & 14 & -18 & 5.77 & 10.13 & 2.4196E+02 & Direct-PRF & 0\\
005471328-02 & 005385778-03 & 1:3 & 152.5 & 34 & -17 & 12.70 & 3.21 & 6.2818E+00 & Direct-PRF & 1\\
005471415-01 & V380-Cyg-pri & 1:1 & 88.4 & 22 & 3 & 5.77 & 6.85 & 3.7941E+02 & Direct-PRF & 0\\
005471415-02 & V380-Cyg-sec & 1:1 & 88.4 & 22 & 3 & 5.77 & 6.85 & 3.9582E+02 & Direct-PRF & 0\\
005471480-01 & V380-Cyg-pri & 1:1 & 317.3 & 68 & 42 & 5.77 & 9.94 & 4.4595E+02 & Direct-PRF & 0\\
005471480-02 & V380-Cyg-sec & 1:1 & 317.3 & 68 & 42 & 5.77 & 9.94 & 4.0964E+02 & Direct-PRF & 0\\
005471489-01 & V380-Cyg-pri & 1:1 & 297.2 & 62 & 41 & 5.77 & 7.27 & 2.1314E+03 & Direct-PRF & 0\\
005471489-02 & V380-Cyg-sec & 1:1 & 297.2 & 62 & 41 & 5.77 & 7.27 & 1.9551E+03 & Direct-PRF & 0\\
005471496-01 & V380-Cyg-pri & 1:1 & 198.2 & 39 & 30 & 5.77 & 10.12 & 1.4364E+02 & Direct-PRF & 0\\
005471496-02 & V380-Cyg-sec & 1:1 & 198.2 & 39 & 30 & 5.77 & 10.12 & 1.4087E+02 & Direct-PRF & 0\\
005471566-01 & 005471619-pri & 1:1 & 109.3 & 28 & 2 & 12.37 & 3.10 & 5.4938E+03 & Direct-PRF & 0\\
005471574-01 & 005471619-pri & 1:1 & 40.6 & 6 & -9 & 12.37 & 1.03 & 7.4492E+03 & Direct-PRF & 0\\
005471606-01 & 005471619-pri & 1:1 & 11.2 & 1 & -3 & 12.37 & -1.55 & 3.9810E+02 & Direct-PRF & 0\\
005471675-01 & 005471619-pri & 1:1 & 53.5 & 1 & 13 & 12.37 & 0.94 & 9.5543E+03 & Direct-PRF & 0\\
005471688-01 & V380-Cyg-pri & 1:1 & 248.6 & 13 & 61 & 5.77 & 9.29 & 4.1058E+02 & Direct-PRF & 0\\
005471688-02 & V380-Cyg-sec & 1:1 & 248.6 & 13 & 61 & 5.77 & 9.29 & 4.3593E+02 & Direct-PRF & 0\\
005471690-01 & V380-Cyg-pri & 1:1 & 241.2 & 10 & 60 & 5.77 & 7.10 & 1.9070E+03 & Direct-PRF & 0\\
005471690-02 & V380-Cyg-sec & 1:2 & 241.2 & 10 & 60 & 5.77 & 7.10 & 2.1871E+03 & Direct-PRF & 0\\
005471769-01 & V380-Cyg-pri & 1:1 & 363.9 & 30 & 87 & 5.77 & 9.19 & 1.3545E+03 & Direct-PRF & 0\\
005471769-02 & 005471770-02 & 1:1 & 78.4 & 17 & 10 & 13.61 & 1.36 & 8.5185E-01 & Direct-PRF & 1\\
005471770-01 & V380-Cyg-pri & 1:1 & 311.0 & 13 & 77 & 5.77 & 7.83 & 1.5097E+03 & Direct-PRF & 0\\
005471770-02 & V380-Cyg-sec & 1:1 & 311.0 & 13 & 77 & 5.77 & 7.83 & 1.4026E+03 & Direct-PRF & 0\\
005471792-01 & V380-Cyg-pri & 1:1 & 312.8 & 7 & 79 & 5.77 & 7.60 & 1.7051E+03 & Direct-PRF & 0\\
005471792-02 & V380-Cyg-sec & 1:1 & 312.8 & 7 & 79 & 5.77 & 7.60 & 1.8434E+03 & Direct-PRF & 0\\
005475641-01 & 005475624-pri & 1:1 & 13.1 & -3 & -2 & 15.55 & -1.25 & 3.3353E+03 & Direct-PRF & 0\\
005475735-01 & 6588.01 & 1:1 & 20.5 & 2 & -4 & 13.28 & 1.12 & 1.3364E+03 & Direct-PRF & 0\\
005475735-02 & 005475712-sec & 1:1 & 20.5 & 2 & -4 & 13.28 & 1.12 & 2.4464E+03 & Direct-PRF & 0\\
005475736-01 & 6588.01 & 1:1 & 12.6 & -2 & -2 & 13.28 & 0.73 & 3.6510E+02 & Direct-PRF & 0\\
005475736-02 & 005475712-sec & 1:1 & 12.6 & -2 & -2 & 13.28 & 0.73 & 4.2025E+02 & Direct-PRF & 0\\
005476835-01 & 005476864-01 & 1:1 & 15.5 & 3 & 3 & 11.47 & 2.38 & 2.7170E+00 & Direct-PRF & 0\\
005478055-01 & 005478083-01 & 1:1 & 12.6 & 2 & 1 & 17.52 & -3.01 & 5.9371E+02 & Direct-PRF & 0\\
005481416-01 & 3772.01 & 1:1 & 6.0 & 1 & 1 & 19.32 & -3.48 & 2.9084E+02 & Direct-PRF & 0\\
005513833-01 & 005513893-01 & 1:1 & 124.4 & -11 & 29 & 13.01 & 2.23 & 1.3846E+00 & Direct-PRF & 1\\
005513857-01 & 005513861-pri & 1:2 & 49.9 & 5 & 11 & 11.64 & 3.80 & 2.6674E+03 & Direct-PRF & 0\\
005513866-01 & 005513893-01 & 1:1 & 43.3 & -5 & 9 & 13.01 & 0.56 & 1.2857E+00 & Direct-PRF & 1\\
005513893-01 & 005513861-01 & 1:1 & 47.9 & 11 & -4 & 11.64 & 1.37 & 1.7537E+03 & Direct-PRF & 0\\
005513897-01 & 005513861-pri & 1:2 & 54.0 & 10 & -9 & 11.64 & 2.34 & 3.5690E+03 & Direct-PRF & 0\\
005521373-02 & 005088084-05 & 1:1 & 2409.4 & -606 & -1 & 14.93 & -2.37 & 1.8614E+01 & Col-Anomaly & 1\\
005529501-01 & 005444392-pri & 1:1 & 247.0 & 62 & 1 & 11.38 & 1.21 & 4.1160E+04 & Direct-PRF & 0\\
005529552-01 & 005529560-01 & 1:1 & 11.9 & 3 & 0 & 15.26 & 0.06 & 1.1379E+00 & Direct-PRF & 0\\
005529560-01 & 005529643-01 & 1:1 & 74.4 & 18 & 5 & 15.93 & -0.67 & 3.2727E+00 & Col-Anomaly & 1\\
005529643-01 & 005444392-01 & 1:1 & 45.7 & 11 & -2 & 11.38 & 4.55 & 3.6579E+03 & Direct-PRF & 0\\
005529738-01 & 005444491-01 & 1:1 & 76.2 & 19 & 1 & 14.92 & -0.05 & 5.4054E-01 & Direct-PRF & 1\\
005530882-01 & 6594.01 & 1:1 & 22.8 & -5 & 3 & 13.51 & 0.94 & 3.0342E+03 & Direct-PRF & 0\\
005534476-02 & 005534702-pri & 1:1 & 360.2 & 90 & 0 & 13.82 & -1.41 & 1.0144E+04 & Col-Anomaly & 0\\
005556726-01 & 005471619-pri & 1:1 & 489.4 & 123 & 1 & 12.37 & -0.20 & 1.1269E+04 & Col-Anomaly & 0\\
005556769-01 & V380-Cyg-pri & 1:1 & 421.9 & 101 & 32 & 5.77 & 8.70 & 2.7872E+03 & Direct-PRF & 0\\
005556769-02 & V380-Cyg-sec & 1:1 & 421.9 & 101 & 32 & 5.77 & 8.70 & 2.6334E+03 & Direct-PRF & 0\\
005556804-01 & V380-Cyg-pri & 1:1 & 398.7 & 94 & 33 & 5.77 & 10.13 & 6.3014E+02 & Direct-PRF & 0\\
005556804-02 & V380-Cyg-sec & 1:1 & 398.7 & 94 & 33 & 5.77 & 10.13 & 7.5021E+02 & Direct-PRF & 0\\
005556830-01 & V380-Cyg-pri & 1:1 & 416.0 & 97 & 38 & 5.77 & 9.90 & 1.0897E+03 & Direct-PRF & 0\\
005556830-02 & V380-Cyg-sec & 1:1 & 416.0 & 97 & 38 & 5.77 & 9.90 & 1.2904E+03 & Direct-PRF & 0\\
005560830-01 & 005560831-pri & 1:1 & 7.3 & 2 & -1 & 16.09 & -1.64 & 2.5138E+02 & Direct-PRF & 0\\
005565497-01 & 3742.01 & 1:1 & 11.3 & -1 & -3 & 14.96 & -3.44 & 9.8505E+03 & Direct-PRF & 0\\
005598595-01 & 005598639-01 & 1:1 & 67.8 & -13 & 11 & 10.20 & 5.20 & 6.0779E+02 & Direct-PRF & 0\\
005598645-01 & 005598639-01 & 1:1 & 84.0 & -11 & -18 & 10.20 & 1.49 & 1.0879E+04 & Direct-PRF & 0\\
005621299-01 & 6606.01 & 1:1 & 27.8 & -7 & -3 & 13.61 & 0.30 & 1.3643E+04 & Direct-PRF & 0\\
005623833-01 & RR-Lyr-pri & 2:1 & 8215.1 & -1 & -4 & 7.86 & 4.81 & 1.7314E+04 & Cross-Talk & 0\\
005623852-01 & RR-Lyr-pri & 1:1 & 8235.2 & -6 & -3 & 7.86 & 5.64 & 2.5971E+04 & Cross-Talk & 0\\
005623915-01 & RR-Lyr-pri & 2:1 & 8296.2 & -21 & 1 & 7.86 & 4.80 & 3.6664E+04 & Col-Anomaly & 0\\
005623915-02 & RR-Lyr-pri & 2:1 & 8296.2 & -21 & 1 & 7.86 & 4.80 & 5.1941E+04 & Col-Anomaly & 0\\
005632701-01 & 6609.01 & 1:3 & 48.7 & -5 & 11 & 12.11 & 1.88 & 8.4571E+03 & Direct-PRF & 0\\
005632745-01 & 005632781-sec & 1:1 & 61.0 & 10 & 12 & 12.11 & 1.19 & 9.6564E+03 & Direct-PRF & 0\\
005636648-01 & 3817.01 & 1:1 & 6.3 & 1 & 2 & 16.43 & -1.10 & 4.8137E+01 & Direct-PRF & 0\\
005649215-01 & 3636.01 & 1:1 & 7.7 & -1 & -1 & 17.99 & -2.97 & 8.2103E+02 & Direct-PRF & 0\\
005649833-01 & 3831.01 & 1:1 & 12.0 & 3 & -1 & 16.38 & -3.01 & 5.3106E+03 & Direct-PRF & 0\\
005652237-01 & 3703.01 & 1:1 & 9.4 & 0 & 2 & 17.30 & -3.79 & 4.3968E+02 & Direct-PRF & 0\\
005653126-03 & 6134.01 & 1:1 & 55.8 & -1 & 14 & 11.94 & 1.23 & 6.4072E+03 & Direct-PRF & 0\\
005653163-01 & 6134.01 & 1:1 & 96.9 & -18 & 16 & 11.94 & -1.31 & 1.0504E+03 & Direct-PRF & 0\\
005686974-01 & 5206.01 & 1:1 & 771.4 & 194 & 1 & 14.74 & -1.01 & 4.1810E+03 & Col-Anomaly & 0\\
005696918-01 & 6614.01 & 1:1 & 8.6 & 2 & 0 & 14.98 & -0.18 & 3.8847E+01 & Direct-PRF & 0\\
005724811-01 & 005724810-01 & 1:1 & 5.2 & -1 & 1 & 10.90 & 1.38 & 3.8333E+00 & Direct-PRF & 0\\
005725846-01 & 6620.01 & 1:1 & 5.4 & -1 & 0 & 13.41 & 1.95 & 3.0455E+00 & Direct-PRF & 0\\
005725851-01 & 005725846-01 & 1:1 & 5.4 & 1 & 0 & 15.36 & -1.95 & 2.6400E+00 & Direct-PRF & 0\\
005730389-01 & 3603.01 & 1:2 & 12.8 & 3 & -1 & 16.12 & -1.50 & 1.2942E+03 & Direct-PRF & 0\\
005738496-01 & 005738506-01 & 1:1 & 11.2 & -1 & 2 & 18.35 & -3.55 & 1.1571E+03 & Direct-PRF & 0\\
005738496-02 & 3676.01 & 1:1 & 11.2 & -1 & 2 & 18.35 & -3.55 & 2.1249E+03 & Direct-PRF & 0\\
005738634-01 & 6134.01 & 1:1 & 72.0 & 18 & -1 & 11.94 & 1.31 & 5.0056E+03 & Direct-PRF & 0\\
005796186-01 & 3369.01 & 1:1 & 8.5 & 2 & 1 & 15.83 & -1.92 & 6.5938E+01 & Direct-PRF & 0\\
005802292-01 & 005802285-pri & 1:2 & 7.0 & 0 & -2 & 15.35 & 0.56 & 5.8929E+01 & Direct-PRF & 0\\
005802478-01 & 6628.01 & 1:1 & 17.5 & 4 & 1 & 13.76 & 0.63 & 5.7487E+02 & Direct-PRF & 0\\
005816811-01 & 3645.01 & 1:1 & 7.0 & -2 & 0 & 17.05 & -2.20 & 2.9693E+02 & Direct-PRF & 0\\
005816811-02 & 005816806-01 & 2:1 & 7.0 & -2 & 0 & 17.05 & -2.20 & 4.7915E+02 & Direct-PRF & 0\\
005817533-01 & 005817566-sec & 1:2 & 51.4 & -9 & 9 & 11.68 & 3.63 & 1.0972E+03 & Direct-PRF & 0\\
005817553-01 & 005817566-sec & 1:2 & 15.3 & -3 & 3 & 11.68 & 2.40 & 1.7565E+02 & Direct-PRF & 0\\
005817613-01 & 6138.01 & 1:1 & 44.5 & -11 & -1 & 11.68 & 4.21 & 5.3223E+02 & Direct-PRF & 0\\
005817685-01 & 005817566-sec & 1:2 & 62.2 & -4 & -15 & 11.68 & 3.05 & 2.9962E+03 & Direct-PRF & 0\\
005817712-01 & 005817566-sec & 1:2 & 74.3 & -8 & -17 & 11.68 & 3.77 & 1.6400E+03 & Direct-PRF & 0\\
005817957-01 & 6586.01 & 30:1 & 2893.7 & 43 & -7 & 12.62 & 2.80 & 1.2871E+00 & Col-Anomaly & 1\\
005823557-01 & 6134.01 & 1:1 & 533.0 & 134 & 0 & 11.94 & 1.95 & 8.8989E+03 & Col-Anomaly & 0\\
005866099-01 & 3651.01 & 1:1 & 5.5 & 0 & -1 & 17.07 & -3.37 & 1.6861E+02 & Direct-PRF & 0\\
005866099-02 & 005866104-02 & 1:1 & 5.5 & 0 & -1 & 17.07 & -3.37 & 2.2602E+02 & Direct-PRF & 0\\
005876368-01 & 005876360-sec & 1:2 & 5.0 & -1 & 1 & 17.17 & -2.38 & 2.2446E+02 & Direct-PRF & 0\\
005903312-01 & 3692.01 & 1:1 & 8.0 & -2 & -1 & 15.15 & -2.70 & 1.2189E+02 & Direct-PRF & 0\\
005904622-01 & 005820209-pri & 1:1 & 388.7 & 98 & 0 & 13.49 & -0.67 & 6.8231E+03 & Col-Anomaly & 0\\
005952309-01 & 6139.01 & 1:1 & 66.3 & -10 & 13 & 6.97 & 7.95 & 7.0447E+01 & Direct-PRF & 0\\
005952366-01 & 6139.01 & 1:1 & 34.5 & 0 & 9 & 6.97 & 6.41 & 2.8323E+00 & Direct-PRF & 0\\
005952403-01 & 3947.01 & 1:1 & 34.5 & 0 & -9 & 13.38 & -6.41 & 1.3200E+00 & Direct-PRF & 1\\
005952448-01 & 6139.01 & 1:1 & 78.8 & -12 & -15 & 6.97 & 8.42 & 6.1315E+01 & Direct-PRF & 0\\
005952457-01 & 6139.01 & 1:1 & 60.3 & -6 & -14 & 6.97 & 8.32 & 3.4490E+01 & Direct-PRF & 0\\
005956787-01 & 3821.01 & 1:1 & 8.2 & 1 & -2 & 16.75 & -4.65 & 1.7220E+04 & Direct-PRF & 0\\
005962509-01 & 005962514-pri & 1:2 & 18.6 & -3 & -4 & 14.84 & 0.69 & 3.4032E+03 & Direct-PRF & 0\\
005982368-01 & 005982353-pri & 1:1 & 11.0 & 3 & 1 & 11.12 & 2.92 & 2.5951E+00 & Direct-PRF & 0\\
006044999-01 & RR-Lyr-pri & 1:1 & 6285.3 & 485 & 2 & 7.86 & 7.18 & 1.6403E+04 & Col-Anomaly & 0\\
006045250-01 & 006045264-pri & 1:1 & 9.0 & 2 & 0 & 13.44 & 1.53 & 3.1640E+01 & Direct-PRF & 0\\
006045250-02 & 006045264-sec & 1:1 & 9.0 & 2 & 0 & 13.44 & 1.53 & 1.8526E+01 & Direct-PRF & 0\\
006050154-01 & RR-Lyr-pri & 1:1 & 9077.8 & -30 & -2 & 7.86 & 7.76 & 1.4840E+04 & Col-Anomaly & 0\\
006058896-01 & 006058875-pri & 1:1 & 10.2 & 0 & 2 & 15.84 & -1.05 & 1.5112E+03 & Direct-PRF & 0\\
006058896-02 & 3616.01 & 2:1 & 10.2 & 0 & 2 & 15.84 & -1.05 & 3.8278E+01 & Direct-PRF & 0\\
006066403-01 & 3649.01 & 1:1 & 12.2 & 3 & -1 & 15.47 & -1.92 & 7.9036E+02 & Direct-PRF & 0\\
006066416-01 & 3649.01 & 1:1 & 14.8 & 2 & -3 & 15.47 & -3.92 & 5.1373E+03 & Direct-PRF & 0\\
006123381-01 & 006204758-01 & 1:1 & 102.0 & -25 & -4 & 15.15 & 0.78 & 1.1429E+00 & Col-Anomaly & 1\\
006126076-01 & 006045264-pri & 1:1 & 432.0 & 109 & 1 & 13.44 & -0.71 & 3.6010E+04 & Col-Anomaly & 0\\
006126076-02 & 006045264-sec & 1:1 & 432.0 & 109 & 1 & 13.44 & -0.71 & 7.0340E+04 & Col-Anomaly & 0\\
006137681-01 & 3605.01 & 1:1 & 9.6 & -1 & -3 & 14.16 & 1.32 & 2.1004E+01 & Direct-PRF & 0\\
006182846-01 & 3512.01 & 1:1 & 8.2 & -2 & 1 & 13.72 & 1.08 & 4.1631E+00 & Direct-PRF & 0\\
006185711-01 & 6671.01 & 1:1 & 11.8 & 3 & -2 & 13.39 & 0.19 & 4.5727E+01 & Direct-PRF & 0\\
006187888-01 & 006187893-pri & 1:1 & 57.2 & 10 & -10 & 11.70 & 3.65 & 9.7576E+02 & Direct-PRF & 0\\
006199702-01 & 1812.01 & 1:1 & 6.1 & 2 & 1 & 13.74 & 0.89 & 5.9247E+00 & Direct-PRF & 0\\
006199716-01 & 1812.01 & 1:1 & 10.6 & 3 & -2 & 13.74 & 2.14 & 1.5064E+01 & Direct-PRF & 0\\
006200715-01 & 3694.01 & 1:1 & 6.9 & 2 & -1 & 16.72 & -1.79 & 9.3807E+01 & Direct-PRF & 0\\
006204758-01 & 006123381-01 & 1:1 & 102.0 & 25 & 4 & 15.93 & -0.78 & 8.7500E-01 & Col-Anomaly & 1\\
006205384-01 & 006205460-pri & 1:1 & 87.6 & 22 & -2 & 12.75 & 1.20 & 1.8318E+04 & Direct-PRF & 0\\
006205405-01 & 006205460-pri & 1:1 & 50.2 & -2 & -12 & 12.75 & 1.79 & 9.7312E+03 & Direct-PRF & 0\\
006205468-01 & 006205460-pri & 1:1 & 17.6 & -4 & 0 & 12.75 & 2.77 & 4.8542E+02 & Direct-PRF & 0\\
006205481-01 & 006205460-pri & 1:1 & 18.1 & -4 & 2 & 12.75 & 2.93 & 1.5928E+03 & Direct-PRF & 0\\
006205483-01 & 006205460-pri & 1:1 & 45.8 & 7 & 10 & 12.75 & 2.80 & 6.4875E+03 & Direct-PRF & 0\\
006205507-01 & 006205460-pri & 1:1 & 107.0 & 14 & 23 & 12.75 & -0.05 & 7.7850E+04 & Direct-PRF & 0\\
006205566-01 & 006205460-pri & 1:1 & 100.2 & -10 & 23 & 12.75 & 2.46 & 1.2212E+04 & Direct-PRF & 0\\
006206470-01 & 6640.01 & 1:1 & 1510.3 & 380 & 0 & 13.88 & -0.15 & 4.6107E+03 & Col-Anomaly & 0\\
006206559-01 & 006206751-pri & 1:1 & 308.0 & 78 & -1 & 12.14 & 0.20 & 8.9667E+03 & Col-Anomaly & 0\\
006233483-01 & 3552.01 & 1:1 & 7.7 & 1 & -1 & 14.68 & -0.77 & 1.8502E+01 & Direct-PRF & 0\\
006233483-02 & 006233466-sec & 1:1 & 7.7 & 1 & -1 & 14.68 & -0.77 & 1.3283E+01 & Direct-PRF & 0\\
006233890-01 & 3609.01 & 1:1 & 10.9 & 1 & 2 & 16.45 & -3.28 & 1.4433E+03 & Direct-PRF & 0\\
006285094-01 & TT-Lyr-pri & 1:1 & 219.0 & -27 & -49 & 9.49 & 5.47 & 1.1542E+04 & Direct-PRF & 0\\
006285396-01 & TT-Lyr-pri & 1:1 & 283.6 & -42 & -26 & 9.49 & 6.30 & 7.5586E+03 & Direct-PRF & 0\\
006285397-01 & TT-Lyr-pri & 1:1 & 261.5 & -37 & -23 & 9.49 & 6.42 & 6.5701E+03 & Direct-PRF & 0\\
006286155-01 & 006286161-01 & 1:1 & 7.5 & -1 & -2 & 16.71 & -2.95 & 3.2336E+02 & Direct-PRF & 0\\
006286155-02 & 3501.01 & 1:1 & 7.5 & -1 & -2 & 16.71 & -2.95 & 3.8575E+02 & Direct-PRF & 0\\
006289897-01 & 006048106-pri & 1:1 & 964.3 & 243 & -1 & 14.09 & -0.73 & 8.7970E+03 & Col-Anomaly & 0\\
006292732-01 & 006292803-01 & 1:1 & 114.2 & 29 & 0 & 14.01 & -0.10 & 7.5767E+03 & Col-Anomaly & 0\\
006301035-01 & 006301030-pri & 1:1 & 8.8 & 3 & 1 & 17.78 & -2.80 & 9.2773E+01 & Direct-PRF & 0\\
006301035-02 & 6027.01 & 1:1 & 8.8 & 3 & 1 & 17.78 & -2.80 & 2.2115E+02 & Direct-PRF & 0\\
006302008-01 & 006302051-pri & 1:1 & 29.3 & -6 & -4 & 13.33 & 1.76 & 4.6683E+03 & Direct-PRF & 0\\
006307063-01 & 3153.01 & 1:1 & 14.6 & 3 & 2 & 14.86 & -1.17 & 1.3618E+03 & Direct-PRF & 0\\
006307083-01 & 3153.01 & 1:1 & 16.4 & 2 & -4 & 14.86 & -2.64 & 1.1563E+03 & Direct-PRF & 0\\
006307083-02 & 006307062-02 & 1:1 & 16.4 & 2 & -4 & 14.86 & -2.64 & 1.3765E+03 & Direct-PRF & 0\\
006307521-01 & 006307537-pri & 1:1 & 19.3 & 2 & 4 & 11.75 & 3.51 & 2.4019E+02 & Direct-PRF & 0\\
006307521-02 & 1120.01 & 8:1 & 19.3 & 2 & 4 & 11.75 & 3.51 & 9.0104E+01 & Direct-PRF & 0\\
006307573-01 & 006307537-pri & 1:1 & 48.2 & 12 & -1 & 11.75 & 2.94 & 1.9637E+03 & Direct-PRF & 0\\
006312534-01 & 3656.01 & 1:2 & 6.2 & 1 & -1 & 17.36 & -1.77 & 8.3120E+01 & Direct-PRF & 0\\
006314185-01 & 3708.01 & 1:1 & 7.0 & 0 & -2 & 17.72 & -2.83 & 6.1453E+01 & Direct-PRF & 0\\
006343576-01 & 3512.01 & 1:1 & 1371.0 & 345 & 0 & 13.72 & -0.21 & 2.0846E+03 & Col-Anomaly & 0\\
006359802-01 & 1121.01 & 1:1 & 4.5 & 1 & -1 & 12.93 & 2.12 & 2.0817E+00 & Direct-PRF & 0\\
006359802-02 & 006359798-02 & 1:1 & 4.5 & 1 & -1 & 12.93 & 2.12 & 1.3450E+00 & Direct-PRF & 0\\
006363560-01 & 006363494-pri & 1:2 & 99.4 & 25 & -1 & 14.42 & -0.89 & 3.0522E+03 & Direct-PRF & 0\\
006363867-01 & TT-Lyr-pri & 1:1 & 379.4 & -68 & -68 & 9.49 & 5.38 & 2.1353E+04 & Direct-PRF & 0\\
006364064-01 & TT-Lyr-pri & 1:1 & 209.5 & -39 & -36 & 9.49 & 5.70 & 7.4271E+03 & Direct-PRF & 0\\
006364067-01 & TT-Lyr-pri & 1:1 & 202.3 & -33 & -39 & 9.49 & 6.07 & 7.0010E+03 & Direct-PRF & 0\\
006364071-01 & 006364126-01 & 1:1 & 88.0 & -22 & 0 & 14.90 & -0.52 & 3.5333E+00 & Direct-PRF & 1\\
006364126-01 & 006364071-01 & 1:1 & 88.0 & 22 & 0 & 14.38 & 0.52 & 2.8302E-01 & Direct-PRF & 1\\
006364143-01 & TT-Lyr-pri & 1:1 & 258.7 & -65 & 3 & 9.49 & 5.09 & 1.3346E+04 & Direct-PRF & 0\\
006364162-01 & TT-Lyr-pri & 1:1 & 149.6 & -36 & -12 & 9.49 & 5.67 & 3.8301E+03 & Direct-PRF & 0\\
006364195-01 & TT-Lyr-pri & 1:1 & 253.4 & -62 & 14 & 9.49 & 6.43 & 7.5586E+03 & Direct-PRF & 0\\
006364200-01 & TT-Lyr-pri & 1:1 & 324.9 & -78 & 25 & 9.49 & 6.37 & 9.4902E+03 & Direct-PRF & 0\\
006364215-01 & TT-Lyr-pri & 1:1 & 252.8 & -61 & 19 & 9.49 & 6.16 & 7.4271E+03 & Direct-PRF & 0\\
006364247-01 & TT-Lyr-pri & 1:1 & 277.0 & -63 & 29 & 9.49 & 4.14 & 3.1634E+04 & Direct-PRF & 0\\
006364276-01 & TT-Lyr-pri & 1:1 & 154.7 & -34 & 19 & 9.49 & 5.80 & 3.8474E+03 & Direct-PRF & 0\\
006364307-01 & TT-Lyr-pri & 1:1 & 179.7 & -35 & 29 & 9.49 & 6.34 & 4.1063E+03 & Direct-PRF & 0\\
006364327-01 & TT-Lyr-pri & 1:1 & 169.8 & -30 & 30 & 9.49 & 5.09 & 4.0867E+03 & Direct-PRF & 0\\
006380593-01 & 006380765-01 & 1:1 & 97.9 & -10 & -23 & 14.85 & -1.41 & 2.4615E+00 & Direct-PRF & 1\\
006380750-01 & 006380765-01 & 1:1 & 53.6 & -13 & 5 & 14.85 & -0.58 & 1.6842E+00 & Direct-PRF & 1\\
006380765-01 & 006380750-01 & 1:1 & 53.6 & 13 & -5 & 14.27 & 0.58 & 5.9375E-01 & Direct-PRF & 1\\
006386784-01 & 6729.01 & 1:1 & 692.6 & 175 & 1 & 13.75 & -1.80 & 1.4949E+04 & Col-Anomaly & 0\\
006421503-01 & 006421483-pri & 1:1 & 20.3 & 4 & 4 & 13.02 & 2.22 & 5.5785E+02 & Direct-PRF & 0\\
006442246-01 & 006521542-01 & 1:1 & 363.7 & 92 & 0 & 14.28 & -0.89 & 1.8905E+04 & Col-Anomaly & 0\\
006445531-01 & 5293.01 & 1:1 & 106.1 & -18 & -20 & 10.15 & 5.61 & 2.0197E+03 & Direct-PRF & 0\\
006449291-01 & 006449358-pri & 1:1 & 100.8 & 25 & -2 & 11.61 & 2.10 & 2.0391E+03 & Direct-PRF & 0\\
006462874-01 & 94.01 & 1:1 & 7.3 & 1 & -1 & 12.21 & 3.51 & 1.9482E+00 & Direct-PRF & 0\\
006462874-02 & 94.03 & 7:1 & 7.3 & 1 & -1 & 12.21 & 3.51 & 3.6094E+00 & Direct-PRF & 0\\
006462874-03 & 94.02 & 1:1 & 7.3 & 1 & -1 & 12.21 & 3.51 & 1.0981E+00 & Direct-PRF & 0\\
006462874-05 & 94.03 & 1:1 & 7.3 & 1 & -1 & 12.21 & 3.51 & 2.1393E+00 & Direct-PRF & 0\\
006470521-01 & 3705.01 & 1:1 & 6.6 & -1 & -1 & 16.45 & -2.59 & 1.3716E+02 & Direct-PRF & 0\\
006470521-02 & 3705.01 & 1:2 & 6.6 & -1 & -1 & 16.45 & -2.59 & 5.7171E+02 & Direct-PRF & 0\\
006471229-01 & 6720.01 & 1:1 & 4.1 & -1 & -1 & 13.29 & 0.68 & 4.5060E+00 & Direct-PRF & 0\\
006471230-01 & 006471229-01 & 1:1 & 4.1 & 1 & 1 & 13.98 & -0.68 & 1.9762E+00 & Direct-PRF & 0\\
006507427-01 & 3815.01 & 1:1 & 4.3 & -1 & 0 & 15.43 & -1.02 & 1.3700E+01 & Direct-PRF & 0\\
006522745-01 & 6724.01 & 1:1 & 43.5 & -9 & 5 & 11.23 & 4.72 & 6.9277E+02 & Direct-PRF & 0\\
006522745-02 & 006522750-02 & 1:1 & 43.5 & -9 & 5 & 11.23 & 4.72 & 6.6898E+02 & Direct-PRF & 0\\
006522824-01 & 6724.01 & 1:1 & 64.5 & 6 & 15 & 11.23 & 4.58 & 9.7755E+02 & Direct-PRF & 0\\
006525106-01 & 5293.01 & 1:1 & 106.3 & -1 & -27 & 10.15 & 5.27 & 1.6940E+03 & Direct-PRF & 0\\
006525185-01 & 5293.01 & 1:1 & 76.3 & 17 & 8 & 10.15 & 5.71 & 7.0964E+02 & Direct-PRF & 0\\
006525193-01 & 5293.01 & 1:1 & 76.5 & -16 & -11 & 10.15 & 5.64 & 6.6193E+02 & Direct-PRF & 0\\
006525209-04 & 5293.01 & 1:1 & 63.8 & -15 & -7 & 10.15 & 4.50 & 1.1253E+03 & Direct-PRF & 0\\
006525249-01 & 5293.01 & 1:1 & 77.6 & -19 & 1 & 10.15 & 5.81 & 4.1026E+02 & Direct-PRF & 0\\
006525280-01 & 5293.01 & 1:1 & 84.8 & 0 & 21 & 10.15 & 3.23 & 4.0395E+03 & Direct-PRF & 0\\
006531491-01 & 3646.01 & 1:1 & 8.3 & -1 & 1 & 16.09 & -0.49 & 6.3252E+01 & Direct-PRF & 0\\
006531491-02 & 3646.01 & 1:2 & 8.3 & -1 & 1 & 16.09 & -0.49 & 1.5943E+02 & Direct-PRF & 0\\
006531491-04 & 006531496-03 & 1:1 & 8.3 & -1 & 1 & 16.09 & -0.49 & 6.0417E+00 & Direct-PRF & 0\\
006543645-01 & 6728.01 & 1:1 & 45.0 & 7 & 9 & 13.91 & -0.46 & 2.5887E+04 & Direct-PRF & 0\\
006543674-01 & 6728.01 & 1:1 & 5.6 & 0 & 1 & 13.91 & -0.37 & 3.2169E+00 & Direct-PRF & 0\\
006543682-01 & 5298.01 & 1:1 & 5.6 & 0 & -1 & 13.54 & 0.37 & 1.8547E+00 & Direct-PRF & 0\\
006543683-01 & 6728.01 & 1:1 & 13.6 & 3 & 1 & 13.91 & 0.09 & 9.3231E+01 & Direct-PRF & 0\\
006545051-01 & 006545018-pri & 1:2 & 22.8 & 0 & -6 & 13.75 & 1.99 & 1.4723E+03 & Direct-PRF & 0\\
006546528-01 & 006546508-01 & 1:1 & 10.3 & 1 & -2 & 15.74 & -1.14 & 1.2130E+02 & Direct-PRF & 0\\
006612284-01 & 006206751-pri & 1:1 & 3776.4 & 0 & -2 & 12.14 & 3.75 & 1.5619E+03 & Cross-Talk & 0\\
006634133-01 & 5308.01 & 1:1 & 12.7 & 3 & 0 & 14.10 & 0.03 & 7.6203E+01 & Direct-PRF & 0\\
006675056-01 & 3611.01 & 1:1 & 9.3 & 1 & 2 & 16.51 & -0.96 & 1.3083E+02 & Direct-PRF & 0\\
006677256-01 & 3622.01 & 1:1 & 19.5 & -4 & -3 & 12.77 & 1.75 & 2.7249E+01 & Direct-PRF & 0\\
006677256-02 & 006677267-02 & 1:1 & 19.5 & -4 & -3 & 12.77 & 1.75 & 8.6207E+00 & Direct-PRF & 0\\
006695801-01 & 6757.01 & 1:1 & 117.2 & 30 & -1 & 15.41 & -0.83 & 3.4010E+03 & Col-Anomaly & 0\\
006705137-01 & 1758.01 & 1:1 & 5.1 & 0 & 2 & 15.97 & -1.34 & 7.4171E+00 & Direct-PRF & 0\\
006778008-01 & 006778050-01 & 1:1 & 22.7 & -2 & -5 & 14.51 & 0.75 & 2.8125E+03 & Direct-PRF & 0\\
006778008-02 & 006778050-sec & 1:1 & 22.7 & -2 & -5 & 14.51 & 0.75 & 2.5548E+03 & Direct-PRF & 0\\
006778019-01 & 006778050-01 & 1:1 & 21.1 & 0 & -5 & 14.51 & 0.25 & 2.7589E+03 & Direct-PRF & 0\\
006778019-02 & 006778050-sec & 1:1 & 21.1 & 0 & -5 & 14.51 & 0.25 & 3.2108E+03 & Direct-PRF & 0\\
006781548-01 & 6769.01 & 1:1 & 15.4 & 3 & -1 & 13.67 & 2.01 & 6.4992E+01 & Direct-PRF & 0\\
006781548-02 & 006781535-02 & 1:1 & 15.4 & 3 & -1 & 13.67 & 2.01 & 7.2769E+01 & Direct-PRF & 0\\
006792124-01 & 006791604-pri & 1:1 & 333.3 & 84 & 0 & 13.92 & -0.65 & 2.1105E+04 & Col-Anomaly & 0\\
006859801-01 & 6778.01 & 1:1 & 10.0 & -2 & -2 & 12.07 & 2.81 & 1.1811E+01 & Direct-PRF & 0\\
006859801-02 & 006859813-02 & 1:1 & 10.0 & -2 & -2 & 12.07 & 2.81 & 1.2079E+01 & Direct-PRF & 0\\
006862332-01 & 865.01 & 1:1 & 5.0 & 1 & 0 & 15.09 & 0.56 & 3.9300E+00 & Direct-PRF & 0\\
006862750-01 & 4020.01 & 1:1 & 3918.6 & -407 & 8 & 14.65 & 1.29 & 1.2474E+01 & Col-Anomaly & 1\\
006863187-01 & 006863229-pri & 1:1 & 77.6 & -19 & 4 & 12.13 & 3.50 & 3.0190E+03 & Direct-PRF & 0\\
006863839-01 & 6779.01 & 1:1 & 17.0 & 4 & -3 & 15.14 & -0.52 & 2.5563E+03 & Direct-PRF & 0\\
006864885-01 & 006864859-01 & 1:1 & 24.5 & 5 & 2 & 11.66 & 3.93 & 4.3860E+02 & Direct-PRF & 0\\
006864885-02 & 006864859-02 & 1:1 & 24.5 & 5 & 2 & 11.66 & 3.93 & 3.9942E+02 & Direct-PRF & 0\\
006864891-01 & 006864859-02 & 1:1 & 49.3 & 12 & 0 & 11.66 & 4.28 & 6.5574E+02 & Direct-PRF & 0\\
006864891-02 & 006864859-01 & 1:1 & 49.3 & 12 & 0 & 11.66 & 4.28 & 5.3638E+02 & Direct-PRF & 0\\
006864893-01 & 006864859-01 & 1:1 & 31.3 & 0 & 8 & 11.66 & 3.26 & 5.0384E+02 & Direct-PRF & 0\\
006864893-02 & 006864859-02 & 1:1 & 31.3 & 0 & 8 & 11.66 & 3.26 & 6.3449E+02 & Direct-PRF & 0\\
006891366-01 & 5335.01 & 1:1 & 63.9 & -9 & 13 & 11.39 & 2.22 & 3.4200E+03 & Direct-PRF & 0\\
006891543-01 & 5335.01 & 1:1 & 25.0 & -2 & -6 & 11.39 & 3.06 & 1.5263E+03 & Direct-PRF & 0\\
006891637-01 & 5335.01 & 1:1 & 63.4 & 5 & -15 & 11.39 & 4.44 & 8.7319E+02 & Direct-PRF & 0\\
006929016-01 & 006669809-pri & 1:1 & 1984.6 & -499 & 2 & 10.76 & 5.01 & 3.1481E+03 & Col-Anomaly & 0\\
006936075-01 & FN-Lyr-pri & 1:1 & 57.3 & -1 & 15 & 12.88 & 2.64 & 6.1016E+02 & Direct-PRF & 0\\
006936966-01 & 6791.01 & 1:1 & 17.3 & 3 & 3 & 14.36 & -2.46 & 2.5323E+03 & Direct-PRF & 0\\
006946700-01 & RR-Lyr-pri & 1:1 & 1186.6 & 173 & -244 & 7.86 & 7.42 & 1.7314E+04 & Direct-PRF & 0\\
006947095-01 & RR-Lyr-pri & 1:1 & 1064.9 & 213 & -163 & 7.86 & 7.26 & 2.3973E+04 & Direct-PRF & 0\\
006947300-01 & RR-Lyr-pri & 1:1 & 1115.3 & 248 & -131 & 7.86 & 7.97 & 6.2330E+05 & Direct-PRF & 0\\
006947339-01 & RR-Lyr-pri & 1:1 & 1147.5 & 261 & -124 & 7.86 & 7.90 & 6.2330E+05 & Direct-PRF & 0\\
006947837-01 & RR-Lyr-pri & 1:1 & 1224.1 & 305 & -39 & 7.86 & 4.47 & 6.2330E+05 & Direct-PRF & 0\\
006948006-01 & RR-Lyr-pri & 1:1 & 1259.1 & 316 & 2 & 7.86 & 5.67 & 2.3973E+04 & Direct-PRF & 0\\
006950275-01 & 006864859-02 & 1:1 & 35.5 & -9 & 3 & 11.66 & 4.16 & 6.1456E+02 & Direct-PRF & 0\\
006950275-02 & 006864859-01 & 1:1 & 35.5 & -9 & 3 & 11.66 & 4.16 & 7.5281E+02 & Direct-PRF & 0\\
006953281-01 & RR-Lyr-pri & 1:1 & 5197.6 & 942 & -2 & 7.86 & 7.70 & 9.4439E+03 & Col-Anomaly & 0\\
006954721-01 & 006954748-01 & 1:1 & 24.8 & 0 & 6 & 13.81 & -0.89 & 2.1789E+00 & Direct-PRF & 1\\
006954748-01 & 006954721-01 & 1:1 & 24.8 & 0 & -6 & 12.92 & 0.89 & 4.5894E-01 & Direct-PRF & 1\\
006956233-01 & 006956216-pri & 1:1 & 10.9 & 0 & -3 & 14.55 & 1.38 & 7.1628E+01 & Direct-PRF & 0\\
006960445-01 & 3654.01 & 1:2 & 6.7 & -1 & -1 & 16.80 & -2.96 & 2.6678E+02 & Direct-PRF & 0\\
006960456-01 & 3654.01 & 1:2 & 8.0 & 0 & -2 & 16.80 & -2.01 & 5.0527E+02 & Direct-PRF & 0\\
006967430-01 & 7048.01 & 1:1 & 8373.6 & 1 & 2 & 13.25 & 1.22 & 2.5266E+03 & Cross-Talk & 0\\
007013923-01 & 007097571-pri & 1:1 & 41.8 & 6 & 8 & 11.27 & 4.58 & 1.0909E+03 & Direct-PRF & 0\\
007021131-01 & 007021124-01 & 1:1 & 10.9 & 1 & -2 & 13.55 & -0.49 & 2.0825E+02 & Direct-PRF & 0\\
007023872-01 & 007023917-pri & 1:1 & 52.0 & 5 & 12 & 10.12 & 4.81 & 1.5000E+03 & Direct-PRF & 0\\
007023973-01 & 007023917-pri & 1:1 & 47.9 & -11 & -3 & 10.12 & 1.65 & 7.3500E+03 & Direct-PRF & 0\\
007024511-01 & 007024530-01 & 6:1 & 12.7 & 1 & 4 & 15.52 & -2.87 & 9.7503E+00 & Direct-PRF & 0\\
007024511-03 & 007024530-01 & 5:1 & 12.7 & 1 & 4 & 15.52 & -2.87 & 2.0336E+01 & Direct-PRF & 0\\
007025526-01 & 3550.01 & 1:1 & 16.2 & 1 & 4 & 15.78 & -4.04 & 1.4328E+04 & Direct-PRF & 0\\
007025846-01 & 6803.01 & 1:1 & 14.8 & 3 & -2 & 14.39 & -0.09 & 1.2190E+03 & Direct-PRF & 0\\
007030996-01 & RR-Lyr-pri & 1:1 & 1320.1 & -6 & -332 & 7.86 & 6.33 & 1.5582E+05 & Direct-PRF & 0\\
007031066-01 & RR-Lyr-pri & 1:1 & 1315.9 & 18 & -331 & 7.86 & 7.08 & 1.8332E+04 & Direct-PRF & 0\\
007031126-01 & RR-Lyr-pri & 1:1 & 1214.7 & 7 & -306 & 7.86 & 6.08 & 6.9255E+04 & Direct-PRF & 0\\
007031132-01 & RR-Lyr-pri & 1:1 & 1353.6 & 56 & -336 & 7.86 & 4.96 & 6.2330E+04 & Direct-PRF & 0\\
007031175-01 & RR-Lyr-pri & 1:1 & 1353.8 & 70 & -334 & 7.86 & 7.16 & 6.2330E+05 & Direct-PRF & 0\\
007031192-01 & RR-Lyr-pri & 1:1 & 1266.4 & 49 & -315 & 7.86 & 7.04 & 3.4628E+04 & Direct-PRF & 0\\
007031195-01 & RR-Lyr-pri & 1:1 & 1169.2 & 17 & -294 & 7.86 & 7.09 & 2.1493E+04 & Direct-PRF & 0\\
007031208-01 & RR-Lyr-pri & 1:1 & 1253.1 & 48 & -312 & 7.86 & 7.46 & 3.6664E+04 & Direct-PRF & 0\\
007031293-01 & RR-Lyr-pri & 1:1 & 1108.7 & 32 & -278 & 7.86 & 4.96 & 6.2330E+04 & Direct-PRF & 0\\
007031316-01 & RR-Lyr-pri & 1:1 & 1197.1 & 67 & -294 & 7.86 & 6.82 & 8.3106E+03 & Direct-PRF & 0\\
007031340-01 & RR-Lyr-pri & 1:1 & 1092.3 & 42 & -272 & 7.86 & 6.58 & 1.1543E+04 & Direct-PRF & 0\\
007031347-01 & RR-Lyr-pri & 1:1 & 1119.8 & 53 & -277 & 7.86 & 6.76 & 1.0746E+04 & Direct-PRF & 0\\
007031363-01 & RR-Lyr-pri & 1:1 & 1282.0 & 103 & -306 & 7.86 & 6.07 & 3.8956E+04 & Direct-PRF & 0\\
007031399-01 & RR-Lyr-pri & 1:1 & 1091.8 & 61 & -268 & 7.86 & 8.09 & 2.9681E+04 & Direct-PRF & 0\\
007031402-01 & RR-Lyr-pri & 1:1 & 1107.5 & 66 & -271 & 7.86 & 4.88 & 3.4628E+04 & Direct-PRF & 0\\
007031421-01 & RR-Lyr-pri & 1:1 & 1130.6 & 80 & -273 & 7.86 & 5.70 & 4.1553E+04 & Direct-PRF & 0\\
007031430-01 & RR-Lyr-pri & 1:1 & 1011.0 & 48 & -250 & 7.86 & 7.65 & 1.0053E+04 & Direct-PRF & 0\\
007031448-01 & RR-Lyr-pri & 1:1 & 1229.2 & 113 & -288 & 7.86 & 5.70 & 5.1941E+04 & Direct-PRF & 0\\
007031477-01 & RR-Lyr-pri & 1:1 & 1142.3 & 98 & -271 & 7.86 & 7.63 & 1.1760E+04 & Direct-PRF & 0\\
007031504-01 & RR-Lyr-pri & 1:1 & 1029.8 & 78 & -247 & 7.86 & 7.76 & 1.4495E+04 & Direct-PRF & 0\\
007031515-01 & RR-Lyr-pri & 1:1 & 1068.2 & 90 & -254 & 7.86 & 7.94 & 3.8956E+04 & Direct-PRF & 0\\
007031520-01 & RR-Lyr-pri & 1:1 & 1086.5 & 96 & -256 & 7.86 & 5.78 & 5.6663E+04 & Direct-PRF & 0\\
007031573-01 & RR-Lyr-pri & 1:1 & 924.4 & 65 & -224 & 7.86 & 7.32 & 2.9681E+04 & Direct-PRF & 0\\
007031638-01 & RR-Lyr-pri & 2:1 & 930.0 & 84 & -219 & 7.86 & 5.28 & 3.8956E+04 & Direct-PRF & 0\\
007031656-01 & RR-Lyr-pri & 1:1 & 926.9 & 87 & -217 & 7.86 & 6.42 & 3.6664E+04 & Direct-PRF & 0\\
007031659-01 & RR-Lyr-pri & 1:1 & 1124.8 & 137 & -248 & 7.86 & 4.47 & 1.2466E+05 & Direct-PRF & 0\\
007031716-01 & RR-Lyr-pri & 1:1 & 991.6 & 119 & -220 & 7.86 & 6.79 & 6.2330E+05 & Direct-PRF & 0\\
007031726-01 & RR-Lyr-pri & 1:1 & 842.6 & 83 & -195 & 7.86 & 3.61 & 2.1493E+04 & Direct-PRF & 0\\
007031732-01 & RR-Lyr-pri & 1:1 & 840.9 & 84 & -194 & 7.86 & 5.79 & 4.1553E+04 & Direct-PRF & 0\\
007031742-01 & RR-Lyr-pri & 1:1 & 939.7 & 112 & -209 & 7.86 & 7.47 & 2.8332E+04 & Direct-PRF & 0\\
007031753-01 & RR-Lyr-pri & 1:1 & 941.8 & 116 & -207 & 7.86 & 7.41 & 7.7912E+04 & Direct-PRF & 0\\
007031767-01 & RR-Lyr-pri & 1:1 & 1022.9 & 138 & -217 & 7.86 & 6.45 & 1.2878E+03 & Direct-PRF & 0\\
007031781-01 & RR-Lyr-pri & 1:1 & 960.1 & 127 & -206 & 7.86 & 7.96 & 7.4202E+03 & Direct-PRF & 0\\
007031824-01 & RR-Lyr-pri & 1:1 & 965.3 & 137 & -201 & 7.86 & 7.08 & 1.9478E+04 & Direct-PRF & 0\\
007031853-01 & RR-Lyr-pri & 1:1 & 960.8 & 141 & -196 & 7.86 & 7.70 & 3.6664E+04 & Direct-PRF & 0\\
007031880-01 & RR-Lyr-pri & 1:1 & 756.8 & 100 & -162 & 7.86 & 7.87 & 3.2805E+04 & Direct-PRF & 0\\
007031898-01 & RR-Lyr-pri & 1:1 & 859.6 & 126 & -176 & 7.86 & 5.12 & 4.4521E+04 & Direct-PRF & 0\\
007031904-01 & RR-Lyr-pri & 1:1 & 982.7 & 155 & -193 & 7.86 & 5.47 & 6.9255E+04 & Direct-PRF & 0\\
007031914-01 & RR-Lyr-pri & 1:1 & 916.7 & 141 & -183 & 7.86 & 8.00 & 6.2330E+05 & Direct-PRF & 0\\
007031942-01 & RR-Lyr-pri & 1:1 & 789.3 & 117 & -161 & 7.86 & 6.01 & 3.2805E+04 & Direct-PRF & 0\\
007031948-01 & RR-Lyr-pri & 1:1 & 774.0 & 115 & -158 & 7.86 & 7.90 & 1.6403E+04 & Direct-PRF & 0\\
007031992-01 & RR-Lyr-pri & 1:1 & 727.3 & 113 & -144 & 7.86 & 7.93 & 2.2261E+04 & Direct-PRF & 0\\
007032001-01 & RR-Lyr-pri & 1:1 & 919.0 & 157 & -170 & 7.86 & 6.98 & 1.8888E+04 & Direct-PRF & 0\\
007032116-01 & RR-Lyr-pri & 1:1 & 830.2 & 157 & -138 & 7.86 & 6.58 & 4.7946E+04 & Direct-PRF & 0\\
007032117-01 & RR-Lyr-pri & 1:1 & 854.6 & 162 & -141 & 7.86 & 7.01 & 1.3851E+04 & Direct-PRF & 0\\
007032132-01 & RR-Lyr-pri & 1:1 & 989.5 & 194 & -156 & 7.86 & 5.83 & 4.4521E+04 & Direct-PRF & 0\\
007032218-01 & RR-Lyr-pri & 1:1 & 741.3 & 151 & -110 & 7.86 & 5.08 & 8.9042E+04 & Direct-PRF & 0\\
007032274-01 & RR-Lyr-pri & 1:1 & 841.6 & 180 & -112 & 7.86 & 7.70 & 2.0777E+05 & Direct-PRF & 0\\
007032365-01 & RR-Lyr-pri & 1:1 & 791.9 & 179 & -87 & 7.86 & 7.32 & 3.8956E+04 & Direct-PRF & 0\\
007032369-01 & RR-Lyr-pri & 1:1 & 1018.9 & 228 & -117 & 7.86 & 7.42 & 2.2261E+04 & Direct-PRF & 0\\
007032383-01 & RR-Lyr-pri & 1:1 & 735.5 & 169 & -76 & 7.86 & 7.49 & 1.6846E+04 & Direct-PRF & 0\\
007032388-01 & RR-Lyr-pri & 1:1 & 900.7 & 204 & -98 & 7.86 & 5.98 & 4.1553E+04 & Direct-PRF & 0\\
007032429-01 & RR-Lyr-pri & 1:1 & 955.1 & 219 & -98 & 7.86 & 7.76 & 4.7946E+04 & Direct-PRF & 0\\
007032438-01 & RR-Lyr-pri & 1:1 & 782.4 & 183 & -73 & 7.86 & 7.88 & 3.2805E+04 & Direct-PRF & 0\\
007032456-01 & RR-Lyr-pri & 1:1 & 772.3 & 182 & -68 & 7.86 & 8.01 & 2.5971E+04 & Direct-PRF & 0\\
007032481-01 & RR-Lyr-pri & 1:1 & 746.4 & 178 & -59 & 7.86 & 7.17 & 2.0777E+05 & Direct-PRF & 0\\
007032524-01 & RR-Lyr-pri & 1:1 & 919.9 & 219 & -74 & 7.86 & 7.76 & 1.8888E+04 & Direct-PRF & 0\\
007032568-01 & RR-Lyr-pri & 1:1 & 772.4 & 189 & -46 & 7.86 & 5.97 & 7.7912E+04 & Direct-PRF & 0\\
007032687-01 & RR-Lyr-pri & 1:1 & 965.8 & 238 & -50 & 7.86 & 7.91 & 3.2805E+04 & Direct-PRF & 0\\
007032727-01 & RR-Lyr-pri & 1:1 & 766.7 & 192 & -14 & 7.86 & 7.17 & 1.6846E+04 & Direct-PRF & 0\\
007032807-01 & RR-Lyr-pri & 1:1 & 1072.4 & 266 & -43 & 7.86 & 7.97 & 1.6846E+04 & Direct-PRF & 0\\
007032923-01 & RR-Lyr-pri & 1:1 & 1093.7 & 275 & -14 & 7.86 & 6.72 & 5.1941E+04 & Direct-PRF & 0\\
007032938-01 & RR-Lyr-pri & 1:1 & 1135.4 & 285 & -17 & 7.86 & 8.06 & 6.2330E+05 & Direct-PRF & 0\\
007032946-01 & RR-Lyr-pri & 1:1 & 997.1 & 251 & 6 & 7.86 & 7.35 & 1.1543E+04 & Direct-PRF & 0\\
007032999-01 & RR-Lyr-pri & 1:1 & 945.6 & 236 & 30 & 7.86 & 8.12 & 6.2330E+05 & Direct-PRF & 0\\
007033044-01 & RR-Lyr-pri & 1:1 & 1026.8 & 257 & 28 & 7.86 & 7.50 & 2.0777E+04 & Direct-PRF & 0\\
007033389-01 & RR-Lyr-pri & 1:1 & 1210.9 & 286 & 103 & 7.86 & 7.32 & 3.8956E+04 & Direct-PRF & 0\\
007033421-01 & RR-Lyr-pri & 1:1 & 1232.1 & 289 & 110 & 7.86 & 6.69 & 2.9681E+04 & Direct-PRF & 0\\
007033713-01 & 007033748-pri & 1:2 & 30.6 & -8 & -2 & 13.69 & 2.13 & 3.1333E+03 & Direct-PRF & 0\\
007038096-01 & RR-Lyr-pri & 2:1 & 4900.3 & 836 & -1 & 7.86 & 6.79 & 6.6308E+03 & Col-Anomaly & 0\\
007038096-02 & RR-Lyr-pri & 1:1 & 4900.3 & 836 & -1 & 7.86 & 6.79 & 5.6663E+03 & Col-Anomaly & 0\\
007097534-01 & 007097571-pri & 1:1 & 39.6 & 5 & -8 & 11.27 & 3.19 & 1.8082E+03 & Direct-PRF & 0\\
007107561-01 & 5353.01 & 1:1 & 13.0 & 3 & -1 & 14.23 & -0.81 & 1.2729E+02 & Direct-PRF & 0\\
007115200-01 & RR-Lyr-pri & 1:1 & 1207.5 & -17 & -304 & 7.86 & 4.90 & 6.9255E+04 & Direct-PRF & 0\\
007115237-01 & RR-Lyr-pri & 1:1 & 1196.1 & -2 & -301 & 7.86 & 7.17 & 1.0252E+03 & Direct-PRF & 0\\
007115249-01 & RR-Lyr-pri & 1:1 & 1165.0 & -9 & -293 & 7.86 & 7.16 & 3.6664E+04 & Direct-PRF & 0\\
007115291-02 & RR-Lyr-pri & 1:1 & 1129.1 & -8 & -284 & 7.86 & 7.33 & 2.2261E+04 & Direct-PRF & 0\\
007115308-01 & RR-Lyr-pri & 1:1 & 1123.8 & -2 & -283 & 7.86 & 6.95 & 3.8956E+04 & Direct-PRF & 0\\
007115332-01 & RR-Lyr-pri & 1:1 & 1042.7 & -26 & -261 & 7.86 & 7.08 & 6.2330E+05 & Direct-PRF & 0\\
007115366-01 & RR-Lyr-pri & 1:1 & 1064.6 & -1 & -268 & 7.86 & 7.88 & 1.7314E+04 & Direct-PRF & 0\\
007115390-01 & RR-Lyr-pri & 1:1 & 983.9 & -26 & -247 & 7.86 & 8.10 & 6.2959E+03 & Direct-PRF & 0\\
007115427-01 & RR-Lyr-pri & 1:1 & 1002.4 & 5 & -253 & 7.86 & 7.21 & 6.2330E+05 & Direct-PRF & 0\\
007115463-01 & RR-Lyr-pri & 1:1 & 958.1 & 4 & -241 & 7.86 & 7.26 & 4.1553E+04 & Direct-PRF & 0\\
007115499-01 & RR-Lyr-pri & 1:1 & 863.4 & -19 & -217 & 7.86 & 7.78 & 1.3851E+04 & Direct-PRF & 0\\
007115530-01 & RR-Lyr-pri & 1:1 & 927.5 & 16 & -233 & 7.86 & 7.67 & 2.2261E+04 & Direct-PRF & 0\\
007115550-01 & RR-Lyr-pri & 1:1 & 956.7 & 30 & -239 & 7.86 & 6.36 & 2.3973E+04 & Direct-PRF & 0\\
007115597-01 & RR-Lyr-pri & 1:1 & 854.0 & 12 & -215 & 7.86 & 8.05 & 5.6153E+03 & Direct-PRF & 0\\
007115671-01 & RR-Lyr-pri & 1:1 & 855.9 & 36 & -213 & 7.86 & 5.99 & 1.0476E+03 & Direct-PRF & 0\\
007115733-01 & RR-Lyr-pri & 1:1 & 811.1 & 43 & -200 & 7.86 & 6.71 & 1.5202E+04 & Direct-PRF & 0\\
007115785-03 & RR-Lyr-pri & 1:1 & 733.4 & 39 & -181 & 7.86 & 6.14 & 2.3085E+04 & Direct-PRF & 0\\
007115816-01 & RR-Lyr-pri & 1:1 & 749.2 & 52 & -181 & 7.86 & 7.19 & 2.8332E+04 & Direct-PRF & 0\\
007115842-01 & RR-Lyr-pri & 1:1 & 687.3 & 41 & -168 & 7.86 & 6.25 & 4.1553E+04 & Direct-PRF & 0\\
007115869-01 & RR-Lyr-pri & 1:1 & 791.2 & 77 & -184 & 7.86 & 5.55 & 8.9042E+04 & Direct-PRF & 0\\
007115878-01 & RR-Lyr-pri & 1:1 & 563.9 & 15 & -142 & 7.86 & 7.04 & 2.0777E+04 & Direct-PRF & 0\\
007115879-01 & RR-Lyr-pri & 1:1 & 543.6 & 8 & -137 & 7.86 & 6.68 & 3.2805E+04 & Direct-PRF & 0\\
007115923-01 & RR-Lyr-pri & 1:1 & 578.5 & 33 & -142 & 7.86 & 5.93 & 5.6663E+04 & Direct-PRF & 0\\
007115925-01 & RR-Lyr-pri & 1:1 & 700.2 & 66 & -164 & 7.86 & 4.67 & 7.7912E+04 & Direct-PRF & 0\\
007116024-01 & RR-Lyr-pri & 6:1 & 643.7 & 73 & -145 & 7.86 & 4.20 & 3.2805E+04 & Direct-PRF & 0\\
007116043-01 & RR-Lyr-pri & 1:1 & 650.3 & 78 & -144 & 7.86 & 6.67 & 1.4840E+04 & Direct-PRF & 0\\
007116046-01 & RR-Lyr-pri & 1:1 & 690.5 & 88 & -150 & 7.86 & 7.95 & 1.2466E+04 & Direct-PRF & 0\\
007116166-01 & RR-Lyr-pri & 1:1 & 522.9 & 73 & -110 & 7.86 & 7.88 & 2.7100E+04 & Direct-PRF & 0\\
007116217-01 & RR-Lyr-pri & 1:1 & 539.5 & 87 & -105 & 7.86 & 7.59 & 2.0106E+04 & Direct-PRF & 0\\
007116226-01 & RR-Lyr-pri & 1:1 & 622.6 & 108 & -114 & 7.86 & 7.56 & 2.8332E+04 & Direct-PRF & 0\\
007116236-01 & RR-Lyr-pri & 1:1 & 615.6 & 108 & -112 & 7.86 & 7.81 & 2.0106E+04 & Direct-PRF & 0\\
007116282-01 & RR-Lyr-pri & 1:1 & 518.6 & 94 & -90 & 7.86 & 7.73 & 4.1553E+04 & Direct-PRF & 0\\
007116382-01 & RR-Lyr-pri & 1:1 & 307.9 & 63 & -45 & 7.86 & 7.91 & 1.4166E+04 & Direct-PRF & 0\\
007116466-01 & RR-Lyr-pri & 1:1 & 635.1 & 140 & -76 & 7.86 & 8.06 & 1.7314E+04 & Direct-PRF & 0\\
007116519-01 & RR-Lyr-pri & 1:1 & 608.1 & 139 & -64 & 7.86 & 7.91 & 6.3472E+02 & Direct-PRF & 0\\
007116561-01 & RR-Lyr-pri & 1:1 & 371.3 & 90 & -25 & 7.86 & 7.96 & 9.8936E+03 & Direct-PRF & 0\\
007116632-01 & RR-Lyr-pri & 1:1 & 378.1 & 94 & -13 & 7.86 & 8.04 & 1.1543E+04 & Direct-PRF & 0\\
007116670-01 & RR-Lyr-pri & 1:1 & 384.7 & 96 & -6 & 7.86 & 8.14 & 1.0746E+04 & Direct-PRF & 0\\
007116719-01 & RR-Lyr-pri & 1:1 & 387.9 & 97 & 6 & 7.86 & 7.55 & 8.9042E+03 & Direct-PRF & 0\\
007116766-01 & RR-Lyr-pri & 1:1 & 603.5 & 151 & -17 & 7.86 & 7.30 & 4.7946E+04 & Direct-PRF & 0\\
007116842-01 & RR-Lyr-pri & 1:1 & 718.8 & 180 & -15 & 7.86 & 6.19 & 1.0388E+05 & Direct-PRF & 0\\
007116849-01 & RR-Lyr-pri & 1:1 & 697.0 & 175 & -10 & 7.86 & 8.09 & 2.0106E+04 & Direct-PRF & 0\\
007116851-01 & RR-Lyr-pri & 1:1 & 684.9 & 172 & -8 & 7.86 & 7.69 & 7.0033E+03 & Direct-PRF & 0\\
007116851-02 & RR-Lyr-pri & 15:1 & 684.9 & 172 & -8 & 7.86 & 7.69 & 1.8939E+02 & Direct-PRF & 0\\
007116859-01 & RR-Lyr-pri & 1:1 & 691.3 & 174 & -8 & 7.86 & 7.30 & 1.4166E+04 & Direct-PRF & 0\\
007117020-01 & RR-Lyr-pri & 1:1 & 692.4 & 171 & 33 & 7.86 & 7.43 & 1.4495E+04 & Direct-PRF & 0\\
007117126-01 & RR-Lyr-pri & 1:1 & 820.3 & 202 & 43 & 7.86 & 5.86 & 3.8956E+04 & Direct-PRF & 0\\
007117147-01 & RR-Lyr-pri & 1:1 & 722.6 & 167 & 70 & 7.86 & 4.89 & 5.1941E+04 & Direct-PRF & 0\\
007117168-01 & RR-Lyr-pri & 1:1 & 871.2 & 214 & 47 & 7.86 & 5.62 & 8.9042E+04 & Direct-PRF & 0\\
007117178-01 & RR-Lyr-pri & 1:1 & 802.9 & 191 & 64 & 7.86 & 6.09 & 1.2466E+05 & Direct-PRF & 0\\
007117270-01 & RR-Lyr-pri & 1:1 & 841.2 & 193 & 85 & 7.86 & 7.52 & 2.4932E+04 & Direct-PRF & 0\\
007117284-01 & RR-Lyr-pri & 1:1 & 868.7 & 201 & 85 & 7.86 & 5.57 & 8.9042E+04 & Direct-PRF & 0\\
007117348-01 & RR-Lyr-pri & 1:1 & 994.2 & 237 & 78 & 7.86 & 7.34 & 9.8936E+03 & Direct-PRF & 0\\
007117355-01 & RR-Lyr-pri & 1:1 & 946.7 & 220 & 90 & 7.86 & 7.03 & 6.9255E+04 & Direct-PRF & 0\\
007117367-01 & RR-Lyr-pri & 1:1 & 989.0 & 234 & 84 & 7.86 & 6.34 & 5.1941E+04 & Direct-PRF & 0\\
007117413-01 & RR-Lyr-pri & 1:1 & 1050.7 & 249 & 87 & 7.86 & 7.52 & 6.7456E+02 & Direct-PRF & 0\\
007117436-01 & RR-Lyr-pri & 1:1 & 1054.7 & 247 & 95 & 7.86 & 7.22 & 5.6663E+04 & Direct-PRF & 0\\
007117444-01 & RR-Lyr-pri & 1:1 & 961.1 & 208 & 123 & 7.86 & 5.67 & 6.2330E+04 & Direct-PRF & 0\\
007117457-01 & RR-Lyr-pri & 1:1 & 1069.3 & 248 & 103 & 7.86 & 7.92 & 6.2330E+05 & Direct-PRF & 0\\
007117485-01 & RR-Lyr-pri & 1:1 & 1092.1 & 252 & 108 & 7.86 & 7.59 & 7.2392E+02 & Direct-PRF & 0\\
007117489-01 & RR-Lyr-pri & 1:1 & 957.4 & 188 & 150 & 7.86 & 6.97 & 1.1783E+03 & Direct-PRF & 0\\
007117492-01 & RR-Lyr-pri & 1:1 & 966.9 & 194 & 146 & 7.86 & 6.44 & 2.5971E+04 & Direct-PRF & 0\\
007117506-01 & RR-Lyr-pri & 1:1 & 1007.0 & 211 & 139 & 7.86 & 7.65 & 1.4495E+04 & Direct-PRF & 0\\
007117513-01 & RR-Lyr-pri & 1:1 & 987.0 & 198 & 149 & 7.86 & 8.05 & 7.6950E+03 & Direct-PRF & 0\\
007117549-01 & RR-Lyr-pri & 1:1 & 1027.3 & 208 & 152 & 7.86 & 7.20 & 1.2466E+05 & Direct-PRF & 0\\
007117561-01 & RR-Lyr-pri & 1:1 & 1043.5 & 216 & 149 & 7.86 & 7.95 & 1.3851E+04 & Direct-PRF & 0\\
007117568-01 & RR-Lyr-pri & 1:1 & 1064.2 & 225 & 145 & 7.86 & 6.67 & 2.0777E+05 & Direct-PRF & 0\\
007117585-02 & RR-Lyr-pri & 1:1 & 1043.4 & 208 & 160 & 7.86 & 7.16 & 5.1941E+04 & Direct-PRF & 0\\
007117710-01 & RR-Lyr-pri & 1:1 & 1146.0 & 231 & 172 & 7.86 & 5.82 & 3.4628E+04 & Direct-PRF & 0\\
007137725-01 & 007137798-pri & 1:1 & 48.7 & 12 & 0 & 13.45 & -0.33 & 2.2483E+03 & Direct-PRF & 0\\
007174351-01 & 3844.01 & 1:2 & 7.4 & -1 & -2 & 19.29 & -3.77 & 6.7920E+02 & Direct-PRF & 0\\
007177555-01 & 6837.01 & 1:1 & 8.8 & -1 & 2 & 11.51 & 3.33 & 6.6899E+00 & Direct-PRF & 0\\
007177555-02 & 007177553-sec & 1:1 & 8.8 & -1 & 2 & 11.51 & 3.33 & 5.8688E+00 & Direct-PRF & 0\\
007177766-01 & 007259917-pri & 2:1 & 494.9 & 124 & 0 & 12.13 & -0.08 & 1.4204E+04 & Col-Anomaly & 0\\
007198648-01 & RR-Lyr-pri & 1:1 & 267.9 & 2 & -68 & 7.86 & 7.66 & 8.4229E+03 & Direct-PRF & 0\\
007198734-01 & RR-Lyr-pri & 1:1 & 194.5 & 0 & -49 & 7.86 & 5.83 & 1.6984E+03 & Direct-PRF & 0\\
007198769-01 & RR-Lyr-pri & 1:1 & 184.7 & 9 & -46 & 7.86 & 7.93 & 7.7912E+04 & Direct-PRF & 0\\
007198769-02 & RR-Lyr-pri & 1:1 & 184.7 & 9 & -46 & 7.86 & 7.93 & 1.0564E+04 & Direct-PRF & 0\\
007198791-01 & RR-Lyr-pri & 1:1 & 233.3 & 25 & -53 & 7.86 & 7.96 & 6.2330E+05 & Direct-PRF & 0\\
007198817-01 & RR-Lyr-pri & 1:1 & 237.7 & 31 & -51 & 7.86 & 4.41 & 3.6664E+04 & Direct-PRF & 0\\
007198846-01 & RR-Lyr-pri & 1:1 & 124.3 & 10 & -30 & 7.86 & 6.12 & 1.1827E+03 & Direct-PRF & 0\\
007198881-01 & RR-Lyr-pri & 1:1 & 60.5 & -15 & -6 & 7.86 & 5.55 & 6.1536E+01 & Direct-PRF & 0\\
007198881-02 & RR-Lyr-pri & 1:1 & 60.5 & -15 & -6 & 7.86 & 5.55 & 3.1165E+03 & Direct-PRF & 0\\
007198941-01 & RR-Lyr-pri & 1:1 & 273.0 & 56 & -40 & 7.86 & 7.93 & 6.2330E+05 & Direct-PRF & 0\\
007199002-01 & RR-Lyr-pri & 1:1 & 175.6 & 39 & -21 & 7.86 & 7.71 & 6.2330E+05 & Direct-PRF & 0\\
007199010-01 & RR-Lyr-pri & 1:1 & 63.5 & 15 & -5 & 7.86 & 8.05 & 2.0777E+05 & Direct-PRF & 0\\
007199010-02 & RR-Lyr-pri & 1:1 & 63.5 & 15 & -5 & 7.86 & 8.05 & 9.5305E+02 & Direct-PRF & 0\\
007199037-01 & RR-Lyr-pri & 1:1 & 63.2 & 16 & 0 & 7.86 & 6.95 & 6.2330E+05 & Direct-PRF & 0\\
007199060-02 & RR-Lyr-pri & 1:1 & 275.8 & 64 & -26 & 7.86 & 5.11 & 2.2261E+04 & Direct-PRF & 0\\
007199087-01 & RR-Lyr-pri & 1:1 & 207.7 & 51 & -12 & 7.86 & 6.04 & 7.7912E+04 & Direct-PRF & 0\\
007199135-01 & RR-Lyr-pri & 5:1 & 120.7 & 22 & 20 & 7.86 & 7.69 & 2.3171E+03 & Direct-PRF & 0\\
007199135-02 & RR-Lyr-pri & 1:1 & 120.7 & 22 & 20 & 7.86 & 7.69 & 2.3754E+02 & Direct-PRF & 0\\
007199168-01 & RR-Lyr-pri & 1:1 & 284.0 & 71 & 1 & 7.86 & 7.84 & 1.3158E+02 & Direct-PRF & 0\\
007199203-01 & RR-Lyr-pri & 1:1 & 220.2 & 50 & 22 & 7.86 & 3.36 & 1.2466E+05 & Direct-PRF & 0\\
007199225-01 & RR-Lyr-pri & 1:1 & 211.0 & 18 & 49 & 7.86 & 3.81 & 6.2330E+05 & Direct-PRF & 0\\
007199235-01 & RR-Lyr-pri & 1:1 & 296.8 & 72 & 19 & 7.86 & 7.09 & 6.2330E+05 & Direct-PRF & 0\\
007199240-01 & RR-Lyr-pri & 1:1 & 259.1 & 58 & 29 & 7.86 & 7.19 & 8.0115E+02 & Direct-PRF & 0\\
007199272-01 & RR-Lyr-pri & 1:1 & 264.1 & 53 & 39 & 7.86 & 5.47 & 9.4439E+03 & Direct-PRF & 0\\
007199343-01 & RR-Lyr-pri & 1:1 & 369.4 & 85 & 37 & 7.86 & 7.70 & 6.2081E+02 & Direct-PRF & 0\\
007199351-01 & RR-Lyr-pri & 1:1 & 382.3 & 89 & 36 & 7.86 & 5.41 & 5.1941E+04 & Direct-PRF & 0\\
007199418-01 & RR-Lyr-pri & 1:1 & 374.4 & 72 & 60 & 7.86 & 7.59 & 6.2330E+05 & Direct-PRF & 0\\
007199644-01 & RR-Lyr-pri & 2:1 & 565.3 & 108 & 91 & 7.86 & 6.35 & 4.4521E+04 & Direct-PRF & 0\\
007199724-01 & RR-Lyr-pri & 1:1 & 644.9 & 131 & 95 & 7.86 & 6.69 & 3.8956E+04 & Direct-PRF & 0\\
007199756-01 & RR-Lyr-pri & 1:1 & 697.1 & 147 & 95 & 7.86 & 7.88 & 9.8936E+03 & Direct-PRF & 0\\
007199814-01 & RR-Lyr-pri & 1:1 & 725.8 & 148 & 106 & 7.86 & 7.42 & 1.7314E+04 & Direct-PRF & 0\\
007199883-01 & RR-Lyr-pri & 1:1 & 768.8 & 146 & 126 & 7.86 & 5.71 & 6.2330E+04 & Direct-PRF & 0\\
007199906-01 & RR-Lyr-pri & 1:1 & 808.4 & 165 & 118 & 7.86 & 7.27 & 6.2330E+05 & Direct-PRF & 0\\
007199917-01 & RR-Lyr-pri & 1:1 & 781.9 & 142 & 136 & 7.86 & 4.92 & 7.7912E+04 & Direct-PRF & 0\\
007199935-01 & RR-Lyr-pri & 1:1 & 794.7 & 145 & 136 & 7.86 & 5.52 & 3.6664E+04 & Direct-PRF & 0\\
007199989-01 & RR-Lyr-pri & 1:1 & 808.6 & 111 & 170 & 7.86 & 4.50 & 2.0777E+05 & Direct-PRF & 0\\
007200001-01 & RR-Lyr-pri & 1:1 & 824.9 & 132 & 159 & 7.86 & 6.93 & 3.1165E+04 & Direct-PRF & 0\\
007200012-01 & RR-Lyr-pri & 1:1 & 827.8 & 109 & 177 & 7.86 & 7.88 & 3.8956E+04 & Direct-PRF & 0\\
007200013-01 & RR-Lyr-pri & 1:1 & 842.9 & 142 & 157 & 7.86 & 7.61 & 8.7788E+03 & Direct-PRF & 0\\
007200014-01 & RR-Lyr-pri & 1:1 & 846.5 & 146 & 154 & 7.86 & 5.72 & 6.2330E+05 & Direct-PRF & 0\\
007200050-01 & RR-Lyr-pri & 1:1 & 868.0 & 145 & 163 & 7.86 & 7.48 & 6.2330E+05 & Direct-PRF & 0\\
007200156-01 & RR-Lyr-pri & 1:1 & 974.0 & 167 & 178 & 7.86 & 6.94 & 2.8332E+04 & Direct-PRF & 0\\
007200225-01 & RR-Lyr-pri & 1:1 & 997.8 & 145 & 204 & 7.86 & 7.47 & 6.2330E+05 & Direct-PRF & 0\\
007200269-01 & RR-Lyr-pri & 1:1 & 1033.4 & 152 & 210 & 7.86 & 4.53 & 6.2330E+04 & Direct-PRF & 0\\
007200301-01 & RR-Lyr-pri & 1:1 & 1066.9 & 164 & 212 & 7.86 & 6.84 & 3.1165E+04 & Direct-PRF & 0\\
007200303-01 & RR-Lyr-pri & 1:1 & 1063.4 & 151 & 220 & 7.86 & 7.83 & 1.9478E+04 & Direct-PRF & 0\\
007200359-01 & RR-Lyr-pri & 1:1 & 1116.2 & 141 & 242 & 7.86 & 7.27 & 3.6664E+04 & Direct-PRF & 0\\
007200373-01 & RR-Lyr-pri & 1:1 & 1135.2 & 181 & 220 & 7.86 & 7.01 & 2.4932E+04 & Direct-PRF & 0\\
007200457-01 & RR-Lyr-pri & 1:1 & 1200.5 & 178 & 244 & 7.86 & 7.76 & 1.8332E+04 & Direct-PRF & 0\\
007200463-01 & RR-Lyr-pri & 1:1 & 1228.9 & 212 & 224 & 7.86 & 7.96 & 2.0777E+04 & Direct-PRF & 0\\
007200485-01 & RR-Lyr-pri & 1:1 & 1236.2 & 200 & 237 & 7.86 & 7.25 & 1.3851E+04 & Direct-PRF & 0\\
007200506-01 & RR-Lyr-pri & 1:1 & 1243.8 & 184 & 252 & 7.86 & 7.39 & 1.8332E+04 & Direct-PRF & 0\\
007203194-01 & 6845.01 & 1:1 & 48.2 & -8 & -9 & 13.43 & 0.81 & 1.2604E+04 & Direct-PRF & 0\\
007204073-02 & RR-Lyr-pri & 1:1 & 4208.6 & 549 & -1 & 7.86 & 4.80 & 2.5971E+04 & Col-Anomaly & 0\\
007220322-01 & 3775.01 & 1:1 & 4.5 & 0 & -1 & 14.08 & -2.20 & 5.0394E+01 & Direct-PRF & 0\\
007257363-01 & 007257373-01 & 1:1 & 24.9 & 1 & 6 & 13.42 & 2.09 & 1.7985E+03 & Direct-PRF & 0\\
007258902-01 & 007258889-pri & 1:1 & 20.8 & 0 & -5 & 13.67 & 1.98 & 3.9190E+03 & Direct-PRF & 0\\
007280687-01 & RR-Lyr-pri & 1:1 & 85.8 & -17 & 13 & 7.86 & 5.69 & 6.2330E+05 & Direct-PRF & 0\\
007280785-01 & RR-Lyr-pri & 1:1 & 128.4 & -7 & 31 & 7.86 & 7.77 & 8.6569E+03 & Direct-PRF & 0\\
007280944-01 & RR-Lyr-pri & 1:1 & 237.1 & 14 & 57 & 7.86 & 4.87 & 3.1165E+05 & Direct-PRF & 0\\
007280953-01 & RR-Lyr-pri & 1:1 & 332.4 & -20 & 81 & 7.86 & 5.21 & 1.6403E+04 & Direct-PRF & 0\\
007281217-01 & RR-Lyr-pri & 1:1 & 521.8 & -5 & 131 & 7.86 & 7.78 & 6.2330E+05 & Direct-PRF & 0\\
007281301-01 & RR-Lyr-pri & 1:1 & 505.4 & 50 & 116 & 7.86 & 5.80 & 4.4521E+04 & Direct-PRF & 0\\
007281311-01 & RR-Lyr-pri & 1:1 & 513.6 & 44 & 121 & 7.86 & 7.98 & 1.9478E+04 & Direct-PRF & 0\\
007281356-01 & RR-Lyr-pri & 1:1 & 590.8 & 17 & 147 & 7.86 & 7.17 & 2.0777E+05 & Direct-PRF & 0\\
007281372-01 & RR-Lyr-pri & 1:1 & 565.8 & 50 & 133 & 7.86 & 7.79 & 6.2330E+05 & Direct-PRF & 0\\
007281399-01 & RR-Lyr-pri & 1:1 & 596.7 & 42 & 143 & 7.86 & 8.13 & 1.3550E+04 & Direct-PRF & 0\\
007281411-01 & RR-Lyr-pri & 1:1 & 602.9 & 45 & 144 & 7.86 & 7.91 & 2.0106E+04 & Direct-PRF & 0\\
007281454-01 & RR-Lyr-pri & 1:1 & 684.5 & 23 & 170 & 7.86 & 6.79 & 7.7912E+04 & Direct-PRF & 0\\
007281468-01 & RR-Lyr-pri & 1:1 & 652.0 & 55 & 154 & 7.86 & 7.26 & 2.9681E+04 & Direct-PRF & 0\\
007281484-01 & RR-Lyr-pri & 1:1 & 650.9 & 67 & 149 & 7.86 & 4.46 & 5.6663E+04 & Direct-PRF & 0\\
007281503-01 & RR-Lyr-pri & 1:1 & 664.8 & 76 & 148 & 7.86 & 7.93 & 2.0777E+04 & Direct-PRF & 0\\
007281615-01 & RR-Lyr-pri & 1:1 & 764.1 & 61 & 182 & 7.86 & 7.98 & 1.5582E+04 & Direct-PRF & 0\\
007281616-01 & RR-Lyr-pri & 1:1 & 791.7 & 41 & 194 & 7.86 & 8.03 & 1.1986E+04 & Direct-PRF & 0\\
007281644-01 & RR-Lyr-pri & 1:1 & 814.2 & 53 & 197 & 7.86 & 8.06 & 1.5202E+04 & Direct-PRF & 0\\
007281664-01 & RR-Lyr-pri & 1:1 & 805.1 & 85 & 183 & 7.86 & 7.98 & 1.2985E+04 & Direct-PRF & 0\\
007281668-01 & RR-Lyr-pri & 1:1 & 811.8 & 87 & 184 & 7.86 & 5.66 & 2.4932E+04 & Direct-PRF & 0\\
007281694-01 & RR-Lyr-pri & 1:1 & 837.9 & 93 & 189 & 7.86 & 6.04 & 2.4932E+04 & Direct-PRF & 0\\
007281699-01 & RR-Lyr-pri & 1:1 & 910.7 & 36 & 226 & 7.86 & 7.91 & 9.5892E+03 & Direct-PRF & 0\\
007281825-01 & RR-Lyr-pri & 1:1 & 1010.2 & 53 & 248 & 7.86 & 6.78 & 6.2330E+05 & Direct-PRF & 0\\
007281838-01 & RR-Lyr-pri & 1:1 & 958.6 & 113 & 212 & 7.86 & 8.10 & 1.3851E+04 & Direct-PRF & 0\\
007281856-01 & RR-Lyr-pri & 1:1 & 1011.4 & 72 & 243 & 7.86 & 5.97 & 2.5971E+04 & Direct-PRF & 0\\
007281864-01 & RR-Lyr-pri & 1:1 & 985.2 & 107 & 223 & 7.86 & 6.55 & 5.1941E+04 & Direct-PRF & 0\\
007281902-01 & RR-Lyr-pri & 1:1 & 1010.2 & 113 & 227 & 7.86 & 5.83 & 8.9042E+04 & Direct-PRF & 0\\
007281947-01 & RR-Lyr-pri & 1:1 & 1059.7 & 98 & 247 & 7.86 & 7.41 & 2.5971E+04 & Direct-PRF & 0\\
007281951-01 & RR-Lyr-pri & 1:1 & 1059.5 & 101 & 246 & 7.86 & 7.80 & 1.4166E+04 & Direct-PRF & 0\\
007281979-01 & RR-Lyr-pri & 1:1 & 1091.7 & 93 & 258 & 7.86 & 5.24 & 4.1553E+04 & Direct-PRF & 0\\
007281980-01 & RR-Lyr-pri & 1:1 & 1108.7 & 79 & 267 & 7.86 & 7.52 & 1.7314E+04 & Direct-PRF & 0\\
007282008-01 & RR-Lyr-pri & 1:1 & 1107.3 & 99 & 260 & 7.86 & 8.02 & 1.5982E+04 & Direct-PRF & 0\\
007282028-01 & RR-Lyr-pri & 1:1 & 1125.2 & 100 & 264 & 7.86 & 5.84 & 8.9042E+04 & Direct-PRF & 0\\
007282042-01 & RR-Lyr-pri & 1:1 & 1127.9 & 112 & 260 & 7.86 & 5.59 & 6.2330E+04 & Direct-PRF & 0\\
007282078-01 & RR-Lyr-pri & 1:1 & 1210.2 & 71 & 295 & 7.86 & 7.64 & 1.2466E+04 & Direct-PRF & 0\\
007282085-01 & RR-Lyr-pri & 1:1 & 1203.4 & 79 & 292 & 7.86 & 7.93 & 6.2330E+05 & Direct-PRF & 0\\
007282108-01 & RR-Lyr-pri & 1:1 & 1182.7 & 119 & 272 & 7.86 & 7.98 & 7.8898E+03 & Direct-PRF & 0\\
007282154-01 & RR-Lyr-pri & 1:1 & 1246.8 & 100 & 297 & 7.86 & 7.96 & 5.0716E+02 & Direct-PRF & 0\\
007282162-01 & RR-Lyr-pri & 1:1 & 1249.2 & 107 & 295 & 7.86 & 3.99 & 1.0388E+05 & Direct-PRF & 0\\
007282168-01 & RR-Lyr-pri & 1:1 & 1261.9 & 101 & 300 & 7.86 & 7.05 & 2.4932E+04 & Direct-PRF & 0\\
007282194-01 & RR-Lyr-pri & 1:1 & 1287.6 & 104 & 306 & 7.86 & 6.87 & 3.2805E+04 & Direct-PRF & 0\\
007282195-01 & RR-Lyr-pri & 1:1 & 1287.5 & 105 & 306 & 7.86 & 7.56 & 1.1130E+04 & Direct-PRF & 0\\
007285616-01 & RR-Lyr-pri & 1:1 & 4106.4 & 495 & -2 & 7.86 & 5.12 & 2.4932E+04 & Col-Anomaly & 0\\
007285673-01 & RR-Lyr-pri & 1:1 & 4147.3 & 521 & 0 & 7.86 & 6.64 & 8.2013E+03 & Col-Anomaly & 0\\
007289162-01 & 399.01 & 1:1 & 16.8 & -3 & -3 & 12.95 & 0.70 & 5.8523E+02 & Direct-PRF & 0\\
007289165-01 & 399.01 & 1:1 & 14.7 & 4 & 1 & 12.95 & -0.09 & 3.2010E+02 & Direct-PRF & 0\\
007289165-03 & 007289157-02 & 1:2 & 14.7 & 4 & 1 & 12.95 & -0.09 & 1.9024E+02 & Direct-PRF & 0\\
007293937-01 & 007374746-01 & 1:1 & 14.1 & -2 & -2 & 15.00 & -3.05 & 4.4348E+03 & Direct-PRF & 0\\
007296086-01 & 3790.01 & 1:1 & 9.4 & -2 & -1 & 18.59 & -3.97 & 9.3064E+02 & Direct-PRF & 0\\
007362301-01 & RR-Lyr-pri & 1:1 & 848.7 & -6 & 213 & 7.86 & 6.85 & 2.5971E+04 & Direct-PRF & 0\\
007362355-01 & RR-Lyr-pri & 1:1 & 868.4 & 10 & 218 & 7.86 & 6.45 & 4.7946E+04 & Direct-PRF & 0\\
007362364-01 & RR-Lyr-pri & 1:1 & 873.8 & 11 & 219 & 7.86 & 6.56 & 3.2805E+04 & Direct-PRF & 0\\
007362391-01 & RR-Lyr-pri & 1:1 & 903.1 & 9 & 226 & 7.86 & 6.53 & 2.7100E+04 & Direct-PRF & 0\\
007362420-01 & RR-Lyr-pri & 1:1 & 966.7 & -3 & 243 & 7.86 & 7.38 & 4.4521E+04 & Direct-PRF & 0\\
007362434-01 & RR-Lyr-pri & 1:1 & 971.0 & 2 & 244 & 7.86 & 7.90 & 1.8332E+04 & Direct-PRF & 0\\
007362450-01 & RR-Lyr-pri & 1:1 & 991.7 & -1 & 249 & 7.86 & 5.04 & 6.9255E+04 & Direct-PRF & 0\\
007362501-01 & RR-Lyr-pri & 1:1 & 1060.1 & -11 & 266 & 7.86 & 7.10 & 1.3550E+04 & Direct-PRF & 0\\
007362573-01 & RR-Lyr-pri & 1:1 & 1147.3 & -15 & 288 & 7.86 & 7.33 & 6.2330E+05 & Direct-PRF & 0\\
007362579-01 & RR-Lyr-pri & 1:1 & 1074.0 & 19 & 269 & 7.86 & 7.49 & 3.1165E+04 & Direct-PRF & 0\\
007362587-01 & RR-Lyr-pri & 1:1 & 1053.3 & 33 & 262 & 7.86 & 4.18 & 6.9255E+04 & Direct-PRF & 0\\
007362592-01 & RR-Lyr-pri & 1:1 & 1122.7 & 3 & 282 & 7.86 & 5.80 & 5.1941E+04 & Direct-PRF & 0\\
007362628-01 & RR-Lyr-pri & 1:1 & 1232.2 & -24 & 308 & 7.86 & 6.91 & 1.9478E+04 & Direct-PRF & 0\\
007362631-01 & RR-Lyr-pri & 1:1 & 1190.1 & -7 & 299 & 7.86 & 6.79 & 1.8888E+04 & Direct-PRF & 0\\
007362632-01 & RR-Lyr-pri & 1:1 & 1172.3 & 0 & 294 & 7.86 & 7.58 & 6.2330E+05 & Direct-PRF & 0\\
007362695-01 & RR-Lyr-pri & 1:1 & 1147.1 & 36 & 286 & 7.86 & 6.99 & 2.0777E+04 & Direct-PRF & 0\\
007362696-03 & RR-Lyr-pri & 1:1 & 1155.4 & 33 & 288 & 7.86 & 7.67 & 5.6663E+04 & Direct-PRF & 0\\
007366036-01 & RR-Lyr-pri & 1:1 & 3852.6 & 346 & -1 & 7.86 & 3.79 & 8.9042E+04 & Col-Anomaly & 0\\
007368137-01 & 007368103-pri & 1:1 & 21.7 & 3 & -5 & 13.42 & 1.48 & 1.7754E+03 & Direct-PRF & 0\\
007376490-01 & 3535.01 & 1:1 & 5.4 & -1 & 0 & 15.18 & -2.03 & 4.5346E+01 & Direct-PRF & 0\\
007376490-02 & 007376500-sec & 1:1 & 5.4 & -1 & 0 & 15.18 & -2.03 & 3.2517E+01 & Direct-PRF & 0\\
007376982-01 & 6848.01 & 1:1 & 1367.4 & 344 & 1 & 13.97 & -0.36 & 8.4643E+03 & Col-Anomaly & 0\\
007382263-01 & 007382250-pri & 1:1 & 27.4 & -5 & 4 & 12.01 & 3.11 & 1.0000E+03 & Direct-PRF & 0\\
007385387-01 & 007385478-pri & 1:1 & 66.0 & 16 & 2 & 11.47 & 4.40 & 1.9010E+03 & Direct-PRF & 0\\
007385509-01 & 007385478-pri & 1:1 & 18.4 & -4 & -3 & 11.47 & 2.37 & 2.6965E+02 & Direct-PRF & 0\\
007431709-01 & 007431703-pri & 1:1 & 65.4 & 8 & 15 & 12.25 & 2.83 & 7.3526E+03 & Direct-PRF & 0\\
007432476-02 & 007432479-pri & 2:1 & 4.3 & -1 & 1 & 14.54 & 1.07 & 2.2016E+02 & Direct-PRF & 0\\
007435780-01 & 007518816-pri & 2:1 & 40.3 & -1 & -10 & 12.85 & 2.17 & 5.3517E+03 & Direct-PRF & 0\\
007440062-01 & 007602309-01 & 1:1 & 1082.4 & -3 & -272 & 15.37 & -2.61 & 2.9403E-01 & Col-Anomaly & 1\\
007448023-01 & RR-Lyr-pri & 1:1 & 3776.6 & 295 & 1 & 7.86 & 7.82 & 7.3329E+03 & Col-Anomaly & 0\\
007458309-01 & 007458285-pri & 1:1 & 18.4 & 3 & -3 & 13.52 & 0.35 & 1.3884E+04 & Direct-PRF & 0\\
007458433-01 & 007458285-pri & 1:1 & 109.4 & 27 & -1 & 13.52 & 0.64 & 9.3811E+03 & Direct-PRF & 0\\
007461307-01 & 007461314-01 & 1:1 & 27.8 & -5 & -6 & 14.88 & -0.27 & 1.0702E+00 & Direct-PRF & 1\\
007461314-01 & 2909.01 & 1:1 & 27.8 & 5 & 6 & 14.62 & 0.27 & 1.2787E+00 & Direct-PRF & 1\\
007501259-01 & 007501230-pri & 1:1 & 65.9 & 16 & -4 & 12.45 & 1.74 & 1.2865E+04 & Direct-PRF & 0\\
007514582-01 & 007431703-pri & 1:1 & 79.0 & -2 & -20 & 12.25 & 3.08 & 7.1641E+03 & Direct-PRF & 0\\
007516354-01 & 007516345-pri & 2:1 & 12.4 & 0 & -3 & 12.32 & -0.89 & 5.3442E+03 & Direct-PRF & 0\\
007516379-02 & 007516345-pri & 2:1 & 71.2 & 0 & -18 & 12.32 & 2.51 & 9.5828E+03 & Direct-PRF & 0\\
007530366-01 & V2680-Cyg-pri & 1:1 & 40.9 & 10 & -1 & 14.70 & -6.33 & 4.5550E+05 & Direct-PRF & 0\\
007537849-01 & 007764561-01 & 1:1 & 2683.1 & -675 & 6 & 15.72 & -0.49 & 2.9937E+00 & Col-Anomaly & 1\\
007584755-01 & 007584739-pri & 1:1 & 29.7 & -3 & -7 & 13.38 & 0.80 & 1.6660E+04 & Direct-PRF & 0\\
007584778-01 & 007584826-pri & 1:1 & 105.1 & 27 & 1 & 15.19 & -0.67 & 4.3667E+03 & Col-Anomaly & 0\\
007602309-01 & 007440062-01 & 1:1 & 1082.4 & 3 & 272 & 12.76 & 2.61 & 3.4010E+00 & Col-Anomaly & 1\\
007609886-01 & RR-Lyr-pri & 1:1 & 3592.0 & 20 & 1 & 7.86 & 8.06 & 7.7912E+03 & Col-Anomaly & 0\\
007620660-02 & 007620664-pri & 1:1 & 10.5 & -2 & -2 & 13.11 & 2.37 & 4.2320E+03 & Direct-PRF & 0\\
007622059-02 & 6894.01 & 1:2 & 16.5 & -3 & -2 & 13.58 & -0.31 & 3.1696E+02 & Direct-PRF & 0\\
007622473-01 & 1447.01 & 1:1 & 14.1 & -4 & 1 & 13.09 & -0.78 & 9.0213E+02 & Direct-PRF & 0\\
007657926-01 & 007657914-pri & 2:1 & 50.8 & -6 & 11 & 12.91 & 1.88 & 7.8058E+03 & Direct-PRF & 0\\
007677313-01 & 007953701-01 & 1:1 & 2024.4 & -1 & -509 & 13.42 & 2.10 & 2.1195E+00 & Col-Anomaly & 1\\
007685693-01 & 007685689-pri & 2:1 & 6.0 & 1 & 0 & 15.54 & -1.59 & 2.5022E+03 & Direct-PRF & 0\\
007685693-02 & 007685689-pri & 2:1 & 6.0 & 1 & 0 & 15.54 & -1.59 & 4.9625E+01 & Direct-PRF & 0\\
007690855-02 & 007690843-pri & 2:1 & 15.2 & 4 & 0 & 11.08 & 2.96 & 6.0263E+00 & Direct-PRF & 0\\
007693494-01 & 007764546-01 & 1:1 & 648.8 & -163 & 3 & 15.13 & 0.34 & 4.6819E-01 & Col-Anomaly & 1\\
007695087-01 & 6041.01 & 1:1 & 8.5 & -1 & 2 & 13.86 & 0.87 & 7.7454E+01 & Direct-PRF & 0\\
007699298-01 & 007770471-01 & 1:1 & 617.8 & 155 & -1 & 14.62 & -1.07 & 2.6802E+04 & Col-Anomaly & 0\\
007700561-01 & 6908.01 & 1:1 & 16.9 & 2 & 3 & 14.15 & 1.39 & 1.0539E+03 & Direct-PRF & 0\\
007700578-01 & 007700590-01 & 1:1 & 9.2 & 1 & 3 & 14.85 & -0.70 & 1.0132E+00 & Direct-PRF & 0\\
007700590-01 & 6908.01 & 1:1 & 9.2 & -1 & -3 & 14.15 & 0.70 & 2.6437E+01 & Direct-PRF & 0\\
007707736-01 & 007707742-pri & 2:1 & 6.5 & -2 & 0 & 16.98 & -1.36 & 6.3952E+01 & Direct-PRF & 0\\
007707736-02 & 007707742-pri & 2:1 & 6.5 & -2 & 0 & 16.98 & -1.36 & 1.5398E+01 & Direct-PRF & 0\\
007708215-01 & 3666.01 & 1:1 & 11.1 & 3 & 0 & 15.99 & -0.73 & 9.6913E+01 & Direct-PRF & 0\\
007708215-02 & 3666.01 & 1:2 & 11.1 & 3 & 0 & 15.99 & -0.73 & 1.5872E+02 & Direct-PRF & 0\\
007747835-01 & 007953895-01 & 1:1 & 1640.3 & -6 & -412 & 15.14 & 0.05 & 1.2350E+00 & Col-Anomaly & 1\\
007751571-01 & 6912.01 & 1:1 & 6.1 & 0 & -1 & 15.25 & 0.32 & 1.6863E+01 & Direct-PRF & 0\\
007751571-02 & 007751562-02 & 1:1 & 6.1 & 0 & -1 & 15.25 & 0.32 & 8.9211E+00 & Direct-PRF & 0\\
007764546-01 & 007693494-01 & 1:1 & 648.8 & 163 & -3 & 15.47 & -0.34 & 2.1359E+00 & Col-Anomaly & 1\\
007764561-01 & 007537849-01 & 1:1 & 2683.1 & 675 & -6 & 15.23 & 0.49 & 3.3404E-01 & Col-Anomaly & 1\\
007766113-01 & 007766199-01 & 1:1 & 75.8 & -9 & 17 & 13.29 & 0.44 & 4.5455E-01 & Direct-PRF & 1\\
007766199-01 & 007766113-01 & 1:1 & 75.8 & 9 & -17 & 13.73 & -0.44 & 2.2000E+00 & Direct-PRF & 1\\
007766209-01 & 007766185-pri & 1:1 & 28.1 & 6 & 3 & 12.11 & 2.70 & 5.0063E+04 & Direct-PRF & 0\\
007770450-01 & 007770471-01 & 1:1 & 17.7 & 3 & 3 & 14.62 & 1.22 & 2.9330E+03 & Direct-PRF & 0\\
007777365-01 & 007777443-pri & 1:1 & 74.7 & -17 & -6 & 11.91 & 3.96 & 2.7357E+03 & Direct-PRF & 0\\
007777372-01 & 6916.01 & 2:1 & 84.8 & 10 & 18 & 15.87 & -1.72 & 2.0959E+00 & Direct-PRF & 1\\
007777372-02 & 007777443-pri & 2:1 & 53.7 & -7 & 12 & 11.91 & 2.24 & 3.9896E+03 & Direct-PRF & 0\\
007777397-01 & 007777416-02 & 2:1 & 9.7 & -3 & 0 & 15.30 & -3.71 & 9.0935E+00 & Direct-PRF & 0\\
007777397-02 & 007777416-01 & 1:1 & 9.7 & -3 & 0 & 15.30 & -3.71 & 8.5045E+00 & Direct-PRF & 0\\
007777471-01 & 007777443-pri & 1:1 & 64.8 & -3 & -16 & 11.91 & 2.63 & 5.1067E+03 & Direct-PRF & 0\\
007777522-01 & 007777443-pri & 1:1 & 56.9 & 15 & -1 & 11.91 & 3.85 & 4.1183E+03 & Direct-PRF & 0\\
007800750-01 & 007938870-pri & 1:1 & 682.7 & 172 & -1 & 12.29 & 1.11 & 2.3660E+04 & Col-Anomaly & 0\\
007812167-01 & 007812175-01 & 1:1 & 9.4 & 0 & -2 & 16.33 & -0.95 & 1.9595E+02 & Direct-PRF & 0\\
007812179-01 & 007812175-01 & 1:1 & 5.1 & 1 & 1 & 16.33 & -1.90 & 7.4029E+01 & Direct-PRF & 0\\
007812179-02 & 007812175-sec & 1:1 & 5.1 & 1 & 1 & 16.33 & -1.90 & 4.8189E+01 & Direct-PRF & 0\\
007816137-01 & 007816201-pri & 1:1 & 75.0 & -9 & 17 & 12.02 & 3.00 & 5.9654E+03 & Direct-PRF & 0\\
007816665-01 & 007816680-01 & 1:1 & 13.2 & -3 & 2 & 15.57 & 0.31 & 3.7897E+02 & Direct-PRF & 0\\
007818447-02 & 007818448-pri & 1:1 & 12.5 & 2 & 3 & 13.89 & -0.30 & 8.5952E+00 & Direct-PRF & 0\\
007835113-01 & 007835169-01 & 1:1 & 39.3 & -10 & -1 & 15.24 & 0.49 & 1.1666E+00 & Direct-PRF & 1\\
007835169-01 & 007835113-01 & 1:1 & 39.3 & 10 & 1 & 15.73 & -0.49 & 8.5718E-01 & Direct-PRF & 1\\
007838213-01 & 007838214-01 & 1:1 & 4.4 & 1 & -1 & 13.81 & 0.59 & 1.9167E+00 & Direct-PRF & 0\\
007838655-01 & 007838639-pri & 1:2 & 10.0 & -1 & -3 & 13.77 & 1.69 & 1.1680E+02 & Direct-PRF & 0\\
007840044-01 & 3758.01 & 1:1 & 6.8 & 0 & -2 & 16.90 & -2.37 & 1.0732E+02 & Direct-PRF & 0\\
007848303-02 & 009488426-01 & 1:4 & 9269.6 & -340 & -9 & 12.98 & -1.70 & 6.6667E-01 & Col-Anomaly & 1\\
007870250-01 & 007870306-01 & 1:1 & 77.2 & 15 & -11 & 15.11 & -0.54 & 1.6522E+00 & Direct-PRF & 1\\
007870282-01 & 007938870-pri & 1:1 & 46.1 & 12 & 2 & 12.29 & 2.94 & 4.4362E+03 & Direct-PRF & 0\\
007870306-01 & 007870250-01 & 1:1 & 77.2 & -15 & 11 & 14.57 & 0.54 & 6.0526E-01 & Direct-PRF & 1\\
007877818-01 & 3530.01 & 1:1 & 8.2 & -1 & -2 & 15.65 & -1.83 & 3.7361E+02 & Direct-PRF & 0\\
007877818-02 & 007877824-02 & 1:1 & 8.2 & -1 & -2 & 15.65 & -1.83 & 3.2526E+02 & Direct-PRF & 0\\
007877820-01 & 3530.01 & 1:1 & 4.7 & -1 & 0 & 15.65 & -2.55 & 4.1185E+01 & Direct-PRF & 0\\
007877820-02 & 007877824-02 & 1:1 & 4.7 & -1 & 0 & 15.65 & -2.55 & 3.9225E+01 & Direct-PRF & 0\\
007884866-01 & 007884842-pri & 1:1 & 20.6 & 3 & -4 & 9.60 & 5.64 & 2.2031E+02 & Direct-PRF & 0\\
007885494-01 & 007885570-pri & 1:1 & 85.3 & -10 & 20 & 11.68 & 3.98 & 2.1907E+03 & Direct-PRF & 0\\
007885558-01 & 007885570-pri & 1:2 & 31.4 & 2 & 8 & 11.68 & 3.22 & 2.6079E+03 & Direct-PRF & 0\\
007889486-01 & 007821010-02 & 1:1 & 106.6 & -14 & 23 & 10.82 & 4.94 & 1.2003E+03 & Direct-PRF & 0\\
007889486-02 & 007821010-01 & 1:1 & 106.6 & -14 & 23 & 10.82 & 4.94 & 9.2306E+02 & Direct-PRF & 0\\
007901074-01 & 007970427-01 & 1:1 & 557.6 & -140 & -4 & 15.24 & 0.35 & 4.5875E-01 & Col-Anomaly & 1\\
007918172-02 & 007918217-01 & 1:1 & 25.6 & -7 & 1 & 10.88 & 3.46 & 1.3004E+00 & Direct-PRF & 0\\
007918217-01 & 007918172-sec & 1:3 & 25.6 & 7 & -1 & 14.34 & -3.46 & 1.3915E+00 & Direct-PRF & 1\\
007938180-01 & 007938179-01 & 1:1 & 5.3 & 0 & 1 & 11.45 & 2.17 & 3.5789E+00 & Direct-PRF & 0\\
007938499-01 & V481-Lyr-pri & 1:1 & 71.3 & -1 & 18 & 13.27 & 1.67 & 3.9411E+03 & Direct-PRF & 0\\
007953701-01 & 007677313-01 & 1:1 & 2024.4 & 1 & 509 & 15.52 & -2.10 & 4.7182E-01 & Col-Anomaly & 1\\
007953895-01 & 007747835-01 & 1:1 & 1640.3 & 6 & 412 & 15.19 & -0.05 & 8.0973E-01 & Col-Anomaly & 1\\
007953935-01 & 007953895-01 & 1:1 & 52.8 & 13 & 3 & 15.14 & 0.26 & 6.9970E-01 & Direct-PRF & 1\\
007953935-02 & 008023034-01 & 1:1 & 517.5 & -130 & 0 & 14.38 & 1.02 & 4.3863E-01 & Col-Anomaly & 1\\
007968400-01 & 007968451-01 & 1:1 & 67.5 & -4 & -17 & 15.47 & -0.03 & 1.2745E+00 & Direct-PRF & 1\\
007968451-01 & 007968400-01 & 1:1 & 67.5 & 4 & 17 & 15.44 & 0.03 & 7.8463E-01 & Direct-PRF & 1\\
007968859-01 & 008107473-01 & 1:1 & 1004.6 & -252 & -5 & 14.70 & -0.14 & 1.0455E+00 & Col-Anomaly & 1\\
007970427-01 & 007901074-01 & 1:1 & 557.6 & 140 & 4 & 15.59 & -0.35 & 2.1798E+00 & Col-Anomaly & 1\\
007970969-01 & 007970972-01 & 1:1 & 68.7 & 9 & -15 & 15.85 & -0.27 & 2.3023E+00 & Direct-PRF & 1\\
007970972-01 & 007970969-01 & 1:1 & 68.7 & -9 & 15 & 15.58 & 0.27 & 4.3434E-01 & Direct-PRF & 1\\
007988303-01 & 007988343-02 & 1:2 & 29.0 & -4 & 7 & 14.49 & -0.56 & 6.2200E+01 & Direct-PRF & 0\\
008009496-01 & 6951.01 & 10:1 & 15.3 & 2 & 3 & 14.58 & -1.18 & 4.1034E+01 & Direct-PRF & 0\\
008009496-02 & 6951.01 & 10:1 & 15.3 & 2 & 3 & 14.58 & -1.18 & 5.5789E+01 & Direct-PRF & 0\\
008009496-03 & 6951.01 & 1:1 & 15.3 & 2 & 3 & 14.58 & -1.18 & 8.0290E+02 & Direct-PRF & 0\\
008016211-01 & 6953.01 & 1:1 & 11.2 & 0 & -3 & 14.36 & 0.03 & 2.0330E+02 & Direct-PRF & 0\\
008022815-01 & 008092488-01 & 1:1 & 970.8 & -244 & -3 & 15.08 & -0.98 & 2.4050E+00 & Col-Anomaly & 1\\
008023034-01 & 007953935-02 & 1:1 & 517.5 & 130 & 0 & 15.40 & -1.02 & 2.2798E+00 & Col-Anomaly & 1\\
008029197-01 & 6964.01 & 1:2 & 293.3 & 74 & -1 & 12.82 & -0.17 & 1.0188E+04 & Col-Anomaly & 0\\
008036315-01 & V1264-Cyg-pri & 1:1 & 1929.5 & 337 & 351 & 6.71 & 5.04 & 4.5869E+03 & Direct-PRF & 0\\
008038392-01 & 008176865-01 & 1:1 & 1455.2 & -366 & -2 & 15.93 & -0.57 & 1.1809E+00 & Col-Anomaly & 1\\
008038823-01 & 008038865-01 & 1:1 & 52.9 & -14 & 1 & 14.32 & 1.22 & 5.5571E-01 & Direct-PRF & 1\\
008038865-01 & 008038823-01 & 1:1 & 52.9 & 14 & -1 & 15.54 & -1.22 & 1.7995E+00 & Direct-PRF & 1\\
008043882-01 & 5469.01 & 1:1 & 60.1 & 15 & -2 & 15.29 & -0.08 & 1.3016E+00 & Direct-PRF & 1\\
008043968-01 & 008043961-pri & 1:1 & 83.8 & -11 & -17 & 10.74 & 4.56 & 2.8338E+03 & Direct-PRF & 0\\
008043968-02 & 008043961-sec & 1:1 & 83.8 & -11 & -17 & 10.74 & 4.56 & 2.6957E+03 & Direct-PRF & 0\\
008044016-01 & 4812.01 & 1:1 & 252.7 & -63 & 1 & 15.70 & -1.96 & 4.2500E+00 & Col-Anomaly & 1\\
008058135-01 & 008058127-01 & 2:1 & 5.8 & 1 & -1 & 13.47 & 0.45 & 4.7609E+00 & Direct-PRF & 0\\
008092039-01 & 008229100-01 & 1:1 & 1194.3 & -300 & -3 & 15.19 & -0.43 & 1.5433E+00 & Col-Anomaly & 1\\
008092488-01 & 008160817-01 & 1:1 & 74.1 & -16 & -10 & 14.41 & 0.67 & 3.3549E-01 & Direct-PRF & 1\\
008094120-01 & 6961.01 & 1:1 & 30.1 & 0 & 8 & 15.16 & -2.27 & 1.0702E+04 & Direct-PRF & 0\\
008095110-01 & 6171.01 & 1:1 & 5.4 & 2 & 0 & 14.17 & -1.00 & 1.5424E+01 & Direct-PRF & 0\\
008097897-01 & 008097902-pri & 2:1 & 7.1 & 1 & 1 & 16.38 & -0.53 & 6.1702E+02 & Direct-PRF & 0\\
008104065-02 & 912.01 & 9:1 & 4475.2 & -833 & 1 & 15.06 & -1.44 & 5.5158E+00 & Col-Anomaly & 1\\
008104436-01 & 006706287-pri & 1:1 & 7756.9 & -2 & 1 & 13.62 & 1.94 & 1.9815E+03 & Cross-Talk & 0\\
008107115-01 & 008244179-01 & 1:1 & 1313.5 & -330 & 1 & 15.12 & 0.25 & 1.4673E+00 & Col-Anomaly & 1\\
008107143-01 & 008244123-01 & 1:1 & 1216.9 & -305 & 0 & 14.60 & 1.26 & 2.7825E-01 & Col-Anomaly & 1\\
008107473-01 & 007968859-01 & 1:1 & 1004.6 & 252 & 5 & 14.55 & 0.14 & 9.5652E-01 & Col-Anomaly & 1\\
008108014-01 & 008038392-01 & 1:1 & 928.8 & 233 & 4 & 15.35 & -0.74 & 1.3106E+00 & Col-Anomaly & 1\\
008108870-01 & 008108933-01 & 1:1 & 55.9 & -14 & -3 & 14.59 & -0.58 & 2.3087E+00 & Direct-PRF & 1\\
008108933-01 & 008108870-01 & 1:1 & 55.9 & 14 & 3 & 14.01 & 0.58 & 4.3315E-01 & Direct-PRF & 1\\
008127586-01 & 1919.01 & 1:1 & 19.7 & 3 & 3 & 14.66 & 0.27 & 2.3688E+00 & Direct-PRF & 0\\
008127639-01 & 3713.01 & 1:1 & 10.0 & 3 & 0 & 17.51 & -2.12 & 3.9886E+02 & Direct-PRF & 0\\
008128247-01 & 008128965-pri & 1:2 & 486.9 & 122 & 0 & 13.23 & 0.10 & 3.1000E+03 & Col-Anomaly & 0\\
008129005-01 & 008128965-pri & 1:2 & 27.9 & -7 & -3 & 13.23 & 1.51 & 2.5095E+03 & Direct-PRF & 0\\
008129631-01 & 008129641-01 & 1:1 & 8.3 & 1 & 1 & 15.94 & -4.78 & 2.2057E+01 & Direct-PRF & 0\\
008145462-01 & 008145477-pri & 1:1 & 20.8 & 3 & -5 & 14.79 & 0.29 & 2.7666E+02 & Direct-PRF & 0\\
008149484-02 & 6958.01 & 1:1 & 229.3 & 58 & 0 & 13.99 & -0.90 & 1.2805E+04 & Col-Anomaly & 0\\
008159807-01 & 008160030-01 & 1:1 & 289.0 & -73 & -1 & 15.99 & -3.95 & 5.6670E-01 & Col-Anomaly & 1\\
008160030-01 & 008159807-01 & 1:1 & 289.0 & 73 & 1 & 12.04 & 3.95 & 1.7646E+00 & Col-Anomaly & 1\\
008160817-01 & 008092488-01 & 1:1 & 74.1 & 16 & 10 & 15.08 & -0.67 & 2.9807E+00 & Direct-PRF & 1\\
008160897-01 & 008229100-01 & 1:1 & 543.2 & -136 & 3 & 15.19 & -0.83 & 2.2448E+00 & Col-Anomaly & 1\\
008160932-01 & 008362712-01 & 1:1 & 1926.3 & -484 & 1 & 14.67 & -1.19 & 1.5695E-01 & Col-Anomaly & 1\\
008161707-01 & 008161830-01 & 1:2 & 121.8 & -23 & 20 & 13.31 & 0.97 & 8.6364E-01 & Direct-PRF & 1\\
008161798-03 & 008161825-01 & 1:1 & 95.1 & -18 & -15 & 11.52 & -1.05 & 7.0000E-01 & Direct-PRF & 1\\
008161816-01 & 008161830-01 & 1:1 & 24.2 & 0 & 6 & 13.31 & 2.23 & 3.7255E-01 & Direct-PRF & 1\\
008161825-01 & 008161798-03 & 1:1 & 95.1 & 18 & 15 & 10.47 & 1.05 & 1.4286E+00 & Direct-PRF & 1\\
008161830-01 & 008161816-01 & 1:1 & 24.2 & 0 & -6 & 15.54 & -2.23 & 2.6842E+00 & Direct-PRF & 1\\
008162376-01 & 6961.01 & 1:1 & 102.9 & 26 & 0 & 15.16 & -1.16 & 7.4912E+03 & Direct-PRF & 0\\
008162790-01 & 521.01 & 1:1 & 3.4 & 0 & -1 & 14.63 & 0.41 & 1.8890E+00 & Direct-PRF & 0\\
008176072-01 & 008176161-01 & 1:1 & 86.7 & -21 & -2 & 14.88 & 0.34 & 6.1415E-01 & Col-Anomaly & 1\\
008176161-01 & 008806072-02 & 1:1 & 24113.3 & 146 & -130 & 14.86 & 0.02 & 9.2408E-01 & Reflection & 1\\
008176865-01 & 008038392-01 & 1:1 & 1455.2 & 366 & 2 & 15.35 & 0.57 & 8.4683E-01 & Col-Anomaly & 1\\
008228228-01 & 008362237-01 & 1:1 & 1640.3 & -413 & 5 & 15.69 & -0.02 & 5.9898E-01 & Col-Anomaly & 1\\
008228396-01 & 008295843-01 & 1:1 & 969.0 & -243 & 4 & 15.96 & -0.90 & 2.1045E+00 & Col-Anomaly & 1\\
008228620-01 & 008228624-01 & 1:1 & 63.6 & 8 & 14 & 14.89 & -0.00 & 4.6971E-01 & Direct-PRF & 1\\
008228624-01 & 008228620-01 & 1:1 & 63.6 & -8 & -14 & 14.89 & 0.00 & 2.1290E+00 & Direct-PRF & 1\\
008228631-01 & 008295843-01 & 1:1 & 769.7 & -193 & -1 & 15.96 & -0.66 & 1.3512E+00 & Col-Anomaly & 1\\
008229100-01 & 008092039-01 & 1:1 & 1194.3 & 300 & 3 & 14.77 & 0.43 & 6.4798E-01 & Col-Anomaly & 1\\
008240109-02 & 3826.01 & 1:2 & 11.7 & -2 & -2 & 15.82 & -2.33 & 5.0666E+00 & Direct-PRF & 0\\
008240109-03 & 3826.01 & 2:1 & 11.7 & -2 & -2 & 15.82 & -2.33 & 1.6403E+01 & Direct-PRF & 0\\
008240123-01 & 008240109-pri & 1:1 & 11.7 & 2 & 2 & 13.49 & 2.33 & 9.4162E+01 & Direct-PRF & 0\\
008240123-02 & 008240109-sec & 1:1 & 11.7 & 2 & 2 & 13.49 & 2.33 & 3.2143E+01 & Direct-PRF & 0\\
008240915-01 & 008374321-02 & 1:1 & 1354.0 & -340 & 3 & 15.48 & 0.24 & 1.6829E+00 & Col-Anomaly & 1\\
008243283-01 & 008243263-pri & 1:2 & 16.1 & 3 & 2 & 12.98 & 2.24 & 2.5217E+02 & Direct-PRF & 0\\
008244123-01 & 008107143-01 & 1:1 & 1216.9 & 305 & 0 & 15.86 & -1.26 & 3.5939E+00 & Col-Anomaly & 1\\
008244179-01 & 008107115-01 & 1:1 & 1313.5 & 330 & -1 & 15.37 & -0.25 & 6.8150E-01 & Col-Anomaly & 1\\
008244190-01 & 3545.01 & 1:1 & 13.7 & 3 & 3 & 15.90 & -1.40 & 4.3533E+03 & Direct-PRF & 0\\
008244295-02 & 3545.01 & 1:1 & 111.4 & 28 & 0 & 15.90 & 0.03 & 4.2687E+03 & Col-Anomaly & 0\\
008245108-01 & 008311255-pri & 1:1 & 46.7 & 7 & 9 & 13.67 & 2.15 & 5.4852E+03 & Direct-PRF & 0\\
008256049-01 & 3652.01 & 1:1 & 7.9 & 2 & -1 & 15.88 & -0.22 & 2.5857E+01 & Direct-PRF & 0\\
008258171-01 & 3870.01 & 1:1 & 9.3 & 2 & -2 & 16.38 & -4.73 & 7.2175E+01 & Direct-PRF & 0\\
008258171-02 & 008258160-02 & 1:1 & 9.3 & 2 & -2 & 16.38 & -4.73 & 4.8737E+01 & Direct-PRF & 0\\
008260234-01 & 1066.01 & 1:1 & 9.6 & 3 & 0 & 15.62 & -1.46 & 5.2220E+01 & Direct-PRF & 0\\
008262210-01 & 008262223-pri & 1:1 & 26.7 & -1 & 6 & 12.15 & 1.80 & 1.9475E+03 & Direct-PRF & 0\\
008263752-01 & 3581.01 & 1:1 & 7.4 & 0 & -1 & 16.75 & -3.32 & 1.2395E+02 & Direct-PRF & 0\\
008263752-02 & 008263746-02 & 1:1 & 7.4 & 0 & -1 & 16.75 & -3.32 & 8.9548E+01 & Direct-PRF & 0\\
008264070-01 & 3655.01 & 1:1 & 14.0 & 3 & 2 & 17.69 & -2.65 & 3.8257E+02 & Direct-PRF & 0\\
008265269-01 & 008265951-pri & 1:1 & 539.2 & 135 & 0 & 12.73 & 0.26 & 2.4500E+04 & Col-Anomaly & 0\\
008265921-01 & 008265953-01 & 1:1 & 86.6 & 14 & -17 & 15.31 & -1.38 & 3.0667E+00 & Direct-PRF & 1\\
008265953-01 & 008265993-01 & 1:1 & 54.3 & 4 & 13 & 13.03 & 2.28 & 2.6087E-01 & Direct-PRF & 1\\
008265993-01 & 008265953-01 & 1:1 & 54.3 & -4 & -13 & 15.31 & -2.28 & 3.8333E+00 & Direct-PRF & 1\\
008295605-01 & 008295843-01 & 1:1 & 228.3 & -57 & -3 & 15.96 & -0.68 & 1.4100E+00 & Col-Anomaly & 1\\
008295843-01 & 008228631-01 & 1:1 & 769.7 & 193 & 1 & 15.30 & 0.66 & 7.4007E-01 & Col-Anomaly & 1\\
008296401-01 & 008362170-01 & 1:1 & 61.0 & 1 & -15 & 15.83 & -0.19 & 1.4331E+00 & Direct-PRF & 1\\
008299955-01 & 3631.01 & 1:1 & 11.2 & -2 & -2 & 17.74 & -4.27 & 5.7498E+03 & Direct-PRF & 0\\
008302450-01 & 008302455-01 & 1:1 & 73.9 & 11 & -15 & 11.54 & 3.75 & 4.4492E+02 & Direct-PRF & 0\\
008302473-01 & 008302455-01 & 1:1 & 56.4 & -10 & 9 & 11.54 & 4.08 & 8.0384E+02 & Direct-PRF & 0\\
008308199-01 & 008308832-01 & 1:1 & 594.7 & -150 & 0 & 15.97 & -1.08 & 1.5054E+00 & Col-Anomaly & 1\\
008308352-01 & 008308347-01 & 1:1 & 5.1 & 1 & 0 & 15.47 & -0.37 & 3.6962E+00 & Direct-PRF & 0\\
008308832-01 & 008308199-01 & 1:1 & 594.7 & 150 & 0 & 14.89 & 1.08 & 6.6430E-01 & Col-Anomaly & 1\\
008314870-01 & 008314879-pri & 1:1 & 21.7 & -2 & -6 & 15.62 & -0.10 & 9.2297E+03 & Direct-PRF & 0\\
008323753-01 & 3767.01 & 1:1 & 7.7 & -2 & 0 & 17.38 & -3.89 & 1.5398E+02 & Direct-PRF & 0\\
008330548-01 & 7020.01 & 1:1 & 12.3 & 2 & 3 & 13.48 & 0.96 & 7.5234E+00 & Direct-PRF & 0\\
008358012-01 & 7022.01 & 1:1 & 10.9 & 3 & 0 & 14.67 & 0.22 & 3.2559E+01 & Direct-PRF & 0\\
008358012-02 & 008358008-02 & 1:1 & 10.9 & 3 & 0 & 14.67 & 0.22 & 3.7957E+01 & Direct-PRF & 0\\
008362170-01 & 008296401-01 & 1:1 & 61.0 & -1 & 15 & 15.63 & 0.19 & 6.9779E-01 & Direct-PRF & 1\\
008362237-01 & 008228228-01 & 1:1 & 1640.3 & 413 & -5 & 15.67 & 0.02 & 1.6695E+00 & Col-Anomaly & 1\\
008362442-01 & 008362455-01 & 1:1 & 41.8 & -9 & -5 & 15.22 & 0.08 & 1.2412E+00 & Direct-PRF & 1\\
008362455-01 & 008362442-01 & 1:1 & 41.8 & 9 & 5 & 15.30 & -0.08 & 8.0569E-01 & Direct-PRF & 1\\
008362712-01 & 008160932-01 & 1:1 & 1926.3 & 484 & -1 & 13.48 & 1.19 & 6.3715E+00 & Col-Anomaly & 1\\
008364115-01 & 7024.01 & 1:1 & 19.3 & -2 & 4 & 12.41 & 0.83 & 6.9792E+02 & Direct-PRF & 0\\
008364115-02 & 008364119-02 & 1:1 & 19.3 & -2 & 4 & 12.41 & 0.83 & 7.0886E+02 & Direct-PRF & 0\\
008373873-01 & 008373988-01 & 1:1 & 84.9 & -19 & -9 & 14.00 & 0.54 & 5.5436E-01 & Direct-PRF & 1\\
008373988-01 & 008373873-01 & 1:1 & 84.9 & 19 & 9 & 14.54 & -0.54 & 1.8039E+00 & Direct-PRF & 1\\
008374321-02 & 008240915-01 & 1:1 & 1354.0 & 340 & -3 & 15.72 & -0.24 & 5.9422E-01 & Col-Anomaly & 1\\
008374494-01 & 7026.01 & 1:1 & 8.3 & -1 & -2 & 14.91 & 0.84 & 3.3309E+01 & Direct-PRF & 0\\
008374494-02 & 008374499-sec & 1:1 & 8.3 & -1 & -2 & 14.91 & 0.84 & 4.6461E+01 & Direct-PRF & 0\\
008374896-01 & 008547387-01 & 1:1 & 22905.5 & 101 & -121 & 15.98 & -0.91 & 1.7534E+00 & Reflection & 1\\
008378634-01 & 008378656-pri & 1:1 & 14.2 & 3 & -1 & 12.79 & 0.27 & 4.5127E+02 & Direct-PRF & 0\\
008378634-02 & 008378656-sec & 1:1 & 14.2 & 3 & -1 & 12.79 & 0.27 & 9.0500E+02 & Direct-PRF & 0\\
008382075-01 & 008382182-pri & 1:1 & 82.7 & 14 & -16 & 8.18 & 6.78 & 2.6727E+02 & Direct-PRF & 0\\
008382091-01 & 008382182-pri & 1:1 & 92.9 & 23 & 7 & 8.18 & 7.33 & 4.3235E+02 & Direct-PRF & 0\\
008382114-01 & 008382182-pri & 2:1 & 57.8 & 7 & -13 & 8.18 & 7.10 & 2.8824E+02 & Direct-PRF & 0\\
008382207-01 & 008382182-pri & 1:1 & 25.3 & -5 & -3 & 8.18 & 5.48 & 2.9400E+03 & Direct-PRF & 0\\
008382223-01 & 008382182-pri & 1:1 & 82.9 & 5 & 20 & 8.18 & 7.81 & 1.7711E+02 & Direct-PRF & 0\\
008386035-01 & 008386048-pri & 1:1 & 11.8 & -2 & 2 & 16.65 & -4.00 & 3.0146E+04 & Direct-PRF & 0\\
008410668-01 & 008410637-pri & 1:1 & 52.4 & -1 & 13 & 10.77 & -0.00 & 1.1186E+02 & Direct-PRF & 0\\
008414216-01 & 7035.01 & 1:1 & 111.1 & 28 & 0 & 14.38 & -0.38 & 2.6962E+03 & Col-Anomaly & 0\\
008414907-01 & 5513.01 & 1:1 & 5.2 & -1 & -1 & 17.91 & -2.13 & 1.0028E+02 & Direct-PRF & 0\\
008414907-02 & 008414914-02 & 1:1 & 5.2 & -1 & -1 & 17.91 & -2.13 & 9.1742E+01 & Direct-PRF & 0\\
008429415-01 & 7039.01 & 1:1 & 28.6 & 7 & -1 & 13.11 & -0.40 & 9.7955E+03 & Direct-PRF & 0\\
008453211-01 & 7043.01 & 1:1 & 14.4 & 3 & 0 & 13.36 & 1.22 & 1.0537E+02 & Direct-PRF & 0\\
008453214-01 & 7043.01 & 1:1 & 15.8 & 3 & -2 & 13.36 & 2.11 & 9.4867E+01 & Direct-PRF & 0\\
008460634-01 & 1730.01 & 1:1 & 22.0 & -6 & -1 & 14.93 & -3.26 & 5.5243E+02 & Direct-PRF & 0\\
008474898-01 & 5520.01 & 1:1 & 7.5 & -1 & 2 & 14.37 & 0.17 & 4.9756E+00 & Direct-PRF & 0\\
008487645-01 & 7054.01 & 1:1 & 125.7 & -31 & 0 & 10.29 & 2.43 & 3.1387E+04 & Direct-PRF & 0\\
008487748-01 & 008552540-01 & 1:1 & 102.6 & -3 & 25 & 10.29 & 5.16 & 1.6903E+03 & Direct-PRF & 0\\
008487805-01 & 008552540-01 & 1:1 & 154.7 & 16 & 35 & 10.29 & 4.76 & 5.8840E+03 & Direct-PRF & 0\\
008487838-01 & 008552540-01 & 1:2 & 223.6 & 17 & 54 & 10.29 & 3.88 & 1.4086E+04 & Direct-PRF & 0\\
008488876-01 & 1248.01 & 1:1 & 5.5 & -1 & 1 & 15.36 & -2.99 & 1.2979E+00 & Direct-PRF & 0\\
008492050-01 & 008557304-01 & 1:1 & 592.1 & 149 & 0 & 15.94 & -0.66 & 1.4897E+00 & Col-Anomaly & 1\\
008492072-01 & 008818524-01 & 1:1 & 3225.7 & 811 & 2 & 15.82 & -0.55 & 1.3020E+00 & Col-Anomaly & 1\\
008492101-01 & 008621026-pri & 1:1 & 951.1 & 0 & 239 & 13.37 & 0.14 & 2.3241E+03 & Col-Anomaly & 0\\
008509361-01 & 008509346-01 & 1:1 & 12.2 & -3 & -1 & 13.74 & 0.21 & 2.6241E+02 & Direct-PRF & 0\\
008509694-02 & 008509703-01 & 1:1 & 7.5 & 0 & -2 & 15.74 & -3.29 & 9.2000E+01 & Direct-PRF & 0\\
008524110-01 & 6060.01 & 1:2 & 1544.2 & 389 & -4 & 14.59 & -1.19 & 5.6130E+02 & Col-Anomaly & 0\\
008524346-01 & 3518.01 & 1:2 & 487.5 & 123 & 0 & 14.00 & -0.28 & 1.9335E+03 & Col-Anomaly & 0\\
008543279-01 & 7052.01 & 1:1 & 5.7 & 1 & 1 & 14.61 & 1.38 & 4.5262E+00 & Direct-PRF & 0\\
008543279-02 & 7052.01 & 1:2 & 5.7 & 1 & 1 & 14.61 & 1.38 & 1.2963E+01 & Direct-PRF & 0\\
008547328-01 & 008547525-01 & 1:1 & 327.0 & 82 & 3 & 15.86 & -0.36 & 1.6168E+00 & Col-Anomaly & 1\\
008547387-01 & 008374896-01 & 1:1 & 22905.5 & -101 & 121 & 15.07 & 0.91 & 5.7031E-01 & Reflection & 1\\
008547525-01 & 008547328-01 & 1:1 & 327.0 & -82 & -3 & 15.49 & 0.36 & 6.1851E-01 & Col-Anomaly & 1\\
008552498-01 & 008552540-01 & 2:1 & 59.3 & -13 & -8 & 10.29 & 3.29 & 6.0368E+03 & Direct-PRF & 0\\
008552498-03 & 008552540-01 & 2:1 & 59.3 & -13 & -8 & 10.29 & 3.29 & 5.6004E+03 & Direct-PRF & 0\\
008552500-01 & 008552540-01 & 1:2 & 125.9 & 4 & -32 & 10.29 & 4.72 & 1.3281E+04 & Direct-PRF & 0\\
008552565-01 & 008552540-01 & 1:1 & 65.4 & 15 & -8 & 10.29 & 2.66 & 8.1550E+03 & Direct-PRF & 0\\
008552583-01 & 008552540-01 & 1:1 & 102.6 & 23 & -13 & 10.29 & 4.77 & 3.0581E+03 & Direct-PRF & 0\\
008552587-01 & 008552540-01 & 1:1 & 58.7 & 6 & 13 & 10.29 & 3.83 & 6.1162E+03 & Direct-PRF & 0\\
008552607-01 & 008552540-01 & 1:1 & 103.0 & 26 & -3 & 10.29 & 3.99 & 6.3676E+03 & Direct-PRF & 0\\
008557246-01 & 008818552-01 & 1:1 & 2774.9 & 697 & 3 & 15.96 & -0.08 & 1.9535E+00 & Col-Anomaly & 1\\
008557304-01 & 008557469-01 & 1:1 & 163.9 & 41 & 1 & 14.80 & 1.13 & 5.3769E-01 & Col-Anomaly & 1\\
008557354-01 & 008688110-01 & 1:1 & 1747.7 & 439 & 2 & 15.82 & 0.06 & 2.1874E+00 & Col-Anomaly & 1\\
008557371-01 & 008557304-01 & 1:1 & 69.8 & -17 & -3 & 15.94 & -0.76 & 1.6050E+00 & Direct-PRF & 1\\
008557469-01 & 008557304-01 & 1:1 & 163.9 & -41 & -1 & 15.94 & -1.13 & 1.8598E+00 & Col-Anomaly & 1\\
008560280-01 & 1249.01 & 1:1 & 10.3 & 0 & 3 & 15.25 & -2.37 & 7.7767E+01 & Direct-PRF & 0\\
008560804-01 & 008560861-01 & 1:1 & 73.8 & 18 & -5 & 8.50 & 4.07 & 4.2448E+02 & Direct-PRF & 0\\
008560804-02 & 008560861-02 & 2:1 & 73.8 & 18 & -5 & 8.50 & 4.07 & 3.5045E+02 & Direct-PRF & 0\\
008560840-01 & 008560861-01 & 1:1 & 61.0 & 10 & -11 & 8.50 & 7.03 & 5.7067E+01 & Direct-PRF & 0\\
008560840-02 & 008560861-02 & 2:1 & 61.0 & 10 & -11 & 8.50 & 7.03 & 6.2105E+01 & Direct-PRF & 0\\
008560861-01 & 009021047-03 & 1:11 & 3024.5 & -7 & 1 & 15.25 & -6.75 & 2.5504E-02 & Col-Anomaly & 1\\
008560927-01 & 008560861-01 & 1:1 & 133.5 & 1 & -34 & 8.50 & 4.54 & 1.9883E+03 & Direct-PRF & 0\\
008560940-01 & 008560861-01 & 1:1 & 94.7 & -14 & -20 & 8.50 & 6.04 & 4.4708E+02 & Direct-PRF & 0\\
008589731-01 & 3518.01 & 1:2 & 19.9 & 4 & 4 & 14.00 & -0.76 & 1.3093E+02 & Direct-PRF & 0\\
008618649-01 & 008618808-01 & 1:1 & 332.8 & 3 & -83 & 15.21 & 0.08 & 5.4764E-01 & Col-Anomaly & 1\\
008618728-01 & 008554005-pri & 1:1 & 68.2 & 16 & -6 & 12.71 & 2.34 & 1.2455E+04 & Direct-PRF & 0\\
008618808-01 & 008618649-01 & 1:1 & 332.8 & -3 & 83 & 15.29 & -0.08 & 1.8260E+00 & Col-Anomaly & 1\\
008619448-01 & 008619436-01 & 2:1 & 15.5 & 4 & 1 & 11.81 & 0.61 & 1.2857E+00 & Direct-PRF & 0\\
008620348-01 & 008880123-02 & 1:1 & 1721.7 & -2 & 433 & 15.22 & 0.53 & 4.8880E-01 & Col-Anomaly & 1\\
008620565-01 & 008620561-01 & 1:1 & 5.2 & 0 & -1 & 16.78 & -1.87 & 3.0223E+02 & Direct-PRF & 0\\
008621348-01 & 3682.01 & 1:1 & 7.3 & 1 & -2 & 17.95 & -3.54 & 5.7990E+02 & Direct-PRF & 0\\
008621348-02 & 008621353-02 & 1:1 & 7.3 & 1 & -2 & 17.95 & -3.54 & 4.0714E+02 & Direct-PRF & 0\\
008621471-01 & 008751461-01 & 1:1 & 1393.4 & 350 & -2 & 15.13 & 0.53 & 1.1533E+00 & Col-Anomaly & 1\\
008621528-01 & 008751641-01 & 1:1 & 1526.7 & 384 & -4 & 14.09 & 1.91 & 8.0909E-02 & Col-Anomaly & 1\\
008621731-01 & 008621528-01 & 1:1 & 225.8 & -57 & 2 & 15.99 & -0.74 & 3.5064E+00 & Col-Anomaly & 1\\
008621839-01 & 008817510-01 & 1:1 & 1775.5 & 446 & 0 & 15.83 & -2.40 & 8.7374E+00 & Col-Anomaly & 1\\
008622875-01 & 008688110-01 & 1:1 & 933.3 & 235 & 4 & 15.82 & -1.81 & 4.8605E+00 & Col-Anomaly & 1\\
008625732-01 & 008560861-01 & 1:1 & 115.2 & -20 & 21 & 8.50 & 6.32 & 6.1932E+02 & Direct-PRF & 0\\
008625813-01 & 1859.01 & 1:1 & 10.8 & 3 & -1 & 15.02 & 0.96 & 1.2995E+00 & Direct-PRF & 0\\
008630973-01 & 008565912-pri & 1:1 & 253.5 & 64 & 0 & 14.71 & 0.51 & 7.7095E+03 & Col-Anomaly & 0\\
008635938-01 & 008700506-02 & 1:1 & 313.4 & 79 & 0 & 13.48 & -0.52 & 2.0408E+03 & Col-Anomaly & 0\\
008635938-02 & 008700506-01 & 1:1 & 313.4 & 79 & 0 & 13.48 & -0.52 & 1.7923E+03 & Col-Anomaly & 0\\
008647295-01 & 008647309-pri & 1:1 & 7.7 & -1 & -2 & 16.63 & -2.04 & 1.5177E+03 & Direct-PRF & 0\\
008684335-01 & 008748659-01 & 1:1 & 75.7 & -1 & 20 & 15.99 & -5.79 & 3.0559E+00 & Direct-PRF & 1\\
008686761-01 & 008884796-01 & 1:1 & 1972.0 & 495 & 1 & 14.81 & -0.89 & 3.0886E+00 & Col-Anomaly & 1\\
008687209-01 & 008884774-01 & 1:1 & 1422.7 & 357 & 3 & 14.80 & 0.86 & 4.4174E-01 & Col-Anomaly & 1\\
008687499-01 & 008752590-01 & 1:1 & 923.3 & 232 & 3 & 15.56 & 0.16 & 1.1481E+00 & Col-Anomaly & 1\\
008688110-01 & 008557354-01 & 1:1 & 1747.7 & -439 & -2 & 15.88 & -0.06 & 4.5716E-01 & Col-Anomaly & 1\\
008700537-01 & 008700506-02 & 1:1 & 21.8 & -5 & 4 & 13.48 & 0.89 & 1.8731E+03 & Direct-PRF & 0\\
008700537-02 & 008700506-01 & 1:1 & 21.8 & -5 & 4 & 13.48 & 0.89 & 2.1875E+03 & Direct-PRF & 0\\
008703884-01 & 008703887-pri & 1:1 & 12.4 & -1 & -3 & 11.05 & 4.32 & 5.2115E+00 & Direct-PRF & 0\\
008746295-01 & 7085.01 & 1:1 & 12.4 & -3 & -2 & 14.77 & -0.03 & 3.9010E+02 & Direct-PRF & 0\\
008747972-01 & 7054.01 & 1:1 & 2341.0 & 589 & 2 & 10.29 & 5.41 & 9.6574E+03 & Col-Anomaly & 0\\
008748659-01 & 008684335-01 & 1:1 & 75.7 & 1 & -20 & 10.21 & 5.79 & 3.2724E-01 & Direct-PRF & 0\\
008751461-01 & 008621471-01 & 1:1 & 1393.4 & -350 & 2 & 15.65 & -0.53 & 8.6704E-01 & Col-Anomaly & 1\\
008751580-01 & 008817499-01 & 1:1 & 671.9 & 169 & -4 & 15.43 & 0.54 & 6.7247E-01 & Col-Anomaly & 1\\
008751641-01 & 008621528-01 & 1:1 & 1526.7 & -384 & 4 & 15.99 & -1.91 & 1.2360E+01 & Col-Anomaly & 1\\
008752295-01 & 008885293-01 & 1:1 & 1052.3 & 264 & -4 & 15.85 & -0.24 & 3.8800E-01 & Col-Anomaly & 1\\
008752538-01 & 008688110-01 & 1:1 & 179.1 & -45 & 0 & 15.82 & -0.69 & 2.7127E+00 & Col-Anomaly & 1\\
008752590-01 & 008687499-01 & 1:1 & 923.3 & -232 & -3 & 15.72 & -0.16 & 8.7097E-01 & Col-Anomaly & 1\\
008752817-01 & 008752914-01 & 2:1 & 81.8 & 15 & -14 & 13.89 & -0.21 & 4.1667E-01 & Direct-PRF & 1\\
008752914-01 & 008752817-01 & 1:2 & 81.8 & -15 & 14 & 13.67 & 0.21 & 2.4000E+00 & Direct-PRF & 1\\
008766222-01 & 5571.01 & 1:1 & 102.7 & 26 & 4 & 10.25 & 3.60 & 1.3594E-01 & Direct-PRF & 1\\
008766268-01 & 008766222-01 & 1:1 & 81.9 & -21 & -3 & 13.85 & 1.80 & 9.5871E+00 & Direct-PRF & 1\\
008766285-01 & 008766222-01 & 1:1 & 102.7 & -26 & -4 & 13.85 & -3.60 & 1.2487E+01 & Direct-PRF & 1\\
008780959-01 & 3653.01 & 1:1 & 8.1 & 2 & 1 & 16.30 & -3.00 & 9.8859E+01 & Direct-PRF & 0\\
008806072-02 & 008176161-01 & 1:1 & 24113.3 & -146 & 130 & 14.88 & -0.02 & 1.0822E+00 & Reflection & 1\\
008817499-01 & 008751580-01 & 1:1 & 671.9 & -169 & 4 & 15.97 & -0.54 & 1.4871E+00 & Col-Anomaly & 1\\
008817510-01 & 008621839-01 & 1:1 & 1775.5 & -446 & 0 & 13.43 & 2.40 & 1.1445E-01 & Col-Anomaly & 1\\
008818096-02 & 008818193-01 & 2:1 & 90.2 & 22 & -3 & 15.86 & 0.12 & 8.8506E-01 & Col-Anomaly & 1\\
008818193-01 & 008818096-02 & 1:2 & 90.2 & -22 & 3 & 15.98 & -0.12 & 1.1299E+00 & Col-Anomaly & 1\\
008818311-01 & 008752295-01 & 1:1 & 761.7 & -191 & -2 & 15.61 & -0.58 & 1.3578E+00 & Col-Anomaly & 1\\
008818524-01 & 008492072-01 & 1:1 & 3225.7 & -811 & -2 & 15.28 & 0.55 & 7.6806E-01 & Col-Anomaly & 1\\
008818552-01 & 008557246-01 & 1:1 & 2774.9 & -697 & -3 & 15.88 & 0.08 & 5.1191E-01 & Col-Anomaly & 1\\
008823426-01 & 7096.01 & 1:1 & 20.5 & 3 & -4 & 13.25 & 2.34 & 1.1848E+03 & Direct-PRF & 0\\
008823833-01 & 7096.01 & 1:1 & 487.8 & 123 & 0 & 13.25 & -0.35 & 1.2364E+04 & Col-Anomaly & 0\\
008823893-01 & 7096.01 & 1:1 & 552.0 & 139 & 2 & 13.25 & 0.66 & 1.3777E+04 & Col-Anomaly & 0\\
008848115-01 & 7100.01 & 1:1 & 14.4 & -1 & -3 & 12.37 & 0.35 & 1.5297E+02 & Direct-PRF & 0\\
008868649-01 & 008868650-pri & 1:1 & 25.8 & 3 & -6 & 11.94 & 2.08 & 2.8341E+03 & Direct-PRF & 0\\
008868657-01 & 008868650-pri & 1:1 & 74.2 & 13 & -14 & 11.94 & 4.05 & 1.8338E+03 & Direct-PRF & 0\\
008868686-01 & 7102.01 & 1:1 & 54.5 & 2 & 14 & 15.99 & -2.48 & 7.0385E+00 & Direct-PRF & 1\\
008878567-01 & 009083523-pri & 1:1 & 1709.6 & -430 & 5 & 12.71 & -0.59 & 4.9744E+04 & Col-Anomaly & 0\\
008879124-01 & 008879302-01 & 1:1 & 291.9 & -2 & -74 & 15.83 & -0.71 & 1.5972E+00 & Col-Anomaly & 1\\
008879302-01 & 008879124-01 & 1:1 & 291.9 & 2 & 74 & 15.13 & 0.71 & 6.2609E-01 & Col-Anomaly & 1\\
008880003-01 & 008620348-01 & 1:1 & 1945.0 & 0 & -489 & 15.75 & -0.57 & 1.3434E+00 & Col-Anomaly & 1\\
008880003-02 & 008879915-pri & 1:2 & 147.2 & 0 & 37 & 15.19 & -0.01 & 9.8979E+03 & Col-Anomaly & 0\\
008880123-02 & 008620348-01 & 1:1 & 1721.7 & 2 & -433 & 15.75 & -0.53 & 2.0458E+00 & Col-Anomaly & 1\\
008884690-01 & 008952695-01 & 1:1 & 712.4 & 179 & 4 & 14.51 & -0.10 & 1.0490E+00 & Col-Anomaly & 1\\
008884774-01 & 008687209-01 & 1:1 & 1422.7 & -357 & -3 & 15.65 & -0.86 & 2.2638E+00 & Col-Anomaly & 1\\
008884796-01 & 008686761-01 & 1:1 & 1972.0 & -495 & -1 & 13.92 & 0.89 & 3.2378E-01 & Col-Anomaly & 1\\
008885293-01 & 008752295-01 & 1:1 & 1052.3 & -264 & 4 & 15.61 & 0.24 & 2.5773E+00 & Col-Anomaly & 1\\
008890996-01 & 7096.01 & 1:1 & 627.1 & 158 & 0 & 13.25 & -0.76 & 2.8365E+04 & Col-Anomaly & 0\\
008892721-01 & 3336.01 & 1:1 & 7.4 & -1 & -2 & 15.52 & 0.42 & 1.7186E+01 & Direct-PRF & 0\\
008906045-01 & 008906039-pri & 1:1 & 3.9 & 1 & -1 & 12.62 & 1.55 & 1.5988E+02 & Direct-PRF & 0\\
008937021-01 & 3754.01 & 1:1 & 4.2 & 0 & 1 & 17.93 & -2.49 & 3.0774E+02 & Direct-PRF & 0\\
008937021-02 & 008937019-02 & 1:1 & 4.2 & 0 & 1 & 17.93 & -2.49 & 1.0343E+02 & Direct-PRF & 0\\
008952695-01 & 008884690-01 & 1:1 & 712.4 & -179 & -4 & 14.41 & 0.10 & 9.5331E-01 & Col-Anomaly & 1\\
008953414-01 & 7113.01 & 1:1 & 82.8 & 13 & 16 & 12.16 & 3.23 & 1.0675E+03 & Direct-PRF & 0\\
008953475-01 & 7113.01 & 1:1 & 118.5 & 0 & 30 & 12.16 & 1.41 & 4.8665E+03 & Direct-PRF & 0\\
008963721-01 & 5614.01 & 1:1 & 1527.8 & 384 & 0 & 13.95 & 0.73 & 6.2434E+03 & Col-Anomaly & 0\\
009007953-01 & 009007918-pri & 1:1 & 55.1 & 0 & -14 & 11.66 & 3.06 & 3.1612E+03 & Direct-PRF & 0\\
009021047-03 & 008560861-01 & 11:1 & 3024.5 & 7 & -1 & 8.50 & 6.75 & 3.9210E+01 & Col-Anomaly & 1\\
009025922-01 & 3596.01 & 1:1 & 8.4 & 2 & 1 & 16.76 & -3.47 & 1.3368E+02 & Direct-PRF & 0\\
009025922-02 & 009025914-02 & 1:1 & 8.4 & 2 & 1 & 16.76 & -3.47 & 4.3604E+01 & Direct-PRF & 0\\
009048161-01 & 6063.01 & 1:1 & 9.0 & 0 & 2 & 13.09 & -0.06 & 1.9352E+01 & Direct-PRF & 0\\
009048161-02 & 009048145-sec & 1:1 & 9.0 & 0 & 2 & 13.09 & -0.06 & 2.3333E+01 & Direct-PRF & 0\\
009049697-01 & 3799.01 & 1:1 & 19.4 & -4 & 1 & 15.82 & -0.66 & 6.1922E+01 & Direct-PRF & 0\\
009053112-01 & 009053086-01 & 1:1 & 14.3 & -3 & 2 & 14.03 & -0.28 & 7.0711E+02 & Direct-PRF & 0\\
009083470-01 & 7128.01 & 1:1 & 29.6 & -5 & -6 & 15.91 & -0.01 & 1.5752E+00 & Direct-PRF & 1\\
009083503-01 & 009083523-pri & 1:1 & 74.9 & -13 & 13 & 12.71 & 3.20 & 4.1454E+03 & Direct-PRF & 0\\
009083564-01 & 4731.01 & 1:1 & 113.5 & 28 & 2 & 15.90 & -3.46 & 1.4923E+01 & Direct-PRF & 1\\
009091897-01 & 009091810-pri & 2:1 & 84.9 & 16 & -14 & 12.76 & 2.07 & 8.9204E+03 & Direct-PRF & 0\\
009093859-01 & 009159301-pri & 1:1 & 93.3 & -23 & -6 & 12.15 & 3.82 & 6.4316E+03 & Direct-PRF & 0\\
009101208-01 & 5614.01 & 1:1 & 69.8 & 17 & 2 & 13.95 & 1.43 & 1.5508E+04 & Direct-PRF & 0\\
009107457-01 & 009171234-02 & 1:1 & 48.2 & 5 & 11 & 14.11 & 1.66 & 4.2602E-01 & Direct-PRF & 1\\
009108085-01 & 5615.01 & 1:1 & 28.0 & 0 & 7 & 14.28 & -0.63 & 1.1224E+04 & Direct-PRF & 0\\
009110357-01 & 3607.01 & 1:1 & 9.9 & 2 & -2 & 16.40 & -2.82 & 2.0650E+03 & Direct-PRF & 0\\
009159198-01 & 009159301-pri & 1:1 & 97.0 & -23 & 8 & 12.15 & 2.74 & 1.1638E+04 & Direct-PRF & 0\\
009159242-01 & 009159301-pri & 1:1 & 48.2 & -10 & 7 & 12.15 & 1.88 & 6.9829E+03 & Direct-PRF & 0\\
009159265-01 & 009159301-pri & 1:1 & 34.5 & -9 & -1 & 12.15 & 2.36 & 2.3844E+03 & Direct-PRF & 0\\
009159275-01 & 009159301-pri & 1:1 & 21.2 & -5 & 3 & 12.15 & 3.47 & 1.1835E+03 & Direct-PRF & 0\\
009166870-01 & 931.01 & 1:1 & 7.5 & -2 & 1 & 15.27 & -0.22 & 1.7506E+01 & Direct-PRF & 0\\
009171234-02 & 009107457-01 & 1:1 & 48.2 & -5 & -11 & 15.76 & -1.66 & 2.3473E+00 & Direct-PRF & 1\\
009210823-01 & 009210828-pri & 1:2 & 15.2 & -2 & -3 & 13.22 & -1.48 & 2.2210E+03 & Direct-PRF & 0\\
009214715-01 & 6064.01 & 1:1 & 4.1 & -1 & 0 & 15.52 & -0.24 & 3.2532E+00 & Direct-PRF & 0\\
009214715-02 & 6064.02 & 1:1 & 4.1 & -1 & 0 & 15.52 & -0.24 & 3.6285E+00 & Direct-PRF & 0\\
009220612-01 & 009220600-pri & 1:1 & 21.2 & 4 & 4 & 12.26 & 3.01 & 5.5000E+02 & Direct-PRF & 0\\
009282762-01 & BR-Cyg-pri & 1:1 & 7602.3 & -2 & 7 & 10.03 & 5.68 & 6.9674E+03 & Cross-Talk & 0\\
009282769-01 & BR-Cyg-pri & 1:1 & 7582.2 & 3 & 2 & 10.03 & 3.38 & 1.6117E+03 & Cross-Talk & 0\\
009283821-01 & 009283826-pri & 2:1 & 30.2 & 3 & -7 & 13.09 & 1.24 & 1.3900E+04 & Direct-PRF & 0\\
009286728-01 & 009159301-pri & 1:1 & 1349.3 & 339 & -1 & 12.15 & 2.42 & 1.1922E+04 & Col-Anomaly & 0\\
009291039-03 & 7155.01 & 1:1 & 304.5 & 77 & 1 & 14.01 & -1.77 & 2.5957E+04 & Col-Anomaly & 0\\
009291378-01 & 7155.01 & 1:1 & 12.6 & -3 & 0 & 14.01 & 1.53 & 2.3077E+02 & Direct-PRF & 0\\
009328864-01 & 7159.01 & 1:1 & 16.6 & -4 & 1 & 15.33 & -1.22 & 6.5538E+03 & Direct-PRF & 0\\
009340955-01 & V2281-Cyg-pri & 1:2 & 240.8 & 38 & 48 & 11.82 & 3.12 & 9.4626E+03 & Direct-PRF & 0\\
009340980-01 & 009402583-01 & 1:1 & 106.2 & -4 & 26 & 15.89 & -0.61 & 2.1935E+00 & Col-Anomaly & 1\\
009345819-01 & 009345838-pri & 1:1 & 66.8 & -12 & 11 & 12.38 & 3.43 & 3.3282E+03 & Direct-PRF & 0\\
009345924-01 & 009345838-pri & 1:1 & 88.0 & 22 & 4 & 12.38 & 2.46 & 1.0274E+04 & Direct-PRF & 0\\
009357375-01 & 009357275-pri & 1:1 & 81.5 & 15 & -15 & 12.19 & 3.27 & 2.2918E+03 & Direct-PRF & 0\\
009366989-01 & 3597.01 & 1:1 & 7.9 & 1 & 2 & 14.37 & 0.54 & 1.5509E+02 & Direct-PRF & 0\\
009389134-01 & 009389122-pri & 2:1 & 16.8 & 4 & 1 & 14.31 & 0.61 & 7.7526E+03 & Direct-PRF & 0\\
009390655-01 & 249.01 & 1:1 & 4.3 & -1 & 0 & 14.49 & 0.98 & 2.7040E+00 & Direct-PRF & 0\\
009394605-01 & 009394601-pri & 1:1 & 18.1 & -4 & -1 & 12.29 & 3.11 & 5.9377E+02 & Direct-PRF & 0\\
009402670-01 & 009402709-01 & 1:1 & 52.9 & 5 & -12 & 13.44 & 2.22 & 3.6232E-01 & Direct-PRF & 1\\
009402709-01 & 009402670-01 & 1:1 & 52.9 & -5 & 12 & 15.67 & -2.22 & 2.7600E+00 & Direct-PRF & 1\\
009412445-01 & 7171.01 & 1:2 & 15.4 & 4 & 0 & 14.85 & -0.20 & 1.7724E+03 & Direct-PRF & 0\\
009468382-01 & 3466.01 & 1:1 & 9.4 & -1 & 2 & 16.41 & -2.85 & 5.4920E+02 & Direct-PRF & 0\\
009468382-02 & 009468384-sec & 1:1 & 9.4 & -1 & 2 & 16.41 & -2.85 & 3.9467E+02 & Direct-PRF & 0\\
009474232-01 & 009474222-pri & 1:1 & 18.2 & -3 & 3 & 13.28 & 1.29 & 7.3706E+02 & Direct-PRF & 0\\
009474483-01 & 5683.01 & 1:1 & 20.9 & 3 & -4 & 14.88 & 0.60 & 5.1266E+03 & Direct-PRF & 0\\
009474493-01 & 5683.01 & 1:1 & 17.3 & 1 & -4 & 14.88 & 0.45 & 3.0451E+03 & Direct-PRF & 0\\
009488426-01 & 007848303-02 & 4:1 & 9269.6 & 340 & 9 & 11.28 & 1.70 & 1.5000E+00 & Col-Anomaly & 1\\
009489348-01 & 009489411-pri & 1:2 & 43.7 & 11 & 1 & 13.96 & -0.36 & 8.3667E+03 & Direct-PRF & 0\\
009509223-01 & 009509207-sec & 1:1 & 34.4 & -8 & 0 & 13.13 & 0.46 & 3.6157E+03 & Direct-PRF & 0\\
009509223-02 & 7181.01 & 1:1 & 34.4 & -8 & 0 & 13.13 & 0.46 & 2.7923E+03 & Direct-PRF & 0\\
009518558-01 & FL-Lyr-pri & 1:1 & 558.6 & -140 & 0 & 9.18 & 5.47 & 3.2467E+03 & Direct-PRF & 0\\
009518651-01 & FL-Lyr-pri & 1:1 & 771.8 & -194 & 2 & 9.18 & 4.93 & 1.0359E+04 & Direct-PRF & 0\\
009529744-01 & 009529733-pri & 1:2 & 14.0 & 4 & 0 & 14.04 & -0.56 & 9.7292E+02 & Direct-PRF & 0\\
009532117-01 & 6069.01 & 1:1 & 12.1 & -1 & -3 & 16.36 & -4.01 & 1.1974E+03 & Direct-PRF & 0\\
009532117-02 & 009532123-02 & 1:1 & 12.1 & -1 & -3 & 16.36 & -4.01 & 9.9916E+02 & Direct-PRF & 0\\
009532424-01 & 3710.01 & 1:1 & 9.4 & 1 & 3 & 16.77 & -2.21 & 1.9561E+02 & Direct-PRF & 0\\
009535876-01 & 4228.01 & 1:1 & 21.5 & 4 & -4 & 13.40 & 1.52 & 4.5031E+01 & Direct-PRF & 0\\
009535876-02 & 009535881-02 & 1:1 & 21.5 & 4 & -4 & 13.40 & 1.52 & 2.2090E+00 & Direct-PRF & 0\\
009540675-01 & V995-Cyg-pri & 1:1 & 119.4 & -1 & -30 & 11.88 & 1.99 & 2.0287E+04 & Direct-PRF & 0\\
009541094-01 & 009541127-pri & 1:1 & 56.6 & 1 & 14 & 12.56 & 1.25 & 1.2403E+04 & Direct-PRF & 0\\
009541163-01 & 009541127-pri & 1:1 & 61.9 & -2 & -16 & 12.56 & 2.89 & 4.7705E+03 & Direct-PRF & 0\\
009549471-01 & 6206.01 & 1:1 & 9.3 & 1 & 2 & 14.05 & 0.24 & 1.7280E+01 & Direct-PRF & 0\\
009549471-02 & 009549472-02 & 1:1 & 9.3 & 1 & 2 & 14.05 & 0.24 & 1.6579E+01 & Direct-PRF & 0\\
009579753-01 & FL-Lyr-pri & 1:2 & 187.4 & 4 & -47 & 9.18 & 6.42 & 4.4852E+03 & Direct-PRF & 0\\
009579789-01 & FL-Lyr-pri & 1:2 & 166.9 & -9 & -41 & 9.18 & 6.28 & 6.2152E+03 & Direct-PRF & 0\\
009592579-01 & 009592575-01 & 1:1 & 6.7 & 0 & 1 & 15.90 & -0.80 & 3.8242E+01 & Direct-PRF & 0\\
009592818-01 & 3883.01 & 1:2 & 59.4 & 0 & -15 & 16.40 & -1.85 & 2.7482E+04 & Direct-PRF & 0\\
009592831-01 & 009592850-01 & 1:1 & 28.8 & -7 & 2 & 16.40 & 0.28 & 1.6476E+03 & Direct-PRF & 0\\
009592855-01 & 3883.01 & 1:2 & 6.9 & 0 & 1 & 16.40 & -4.18 & 3.5300E+00 & Direct-PRF & 0\\
009592918-01 & 009592831-01 & 1:1 & 114.0 & 28 & -2 & 16.68 & -1.67 & 5.3684E+00 & Col-Anomaly & 1\\
009593757-01 & 009593759-01 & 1:1 & 6.2 & 0 & -2 & 17.47 & 0.22 & 4.7146E+01 & Direct-PRF & 0\\
009593757-02 & 009593759-02 & 1:1 & 6.2 & 0 & -2 & 17.47 & 0.22 & 1.5637E+01 & Direct-PRF & 0\\
009602421-01 & V995-Cyg-pri & 1:1 & 134.2 & -34 & 1 & 11.88 & 0.96 & 4.2828E+04 & Direct-PRF & 0\\
009602431-01 & V995-Cyg-pri & 1:1 & 123.0 & -18 & 25 & 11.88 & 3.31 & 1.1506E+04 & Direct-PRF & 0\\
009602514-01 & V995-Cyg-pri & 1:1 & 58.7 & -15 & 1 & 11.88 & 2.24 & 3.3229E+03 & Direct-PRF & 0\\
009602538-01 & V995-Cyg-pri & 1:1 & 197.3 & 14 & 48 & 11.88 & 2.73 & 1.6759E+04 & Direct-PRF & 0\\
009602562-01 & V995-Cyg-pri & 1:1 & 104.7 & 5 & 26 & 11.88 & 2.50 & 3.6193E+03 & Direct-PRF & 0\\
009602658-01 & V995-Cyg-pri & 1:1 & 178.9 & 31 & 33 & 11.88 & 3.92 & 7.0083E+03 & Direct-PRF & 0\\
009602775-01 & V995-Cyg-pri & 1:1 & 134.2 & 29 & -16 & 11.88 & 4.04 & 6.8832E+03 & Direct-PRF & 0\\
009635510-01 & 009635529-pri & 1:2 & 33.1 & 8 & 1 & 12.23 & 3.12 & 9.0600E+02 & Direct-PRF & 0\\
009636563-01 & 3618.01 & 1:1 & 10.2 & -2 & -1 & 17.04 & -1.94 & 9.5792E+02 & Direct-PRF & 0\\
009636569-01 & 3618.01 & 1:1 & 10.1 & -2 & 2 & 17.04 & -2.60 & 1.4789E+03 & Direct-PRF & 0\\
009640907-01 & FL-Lyr-pri & 1:1 & 170.1 & 30 & -30 & 9.18 & 6.52 & 1.9866E+03 & Direct-PRF & 0\\
009640921-03 & FL-Lyr-pri & 1:1 & 153.6 & 8 & -38 & 9.18 & 6.22 & 3.9195E+03 & Direct-PRF & 0\\
009640924-01 & FL-Lyr-pri & 1:2 & 143.3 & 30 & -20 & 9.18 & 5.80 & 6.1276E+03 & Direct-PRF & 0\\
009640931-01 & FL-Lyr-pri & 1:1 & 151.6 & 2 & -38 & 9.18 & 6.74 & 1.9597E+03 & Direct-PRF & 0\\
009640946-01 & 009641031-01 & 1:2 & 153.8 & 38 & -8 & 9.18 & 5.78 & 6.0066E+03 & Direct-PRF & 0\\
009640962-01 & FL-Lyr-pri & 1:2 & 122.6 & 31 & -5 & 9.18 & 6.29 & 3.2467E+03 & Direct-PRF & 0\\
009640976-01 & FL-Lyr-pri & 1:1 & 138.2 & 35 & 2 & 9.18 & 4.54 & 3.1526E+03 & Direct-PRF & 0\\
009640976-02 & 7211.01 & 2:1 & 138.2 & 35 & 2 & 9.18 & 4.54 & 8.1876E+03 & Direct-PRF & 0\\
009640985-01 & FL-Lyr-pri & 1:1 & 63.1 & 13 & -9 & 9.18 & 4.66 & 1.9336E+03 & Direct-PRF & 0\\
009641008-01 & FL-Lyr-pri & 1:1 & 70.0 & -10 & -14 & 9.18 & 5.31 & 1.3065E+03 & Direct-PRF & 0\\
009641018-01 & FL-Lyr-pri & 1:1 & 90.3 & 21 & 10 & 9.18 & 4.89 & 2.1862E+03 & Direct-PRF & 0\\
009641041-01 & FL-Lyr-pri & 1:1 & 66.6 & -15 & -7 & 9.18 & 3.04 & 4.5796E+03 & Direct-PRF & 0\\
009641076-01 & FL-Lyr-pri & 1:1 & 143.3 & 15 & 33 & 9.18 & 5.95 & 3.8845E+03 & Direct-PRF & 0\\
009641103-01 & 7211.01 & 1:1 & 230.9 & 25 & 53 & 9.18 & 4.95 & 1.1220E+04 & Direct-PRF & 0\\
009641144-01 & 7211.01 & 1:1 & 173.5 & -26 & 35 & 9.18 & 4.76 & 7.9721E+03 & Direct-PRF & 0\\
009644683-01 & 009644680-pri & 1:1 & 16.0 & 2 & -4 & 13.44 & 2.48 & 2.8010E+05 & Direct-PRF & 0\\
009652649-01 & 7217.01 & 1:1 & 31.7 & 4 & 7 & 11.58 & 2.53 & 2.7402E+03 & Direct-PRF & 0\\
009652655-01 & 7217.01 & 1:1 & 38.5 & 8 & 6 & 11.58 & 3.19 & 1.8790E+03 & Direct-PRF & 0\\
009656547-01 & 3588.01 & 1:2 & 15.4 & -4 & -2 & 16.32 & -0.86 & 5.9380E+03 & Direct-PRF & 0\\
009661877-01 & 3647.01 & 1:1 & 7.8 & 2 & 0 & 16.68 & -1.51 & 1.1173E+02 & Direct-PRF & 0\\
009664387-02 & 009664382-pri & 2:1 & 6.7 & 0 & -2 & 16.58 & -2.19 & 6.8954E+01 & Direct-PRF & 0\\
009674564-01 & 009674592-01 & 1:1 & 16.5 & 4 & 0 & 15.93 & -1.89 & 4.8885E+01 & Direct-PRF & 0\\
009674564-02 & 3729.01 & 1:1 & 16.5 & 4 & 0 & 15.93 & -1.89 & 5.7760E+01 & Direct-PRF & 0\\
009692128-01 & 7191.01 & 1:1 & 845.0 & 212 & 0 & 13.98 & -0.32 & 4.2453E+03 & Col-Anomaly & 0\\
009692345-01 & 3859.01 & 1:1 & 13.3 & -2 & 3 & 17.49 & -1.83 & 1.9962E+03 & Direct-PRF & 0\\
009716262-01 & 009838414-01 & 1:1 & 1486.9 & 374 & 2 & 17.51 & 0.07 & 1.4228E+00 & Col-Anomaly & 1\\
009716302-01 & BR-Cyg-pri & 1:1 & 2638.5 & 663 & 5 & 10.03 & 6.46 & 2.1930E+03 & Col-Anomaly & 0\\
009719634-01 & 3686.01 & 1:1 & 8.6 & 0 & 2 & 17.28 & -2.46 & 1.9301E+02 & Direct-PRF & 0\\
009724984-01 & 5708.01 & 1:1 & 9.7 & -1 & 2 & 12.52 & 0.42 & 3.9900E+01 & Direct-PRF & 0\\
009752973-01 & 3871.01 & 1:1 & 13.0 & 3 & 0 & 12.22 & -2.18 & 1.5333E+01 & Direct-PRF & 0\\
009762514-01 & 7228.01 & 1:1 & 18.1 & 1 & -4 & 13.71 & 1.81 & 5.9206E+02 & Direct-PRF & 0\\
009777087-01 & 3672.01 & 1:1 & 4.1 & 1 & 0 & 17.78 & -0.71 & 1.0099E+01 & Direct-PRF & 0\\
009777089-01 & 009777062-01 & 1:1 & 27.7 & -7 & 0 & 12.24 & 2.19 & 2.4692E+03 & Direct-PRF & 0\\
009777200-01 & BR-Cyg-pri & 1:1 & 2041.8 & 513 & 1 & 10.03 & 3.89 & 2.2296E+04 & Col-Anomaly & 0\\
009777251-01 & BR-Cyg-pri & 1:1 & 1984.9 & 499 & 3 & 10.03 & 5.03 & 5.9192E+03 & Col-Anomaly & 0\\
009777256-01 & BR-Cyg-pri & 1:1 & 1975.9 & 496 & 1 & 10.03 & 5.23 & 5.9192E+03 & Col-Anomaly & 0\\
009777290-01 & BR-Cyg-pri & 1:1 & 1957.7 & 492 & 5 & 10.03 & 6.31 & 3.5019E+03 & Col-Anomaly & 0\\
009777556-01 & BR-Cyg-pri & 1:1 & 1676.0 & 421 & 3 & 10.03 & 6.04 & 1.3458E+03 & Col-Anomaly & 0\\
009777724-01 & BR-Cyg-pri & 1:1 & 1509.7 & 379 & 3 & 10.03 & 5.84 & 5.9192E+03 & Col-Anomaly & 0\\
009777757-01 & BR-Cyg-pri & 1:1 & 1477.6 & 371 & 4 & 10.03 & 2.97 & 2.0902E+04 & Col-Anomaly & 0\\
009784222-01 & 3851.01 & 1:1 & 9.1 & -2 & -1 & 17.58 & -2.97 & 4.1314E+03 & Direct-PRF & 0\\
009784222-02 & 009784230-01 & 1:1 & 9.1 & -2 & -1 & 17.58 & -2.97 & 5.0906E+03 & Direct-PRF & 0\\
009821151-01 & 7234.01 & 1:1 & 173.3 & 44 & -1 & 14.12 & -1.73 & 5.7963E+03 & Direct-PRF & 0\\
009821151-02 & 009821078-02 & 1:1 & 173.3 & 44 & -1 & 14.12 & -1.73 & 4.1215E+03 & Direct-PRF & 0\\
009827596-01 & 6211.01 & 1:1 & 529.6 & 133 & -1 & 14.71 & -0.15 & 7.4896E+03 & Col-Anomaly & 0\\
009833599-01 & 009833618-pri & 1:1 & 29.0 & -3 & -7 & 13.68 & 1.74 & 6.5067E+03 & Direct-PRF & 0\\
009833625-02 & 009833618-sec & 1:1 & 7.7 & 2 & 0 & 13.68 & 1.51 & 4.4456E+00 & Direct-PRF & 0\\
009834257-01 & 009773869-01 & 1:1 & 7.0 & 0 & -1 & 16.67 & -4.24 & 3.2707E+02 & Direct-PRF & 0\\
009834257-02 & 3568.01 & 1:1 & 7.0 & 0 & -1 & 16.67 & -4.24 & 8.2412E+02 & Direct-PRF & 0\\
009837578-03 & 3442.01 & 1:3 & 5.4 & 1 & 1 & 17.47 & -1.75 & 1.1743E+03 & Direct-PRF & 0\\
009837586-01 & 2937.01 & 1:2 & 5.4 & -1 & -1 & 15.73 & 1.75 & 7.4601E+00 & Direct-PRF & 0\\
009838414-01 & 009959765-01 & 1:1 & 1402.7 & 352 & -1 & 13.79 & 3.72 & 2.5143E-02 & Col-Anomaly & 1\\
009838537-01 & BR-Cyg-pri & 1:1 & 1056.9 & 265 & 3 & 10.03 & 3.43 & 2.6755E+04 & Col-Anomaly & 0\\
009838608-01 & BR-Cyg-pri & 1:1 & 982.9 & 247 & 2 & 10.03 & 5.14 & 7.5154E+03 & Col-Anomaly & 0\\
009838761-01 & BR-Cyg-pri & 1:1 & 802.4 & 201 & 2 & 10.03 & 5.81 & 7.8362E+03 & Col-Anomaly & 0\\
009838804-01 & BR-Cyg-pri & 1:1 & 763.2 & 191 & 3 & 10.03 & 5.96 & 4.1035E+03 & Col-Anomaly & 0\\
009840429-01 & 009840412-pri & 1:1 & 19.8 & -4 & -3 & 12.84 & 3.04 & 5.5618E+03 & Direct-PRF & 0\\
009842906-01 & 009842890-pri & 1:1 & 10.3 & 3 & -1 & 15.75 & -0.31 & 1.7131E+00 & Direct-PRF & 0\\
009842937-01 & 009842890-pri & 1:1 & 40.0 & 9 & 3 & 15.75 & -0.42 & 4.0201E+00 & Direct-PRF & 1\\
009849884-01 & 7268.01 & 1:1 & 1507.6 & 379 & 0 & 13.17 & -0.57 & 2.7370E+03 & Col-Anomaly & 0\\
009850843-01 & 009851142-pri & 1:1 & 218.0 & 53 & 12 & 7.63 & 7.23 & 7.6555E+02 & Direct-PRF & 0\\
009850893-01 & 009851142-pri & 1:1 & 192.2 & 29 & 39 & 7.63 & 7.04 & 3.3616E+02 & Direct-PRF & 0\\
009850912-01 & 009851142-pri & 1:1 & 202.8 & 22 & 46 & 7.63 & 8.16 & 2.9105E+02 & Direct-PRF & 0\\
009850957-01 & 009851142-pri & 1:1 & 138.4 & 22 & 27 & 7.63 & 5.49 & 8.5943E+02 & Direct-PRF & 0\\
009850966-01 & 009851142-pri & 1:1 & 160.5 & 39 & -10 & 7.63 & 8.23 & 2.9967E+02 & Direct-PRF & 0\\
009851021-01 & 009851142-pri & 1:1 & 113.1 & 10 & 27 & 7.63 & 2.63 & 1.6268E+03 & Direct-PRF & 0\\
009851123-01 & 009851142-pri & 1:1 & 56.7 & -3 & 14 & 7.63 & 8.11 & 3.7583E+01 & Direct-PRF & 0\\
009851123-02 & 009851142-sec & 1:1 & 56.7 & -3 & 14 & 7.63 & 8.11 & 1.4420E+01 & Direct-PRF & 0\\
009851126-01 & 009851142-pri & 1:1 & 21.4 & 1 & 5 & 7.63 & 5.55 & 1.1357E+00 & Direct-PRF & 0\\
009851126-02 & 009851142-sec & 1:1 & 21.4 & 1 & 5 & 7.63 & 5.55 & 1.5257E+00 & Direct-PRF & 0\\
009851142-01 & 3592.01 & 1:1 & 21.4 & -1 & -5 & 13.18 & -5.55 & 1.0052E+00 & Direct-PRF & 1\\
009851226-01 & 009851142-pri & 1:1 & 77.9 & -6 & -19 & 7.63 & 7.63 & 6.8703E+01 & Direct-PRF & 0\\
009851226-02 & 009851142-sec & 1:1 & 77.9 & -6 & -19 & 7.63 & 7.63 & 7.1512E+01 & Direct-PRF & 0\\
009851271-01 & 009851142-pri & 1:1 & 91.0 & -14 & -18 & 7.63 & 6.98 & 2.6560E+02 & Direct-PRF & 0\\
009851360-01 & 009851142-pri & 1:1 & 184.5 & -45 & 9 & 7.63 & 7.68 & 5.4551E+02 & Direct-PRF & 0\\
009851845-01 & 009851944-pri & 1:2 & 113.9 & 7 & 27 & 11.25 & 2.63 & 7.6852E+03 & Direct-PRF & 0\\
009851943-01 & 009851944-pri & 1:2 & 33.2 & -4 & 7 & 11.25 & 4.00 & 1.2809E+03 & Direct-PRF & 0\\
009851970-01 & 009851944-pri & 1:2 & 89.4 & -14 & 17 & 11.25 & 4.22 & 1.9393E+03 & Direct-PRF & 0\\
009873759-01 & 7241.01 & 1:1 & 324.1 & 82 & 1 & 13.04 & 0.78 & 2.9317E+03 & Col-Anomaly & 0\\
009886221-01 & 3614.01 & 1:1 & 13.4 & -1 & 3 & 16.33 & -1.93 & 1.2226E+03 & Direct-PRF & 0\\
009893365-01 & 009893419-01 & 1:1 & 71.2 & -3 & -17 & 15.04 & -0.71 & 1.2105E+00 & Direct-PRF & 1\\
009893419-01 & 009893365-01 & 1:1 & 71.2 & 3 & 17 & 14.34 & 0.71 & 8.2609E-01 & Direct-PRF & 1\\
009893463-01 & 009893419-01 & 1:1 & 54.2 & 14 & 2 & 15.04 & 0.52 & 4.8936E-01 & Direct-PRF & 1\\
009896438-01 & 3755.01 & 1:1 & 6.2 & -1 & 1 & 16.64 & 0.03 & 2.9446E+00 & Direct-PRF & 0\\
009899065-01 & BR-Cyg-pri & 1:1 & 361.9 & 91 & 2 & 10.03 & 5.83 & 4.9182E+03 & Direct-PRF & 0\\
009899141-01 & BR-Cyg-pri & 1:1 & 236.5 & 57 & -17 & 10.03 & 2.47 & 3.5204E+04 & Direct-PRF & 0\\
009899153-01 & BR-Cyg-pri & 1:1 & 215.8 & 42 & -34 & 10.03 & 4.85 & 1.1609E+04 & Direct-PRF & 0\\
009899181-01 & BR-Cyg-pri & 1:1 & 196.6 & 47 & -14 & 10.03 & 2.88 & 2.9081E+04 & Direct-PRF & 0\\
009899193-01 & BR-Cyg-pri & 1:1 & 250.7 & 61 & 15 & 10.03 & 3.16 & 2.4773E+04 & Direct-PRF & 0\\
009899216-01 & BR-Cyg-pri & 1:1 & 205.0 & 51 & 6 & 10.03 & 0.86 & 7.4319E+04 & Direct-PRF & 0\\
009899217-01 & BR-Cyg-pri & 1:1 & 181.5 & 45 & -3 & 10.03 & 5.24 & 5.5739E+03 & Direct-PRF & 0\\
009899233-01 & BR-Cyg-pri & 1:1 & 186.6 & 46 & 5 & 10.03 & 5.14 & 5.3941E+03 & Direct-PRF & 0\\
009899256-01 & BR-Cyg-pri & 1:1 & 261.3 & 56 & 34 & 10.03 & 4.25 & 2.4773E+04 & Direct-PRF & 0\\
009899280-01 & BR-Cyg-pri & 1:1 & 104.9 & 22 & -15 & 10.03 & 5.01 & 4.0538E+03 & Direct-PRF & 0\\
009899315-01 & BR-Cyg-pri & 1:1 & 203.7 & 39 & 33 & 10.03 & 5.35 & 9.2898E+03 & Direct-PRF & 0\\
009899352-01 & BR-Cyg-pri & 1:1 & 135.3 & 25 & 22 & 10.03 & 5.82 & 4.6129E+03 & Direct-PRF & 0\\
009899355-01 & 009899416-01 & 1:1 & 108.1 & 21 & 16 & 10.03 & 5.84 & 5.7042E+03 & Direct-PRF & 0\\
009899410-01 & BR-Cyg-pri & 1:1 & 89.5 & 12 & 18 & 10.03 & 3.48 & 8.2576E+03 & Direct-PRF & 0\\
009899414-01 & BR-Cyg-pri & 1:1 & 43.4 & 6 & 9 & 10.03 & 4.89 & 3.5204E+03 & Direct-PRF & 0\\
009899421-01 & BR-Cyg-pri & 1:1 & 53.4 & 4 & 12 & 10.03 & 2.27 & 8.6866E+03 & Direct-PRF & 0\\
009899449-01 & BR-Cyg-pri & 1:1 & 51.9 & -13 & -3 & 10.03 & 5.60 & 1.3540E+03 & Direct-PRF & 0\\
009899483-01 & BR-Cyg-pri & 1:1 & 105.9 & -4 & 26 & 10.03 & 3.59 & 8.3609E+03 & Direct-PRF & 0\\
009899505-01 & BR-Cyg-pri & 1:1 & 85.2 & -17 & 13 & 10.03 & 5.92 & 7.1921E+03 & Direct-PRF & 0\\
009899514-01 & BR-Cyg-pri & 1:1 & 166.0 & -2 & 41 & 10.03 & 5.89 & 5.1451E+03 & Direct-PRF & 0\\
009899577-01 & BR-Cyg-pri & 1:1 & 149.9 & -25 & 28 & 10.03 & 4.79 & 9.1626E+03 & Direct-PRF & 0\\
009899583-01 & BR-Cyg-pri & 1:1 & 182.5 & -19 & 42 & 10.03 & 4.81 & 1.2056E+04 & Direct-PRF & 0\\
009899607-01 & BR-Cyg-pri & 1:1 & 168.4 & -32 & 27 & 10.03 & 5.27 & 9.2898E+03 & Direct-PRF & 0\\
009899621-01 & BR-Cyg-pri & 1:1 & 241.0 & -19 & 57 & 10.03 & 5.24 & 9.5553E+03 & Direct-PRF & 0\\
009899623-01 & BR-Cyg-pri & 1:1 & 183.1 & -45 & 12 & 10.03 & 5.95 & 7.6008E+03 & Direct-PRF & 0\\
009899630-01 & BR-Cyg-pri & 1:1 & 189.7 & -35 & 33 & 10.03 & 5.53 & 6.2511E+03 & Direct-PRF & 0\\
009899682-01 & BR-Cyg-pri & 1:1 & 231.5 & -56 & 18 & 10.03 & 5.37 & 1.5925E+04 & Direct-PRF & 0\\
009910828-01 & 009851142-pri & 1:1 & 206.6 & -21 & 47 & 7.63 & 7.25 & 4.6718E+02 & Direct-PRF & 0\\
009910942-01 & 009851142-pri & 1:1 & 183.3 & -33 & 32 & 7.63 & 5.17 & 2.3359E+03 & Direct-PRF & 0\\
009934274-01 & 7241.01 & 1:1 & 458.1 & 116 & -1 & 13.04 & 0.31 & 5.2184E+03 & Col-Anomaly & 0\\
009950201-02 & 009950279-01 & 1:1 & 138.2 & 35 & -1 & 15.65 & 0.04 & 1.3561E+00 & Col-Anomaly & 1\\
009950279-01 & 009950201-02 & 1:1 & 138.2 & -35 & 1 & 15.70 & -0.04 & 7.3738E-01 & Col-Anomaly & 1\\
009957659-01 & 5744.01 & 1:1 & 9.6 & 2 & 1 & 12.51 & 2.99 & 4.5073E+00 & Direct-PRF & 0\\
009959368-01 & BR-Cyg-pri & 1:1 & 240.9 & 20 & -57 & 10.03 & 5.28 & 1.3650E+04 & Direct-PRF & 0\\
009959492-01 & BR-Cyg-pri & 1:1 & 184.6 & -6 & -46 & 10.03 & 5.25 & 1.0617E+04 & Direct-PRF & 0\\
009959494-01 & BR-Cyg-pri & 1:1 & 127.6 & 1 & -32 & 10.03 & 1.81 & 3.7159E+04 & Direct-PRF & 0\\
009959545-01 & BR-Cyg-pri & 1:1 & 141.5 & -14 & -33 & 10.03 & 4.12 & 1.5555E+04 & Direct-PRF & 0\\
009959589-01 & BR-Cyg-pri & 1:1 & 127.2 & -21 & -25 & 10.03 & 5.76 & 4.5501E+03 & Direct-PRF & 0\\
009959765-01 & 009838414-01 & 1:1 & 1402.7 & -352 & 1 & 17.51 & -3.72 & 3.9773E+01 & Col-Anomaly & 1\\
009965184-01 & 009965206-02 & 1:1 & 12.5 & -3 & 0 & 15.90 & -0.51 & 3.2562E+02 & Direct-PRF & 0\\
009965184-02 & 3558.01 & 1:1 & 12.5 & -3 & 0 & 15.90 & -0.51 & 4.2660E+02 & Direct-PRF & 0\\
010002266-01 & 010002261-pri & 1:1 & 22.4 & 5 & -2 & 13.10 & 2.03 & 1.9492E+02 & Direct-PRF & 0\\
010014702-01 & 5742.01 & 1:1 & 157.5 & 40 & 1 & 14.56 & 0.57 & 1.1226E+04 & Col-Anomaly & 0\\
010015534-01 & 010015516-pri & 1:1 & 24.5 & -6 & 1 & 10.70 & 0.49 & 2.2102E+03 & Direct-PRF & 0\\
010026458-01 & 7275.01 & 1:1 & 7.4 & -1 & -2 & 15.39 & 0.39 & 2.3715E+01 & Direct-PRF & 0\\
010026458-02 & 010026457-sec & 1:1 & 7.4 & -1 & -2 & 15.39 & 0.39 & 2.4262E+01 & Direct-PRF & 0\\
010031500-01 & 010031808-01 & 1:1 & 228.3 & 58 & 2 & 9.56 & 5.66 & 1.4218E+03 & Direct-PRF & 0\\
010031526-01 & 010031808-01 & 1:1 & 188.8 & 41 & 25 & 9.56 & 6.13 & 1.4070E+03 & Direct-PRF & 0\\
010031643-01 & 010031808-01 & 1:1 & 195.5 & 9 & 48 & 9.56 & 4.92 & 3.2944E+03 & Direct-PRF & 0\\
010031656-01 & 010031808-01 & 1:1 & 112.5 & 19 & 21 & 9.56 & 5.85 & 8.7707E+02 & Direct-PRF & 0\\
010031707-01 & 010031808-01 & 1:1 & 68.7 & 18 & 0 & 9.56 & 4.31 & 5.4795E+02 & Direct-PRF & 0\\
010031707-02 & 010031808-02 & 1:1 & 68.7 & 18 & 0 & 9.56 & 4.31 & 6.4558E+02 & Direct-PRF & 0\\
010031885-01 & 010031808-01 & 1:1 & 62.5 & -15 & 2 & 9.56 & 3.92 & 1.1953E+03 & Direct-PRF & 0\\
010031885-02 & 010031808-02 & 1:1 & 62.5 & -15 & 2 & 9.56 & 3.92 & 1.3913E+03 & Direct-PRF & 0\\
010031907-01 & 010031808-01 & 1:1 & 69.4 & -17 & 0 & 9.56 & 5.09 & 2.6253E+02 & Direct-PRF & 0\\
010031907-02 & 010031808-02 & 1:1 & 69.4 & -17 & 0 & 9.56 & 5.09 & 2.9888E+02 & Direct-PRF & 0\\
010031918-01 & 010031808-01 & 1:1 & 117.8 & -26 & 13 & 9.56 & 5.28 & 2.3490E+03 & Direct-PRF & 0\\
010068024-01 & 529.01 & 1:1 & 5.8 & 2 & 1 & 14.98 & -1.85 & 2.2100E+01 & Direct-PRF & 0\\
010090219-01 & 010090246-pri & 1:1 & 16.7 & -3 & 2 & 13.57 & 1.55 & 8.1795E+02 & Direct-PRF & 0\\
010090257-01 & 010090246-pri & 1:1 & 15.3 & 2 & -4 & 13.57 & 1.98 & 7.2914E+02 & Direct-PRF & 0\\
010092312-02 & 1080.01 & 1:1 & 9.9 & -1 & -2 & 14.87 & -0.91 & 1.7688E+00 & Direct-PRF & 0\\
010095484-01 & 010095469-pri & 1:1 & 15.2 & -3 & 1 & 14.69 & -0.31 & 2.6337E+03 & Direct-PRF & 0\\
010130057-01 & FL-Lyr-pri & 1:1 & 3770.8 & -384 & 5 & 9.18 & 6.44 & 4.7289E+03 & Col-Anomaly & 0\\
010156055-01 & 010156064-pri & 1:2 & 58.1 & -8 & 12 & 10.37 & 3.68 & 1.8588E+03 & Direct-PRF & 0\\
010156110-01 & 010156064-pri & 1:1 & 100.6 & -2 & 9 & 10.37 & 4.46 & 1.6416E+03 & Direct-PRF & 0\\
010158990-01 & 1823.02 & 1:1 & 9.9 & 1 & 2 & 13.95 & 0.91 & 4.7895E+00 & Direct-PRF & 0\\
010189542-01 & 427.01 & 1:1 & 6.4 & 0 & 1 & 14.62 & -0.28 & 8.0258E+00 & Direct-PRF & 0\\
010191036-01 & 5774.01 & 1:1 & 66.2 & 17 & -2 & 10.81 & 1.30 & 8.0400E+03 & Direct-PRF & 0\\
010191070-01 & 5774.01 & 1:1 & 26.5 & -1 & -7 & 10.81 & 5.01 & 1.3209E+03 & Direct-PRF & 0\\
010226316-01 & 010226388-pri & 1:1 & 64.7 & 7 & 14 & 10.77 & 3.69 & 1.2167E+04 & Direct-PRF & 0\\
010226343-01 & 010226388-pri & 1:1 & 72.3 & 14 & -12 & 10.77 & 4.89 & 2.0555E+02 & Direct-PRF & 0\\
010226382-01 & 010226451-01 & 1:1 & 42.1 & 10 & 3 & 14.95 & -1.23 & 3.1818E+00 & Direct-PRF & 1\\
010226420-01 & 010226388-pri & 1:1 & 56.0 & -11 & 9 & 10.77 & 4.01 & 6.2317E+03 & Direct-PRF & 0\\
010226448-01 & 010226451-01 & 1:1 & 94.5 & 11 & -21 & 14.95 & -0.94 & 3.8889E+00 & Direct-PRF & 1\\
010226451-01 & 010226388-pri & 1:1 & 66.5 & -15 & 8 & 10.77 & 4.17 & 7.3000E+03 & Direct-PRF & 0\\
010226479-01 & 010226498-01 & 1:1 & 38.3 & 8 & -6 & 14.93 & 0.29 & 1.1111E+00 & Direct-PRF & 1\\
010226488-01 & 010226451-01 & 1:1 & 32.8 & -8 & 2 & 14.95 & -0.72 & 2.3333E+00 & Direct-PRF & 1\\
010226498-01 & 010226451-01 & 1:1 & 34.5 & -6 & -7 & 14.95 & -0.01 & 1.7500E+00 & Direct-PRF & 1\\
010227863-01 & 5780.01 & 1:1 & 20.2 & 4 & -3 & 15.53 & -1.77 & 7.8475E+00 & Direct-PRF & 1\\
010227881-01 & 3983.01 & 1:1 & 20.2 & -4 & 3 & 13.75 & 1.77 & 5.7092E-01 & Direct-PRF & 0\\
010259031-01 & 3630.01 & 1:1 & 6.1 & -2 & 1 & 17.11 & -1.52 & 1.0371E+02 & Direct-PRF & 0\\
010259031-02 & 010259029-02 & 1:1 & 6.1 & -2 & 1 & 17.11 & -1.52 & 5.7613E+01 & Direct-PRF & 0\\
010266860-01 & FL-Lyr-pri & 1:1 & 4294.0 & 32 & 4 & 9.18 & 4.25 & 1.6733E+04 & Col-Anomaly & 0\\
010268907-01 & 3773.01 & 1:2 & 6.0 & -1 & 0 & 17.36 & -1.63 & 4.9769E+02 & Direct-PRF & 0\\
010272389-01 & V850-Cyg-pri & 1:1 & 311.7 & 78 & 1 & 11.20 & 3.14 & 2.9797E+03 & Direct-PRF & 0\\
010272394-01 & V850-Cyg-pri & 1:1 & 299.6 & 75 & 1 & 11.20 & 4.08 & 9.7080E+03 & Direct-PRF & 0\\
010275766-01 & 010275747-pri & 1:1 & 31.0 & 4 & 6 & 12.80 & 2.60 & 6.8203E+03 & Direct-PRF & 0\\
010275880-01 & 010275887-pri & 1:1 & 10.0 & 2 & -1 & 13.04 & 0.17 & 5.9447E+01 & Direct-PRF & 0\\
010275880-02 & 010275887-sec & 1:1 & 10.0 & 2 & -1 & 13.04 & 0.17 & 1.2466E+02 & Direct-PRF & 0\\
010292554-01 & 010226388-pri & 1:1 & 108.4 & -19 & 19 & 10.77 & 3.91 & 1.1109E+04 & Direct-PRF & 0\\
010294509-01 & 010294608-pri & 1:2 & 67.8 & 17 & 1 & 13.34 & 2.36 & 1.5803E+03 & Direct-PRF & 0\\
010294613-01 & 010294608-01 & 1:1 & 16.1 & -3 & 3 & 13.34 & 1.55 & 7.9353E+02 & Direct-PRF & 0\\
010322797-01 & 010191036-01 & 1:1 & 727.6 & 183 & 3 & 12.11 & 1.10 & 1.2778E+00 & Col-Anomaly & 1\\
010339975-01 & V2083-Cyg-pri & 1:2 & 1956.2 & 263 & -416 & 6.90 & 8.72 & 4.9580E+03 & Direct-PRF & 0\\
010340115-01 & V2083-Cyg-pri & 1:2 & 1810.3 & 207 & -406 & 6.90 & 8.51 & 4.2196E+03 & Direct-PRF & 0\\
010340212-01 & 010340115-01 & 1:1 & 95.3 & -1 & 24 & 15.41 & -1.60 & 5.0538E-01 & Direct-PRF & 1\\
010340228-01 & V2083-Cyg-pri & 1:2 & 1699.4 & 228 & -362 & 6.90 & 8.89 & 3.3054E+03 & Direct-PRF & 0\\
010341755-01 & V2083-Cyg-pri & 1:2 & 267.2 & 24 & -63 & 6.90 & 8.77 & 2.6443E+03 & Direct-PRF & 0\\
010341777-01 & V2083-Cyg-pri & 1:2 & 246.8 & 24 & -58 & 6.90 & 6.18 & 1.4166E+04 & Direct-PRF & 0\\
010341781-01 & 010341755-01 & 1:1 & 24.4 & 0 & 6 & 15.67 & -0.27 & 1.0135E+00 & Direct-PRF & 1\\
010341787-01 & 010407271-01 & 1:1 & 547.6 & -48 & 2 & 14.98 & 0.94 & 1.7164E-01 & Col-Anomaly & 1\\
010341831-01 & 2823.01 & 1:1 & 170.6 & 43 & -3 & 15.81 & -0.85 & 7.1720E+00 & Col-Anomaly & 1\\
010341878-01 & V2083-Cyg-pri & 1:2 & 184.1 & -6 & -46 & 6.90 & 6.33 & 1.4166E+04 & Direct-PRF & 0\\
010341905-01 & 2823.01 & 1:1 & 12.1 & 1 & -3 & 15.81 & -0.57 & 5.2520E+00 & Direct-PRF & 0\\
010341913-01 & 010407221-pri & 1:1 & 360.3 & -47 & 14 & 15.65 & -2.57 & 4.5455E+01 & Col-Anomaly & 1\\
010341917-01 & 2605.01 & 1:1 & 387.6 & -56 & 11 & 15.65 & 0.16 & 3.2716E+00 & Col-Anomaly & 1\\
010342041-01 & 010342065-01 & 1:1 & 47.6 & 12 & 0 & 13.96 & 0.69 & 3.3940E-01 & Direct-PRF & 1\\
010342065-01 & V2083-Cyg-pri & 1:2 & 58.9 & -5 & -13 & 6.90 & 7.06 & 3.4312E+02 & Direct-PRF & 0\\
010342097-01 & V2083-Cyg-pri & 1:2 & 102.9 & 3 & -25 & 6.90 & 6.60 & 4.1317E+03 & Direct-PRF & 0\\
010342248-01 & V2083-Cyg-pri & 1:2 & 229.2 & -34 & -45 & 6.90 & 7.86 & 3.3054E+03 & Direct-PRF & 0\\
010342316-01 & 010341755-01 & 1:1 & 562.8 & -47 & -6 & 15.67 & -0.35 & 3.9474E+00 & Col-Anomaly & 1\\
010352945-01 & 010352938-pri & 1:1 & 7.3 & 2 & 2 & 14.35 & 1.05 & 2.0548E+01 & Direct-PRF & 0\\
010363281-01 & 010363300-pri & 1:1 & 15.2 & 2 & 3 & 14.68 & -2.37 & 2.7633E+03 & Direct-PRF & 0\\
010383687-01 & 3671.01 & 1:1 & 10.9 & -1 & -3 & 16.95 & -3.65 & 1.1655E+03 & Direct-PRF & 0\\
010383729-01 & 010383620-pri & 1:1 & 245.6 & 61 & -1 & 12.83 & 0.76 & 1.0577E+04 & Col-Anomaly & 0\\
010397315-01 & FL-Lyr-pri & 1:1 & 4676.2 & -143 & 4 & 9.18 & 5.18 & 7.9102E+03 & Col-Anomaly & 0\\
010405224-01 & V2083-Cyg-pri & 1:2 & 1926.2 & 277 & -398 & 6.90 & 8.99 & 3.1480E+03 & Direct-PRF & 0\\
010405482-01 & V2083-Cyg-pri & 1:2 & 1694.7 & 284 & -318 & 6.90 & 8.29 & 9.9161E+03 & Direct-PRF & 0\\
010405546-01 & V2083-Cyg-pri & 1:2 & 1638.7 & 276 & -307 & 6.90 & 6.78 & 1.1666E+04 & Direct-PRF & 0\\
010405926-01 & V2083-Cyg-pri & 1:2 & 1271.1 & 220 & -232 & 6.90 & 8.21 & 9.0146E+03 & Direct-PRF & 0\\
010407020-01 & V2083-Cyg-pri & 1:2 & 170.4 & 41 & -13 & 6.90 & 6.47 & 7.3453E+03 & Direct-PRF & 0\\
010407047-01 & V2083-Cyg-pri & 1:2 & 232.4 & 59 & -5 & 6.90 & 6.42 & 3.1987E+03 & Direct-PRF & 0\\
010407054-01 & 1155.01 & 1:1 & 242.7 & 61 & 1 & 14.66 & -1.31 & 9.4302E+01 & Col-Anomaly & 1\\
010407086-01 & V2083-Cyg-pri & 1:2 & 349.6 & 82 & -31 & 6.90 & 5.98 & 1.2395E+04 & Direct-PRF & 0\\
010407210-01 & V2083-Cyg-pri & 1:2 & 265.9 & 51 & -43 & 6.90 & 4.06 & 2.4790E+04 & Direct-PRF & 0\\
010407221-01 & 2823.01 & 1:1 & 387.6 & 56 & -11 & 15.81 & -0.16 & 5.0530E+00 & Col-Anomaly & 1\\
010407271-01 & 010341787-01 & 1:1 & 547.6 & 48 & -2 & 15.93 & -0.94 & 5.8261E+00 & Col-Anomaly & 1\\
010407430-01 & V2083-Cyg-pri & 1:2 & 306.4 & -11 & -75 & 6.90 & 8.72 & 4.2196E+03 & Direct-PRF & 0\\
010407464-01 & V2083-Cyg-pri & 1:2 & 352.3 & -3 & -87 & 6.90 & 5.82 & 1.9832E+04 & Direct-PRF & 0\\
010420301-01 & 010420279-01 & 7:1 & 13.1 & 2 & 2 & 14.77 & 1.00 & 3.9102E+02 & Direct-PRF & 0\\
010420301-02 & 010420279-02 & 1:1 & 13.1 & 2 & 2 & 14.77 & 1.00 & 6.2673E+02 & Direct-PRF & 0\\
010420301-03 & 010420279-01 & 8:1 & 13.1 & 2 & 2 & 14.77 & 1.00 & 3.9102E+02 & Direct-PRF & 0\\
010420301-04 & 7325.01 & 4:1 & 13.1 & 2 & 2 & 14.77 & 1.00 & 5.3584E+02 & Direct-PRF & 0\\
010470882-01 & V2083-Cyg-pri & 1:2 & 1853.6 & 339 & -320 & 6.90 & 9.06 & 2.8332E+03 & Direct-PRF & 0\\
010470935-01 & V2083-Cyg-pri & 1:2 & 1809.7 & 342 & -301 & 6.90 & 8.84 & 4.8371E+03 & Direct-PRF & 0\\
010470993-01 & V2083-Cyg-pri & 1:2 & 1790.6 & 351 & -283 & 6.90 & 7.71 & 8.6227E+03 & Direct-PRF & 0\\
010471005-01 & V2083-Cyg-pri & 1:2 & 1744.7 & 325 & -296 & 6.90 & 8.00 & 5.0852E+03 & Direct-PRF & 0\\
010471055-01 & V2083-Cyg-pri & 1:2 & 1726.2 & 330 & -283 & 6.90 & 8.12 & 5.0852E+03 & Direct-PRF & 0\\
010471090-01 & V2083-Cyg-pri & 1:2 & 1744.6 & 360 & -252 & 6.90 & 7.49 & 8.2634E+03 & Direct-PRF & 0\\
010471107-01 & 7612.01 & 1:1 & 69.0 & 12 & -13 & 13.01 & 2.22 & 5.3667E+00 & Direct-PRF & 1\\
010471167-01 & V2083-Cyg-pri & 1:2 & 1696.6 & 362 & -226 & 6.90 & 6.10 & 3.4793E+03 & Direct-PRF & 0\\
010471174-01 & 010471167-01 & 1:1 & 103.3 & -23 & -12 & 13.01 & 2.98 & 8.7692E-01 & Direct-PRF & 1\\
010471204-01 & 7613.01 & 1:1 & 52.8 & -13 & -1 & 15.98 & -0.16 & 2.2222E+00 & Direct-PRF & 1\\
010471243-01 & V2083-Cyg-pri & 1:2 & 1554.2 & 311 & -237 & 6.90 & 8.63 & 5.3601E+03 & Direct-PRF & 0\\
010471270-01 & V2083-Cyg-pri & 1:2 & 1487.0 & 282 & -246 & 6.90 & 8.79 & 3.0049E+03 & Direct-PRF & 0\\
010471296-01 & V2083-Cyg-pri & 1:2 & 1494.6 & 301 & -225 & 6.90 & 7.74 & 8.6227E+03 & Direct-PRF & 0\\
010471328-01 & V2083-Cyg-pri & 1:2 & 1485.2 & 306 & -214 & 6.90 & 9.09 & 3.8887E+03 & Direct-PRF & 0\\
010471345-01 & V2083-Cyg-pri & 1:2 & 1469.3 & 303 & -212 & 6.90 & 8.86 & 3.2512E+03 & Direct-PRF & 0\\
010480921-01 & 5797.01 & 1:1 & 33.7 & -8 & 3 & 12.22 & 1.97 & 2.4794E+03 & Direct-PRF & 0\\
010480982-02 & 5797.01 & 1:1 & 74.0 & 14 & -12 & 12.22 & 3.12 & 2.7946E+03 & Direct-PRF & 0\\
010481045-01 & 5797.01 & 1:1 & 96.7 & 24 & 2 & 12.22 & 2.83 & 2.8185E+03 & Direct-PRF & 0\\
010481054-01 & 5797.01 & 1:1 & 118.0 & 13 & 27 & 12.22 & 1.71 & 1.1371E+04 & Direct-PRF & 0\\
010485047-01 & T-Cyg1-03567-pri & 2:1 & 62.2 & -8 & -14 & 11.88 & 3.89 & 3.9445E+03 & Direct-PRF & 0\\
010485165-01 & T-Cyg1-03567-pri & 2:1 & 66.5 & 13 & -10 & 11.88 & 2.63 & 7.8890E+03 & Direct-PRF & 0\\
010485179-01 & T-Cyg1-03567-pri & 2:1 & 37.0 & 9 & 0 & 11.88 & 2.62 & 1.0905E+04 & Direct-PRF & 0\\
010489525-01 & 3625.01 & 1:2 & 11.8 & -2 & -2 & 16.17 & -3.39 & 4.7350E+03 & Direct-PRF & 0\\
010491044-01 & 7336.01 & 1:1 & 21.0 & -4 & 3 & 13.24 & 2.71 & 6.0536E+02 & Direct-PRF & 0\\
010491062-01 & 7336.01 & 1:1 & 16.9 & -4 & -2 & 13.24 & 2.09 & 4.1051E+02 & Direct-PRF & 0\\
010491544-01 & 3576.01 & 1:1 & 4.4 & 1 & 1 & 15.02 & -1.58 & 8.4382E+00 & Direct-PRF & 0\\
010491544-02 & 010491554-02 & 1:1 & 4.4 & 1 & 1 & 15.02 & -1.58 & 7.8724E+00 & Direct-PRF & 0\\
010514429-01 & 010514430-03 & 1:4 & 2.1 & -1 & -1 & 10.82 & 0.59 & 1.3289E+00 & Direct-PRF & 0\\
010514430-02 & 1614.01 & 2:1 & 2.1 & 1 & 1 & 11.41 & -0.59 & 1.3596E+00 & Direct-PRF & 0\\
010518399-01 & 010583181-pri & 1:1 & 106.1 & -4 & 26 & 11.01 & 3.51 & 2.5350E+03 & Direct-PRF & 0\\
010518424-01 & 010583181-pri & 1:1 & 85.0 & -11 & 19 & 11.01 & 4.31 & 1.4006E+03 & Direct-PRF & 0\\
010518424-02 & 010583181-sec & 1:1 & 85.0 & -11 & 19 & 11.01 & 4.31 & 1.0720E+03 & Direct-PRF & 0\\
010518725-01 & 3612.01 & 1:1 & 14.6 & 4 & 1 & 16.74 & -3.62 & 2.4709E+03 & Direct-PRF & 0\\
010518725-02 & 010518735-02 & 1:1 & 14.6 & 4 & 1 & 16.74 & -3.62 & 1.7845E+03 & Direct-PRF & 0\\
010535696-01 & V2083-Cyg-pri & 1:2 & 1992.0 & 444 & -234 & 6.90 & 8.38 & 4.9580E+03 & Direct-PRF & 0\\
010535708-01 & V2083-Cyg-pri & 1:2 & 1927.9 & 417 & -248 & 6.90 & 8.71 & 4.5073E+03 & Direct-PRF & 0\\
010535848-01 & V2083-Cyg-pri & 1:2 & 1826.9 & 404 & -220 & 6.90 & 7.94 & 5.8330E+03 & Direct-PRF & 0\\
010535858-01 & 7614.01 & 1:1 & 466.3 & 118 & 4 & 15.76 & -0.33 & 1.1250E+00 & Col-Anomaly & 1\\
010535867-01 & 7338.01 & 1:1 & 9.3 & -1 & 2 & 15.43 & -0.04 & 2.2759E+00 & Direct-PRF & 0\\
010535886-01 & V2083-Cyg-pri & 1:2 & 1830.9 & 413 & -204 & 6.90 & 8.54 & 3.4193E+03 & Direct-PRF & 0\\
010535897-01 & 7612.01 & 1:1 & 119.5 & 28 & 11 & 13.01 & 0.79 & 1.2385E+01 & Direct-PRF & 1\\
010535926-01 & 010535886-01 & 1:1 & 71.4 & 7 & 16 & 15.45 & -0.53 & 2.4167E+00 & Direct-PRF & 1\\
010535991-01 & V2083-Cyg-pri & 1:2 & 1721.9 & 394 & -181 & 6.90 & 8.86 & 4.1317E+03 & Direct-PRF & 0\\
010536006-01 & V2083-Cyg-pri & 1:2 & 1686.0 & 384 & -181 & 6.90 & 8.43 & 6.3975E+03 & Direct-PRF & 0\\
010549562-01 & 7341.01 & 1:1 & 14.3 & -3 & 3 & 13.02 & 1.39 & 1.4706E+02 & Direct-PRF & 0\\
010549562-02 & 010549576-sec & 1:1 & 14.3 & -3 & 3 & 13.02 & 1.39 & 1.8200E+02 & Direct-PRF & 0\\
010555375-01 & 3771.01 & 1:1 & 6.7 & -2 & 0 & 16.61 & -2.85 & 9.7872E+01 & Direct-PRF & 0\\
010583180-01 & 010583181-pri & 1:1 & 52.9 & -10 & 9 & 11.01 & 4.26 & 7.7287E+02 & Direct-PRF & 0\\
010583180-02 & 010583181-sec & 1:1 & 52.9 & -10 & 9 & 11.01 & 4.26 & 9.1468E+02 & Direct-PRF & 0\\
010583225-01 & 010583181-pri & 1:1 & 71.8 & -17 & -4 & 11.01 & 3.54 & 1.4403E+03 & Direct-PRF & 0\\
010583225-02 & 010583181-sec & 1:1 & 71.8 & -17 & -4 & 11.01 & 3.54 & 1.8811E+03 & Direct-PRF & 0\\
010601538-01 & 010601549-pri & 1:1 & 19.1 & 5 & 1 & 13.32 & -0.15 & 2.1226E+03 & Direct-PRF & 0\\
010618236-01 & 010618322-01 & 1:1 & 64.8 & 17 & 0 & 12.96 & 2.57 & 1.0580E+00 & Direct-PRF & 1\\
010618322-01 & 010618236-01 & 1:1 & 64.8 & -17 & 0 & 15.53 & -2.57 & 9.4521E-01 & Direct-PRF & 1\\
010619142-01 & 010619109-pri & 1:1 & 83.0 & -14 & -16 & 11.70 & 3.27 & 1.8162E+03 & Direct-PRF & 0\\
010621666-01 & 7363.01 & 1:1 & 56.6 & 0 & 14 & 11.73 & 2.87 & 1.3874E+03 & Direct-PRF & 0\\
010661679-01 & 010661783-pri & 1:1 & 110.6 & -19 & -20 & 9.59 & 5.22 & 4.1885E+03 & Direct-PRF & 0\\
010661718-01 & 010661783-pri & 1:1 & 66.9 & -15 & -9 & 9.59 & 5.69 & 1.9446E+03 & Direct-PRF & 0\\
010661771-01 & 010661783-pri & 1:1 & 41.2 & 7 & -8 & 9.59 & 5.38 & 2.5034E+03 & Direct-PRF & 0\\
010661778-01 & 010661783-pri & 1:1 & 42.6 & -10 & 5 & 9.59 & 8.08 & 3.2315E+02 & Direct-PRF & 0\\
010661913-01 & 010661783-pri & 1:1 & 124.7 & 27 & 16 & 9.59 & 5.29 & 3.5129E+03 & Direct-PRF & 0\\
010661917-01 & 010661783-pri & 1:1 & 129.0 & 26 & 19 & 9.59 & 3.39 & 1.3612E+04 & Direct-PRF & 0\\
010661976-01 & 010661783-pri & 1:1 & 197.0 & 12 & 48 & 9.59 & 4.15 & 1.3612E+04 & Direct-PRF & 0\\
010662021-01 & 010661783-pri & 1:1 & 237.3 & 17 & 57 & 9.59 & 5.56 & 5.5846E+03 & Direct-PRF & 0\\
010676923-01 & 010676927-pri & 1:1 & 10.8 & -2 & 2 & 17.02 & -1.89 & 1.4293E+03 & Direct-PRF & 0\\
010686814-01 & 7363.01 & 1:1 & 56.1 & 14 & -3 & 11.73 & 3.87 & 8.3342E+02 & Direct-PRF & 0\\
010686909-01 & 7363.01 & 1:1 & 47.1 & -10 & -6 & 11.73 & 1.41 & 1.2194E+04 & Direct-PRF & 0\\
010686930-01 & 7363.01 & 1:1 & 61.3 & -15 & -4 & 11.73 & 0.66 & 5.9408E+03 & Direct-PRF & 0\\
010724372-01 & 010724533-pri & 1:1 & 188.2 & -10 & 46 & 9.04 & 5.58 & 4.3793E+03 & Direct-PRF & 0\\
010724379-01 & 010724429-01 & 1:1 & 69.7 & -16 & 6 & 14.91 & 0.45 & 5.0000E-01 & Direct-PRF & 1\\
010724429-01 & 010724379-01 & 1:1 & 69.7 & 16 & -6 & 15.36 & -0.45 & 2.0000E+00 & Direct-PRF & 1\\
010724450-01 & 010724551-01 & 1:1 & 109.8 & -14 & 23 & 15.88 & -2.28 & 5.8333E+00 & Direct-PRF & 1\\
010724544-01 & 010724533-pri & 2:1 & 88.7 & 20 & 11 & 9.04 & 5.97 & 1.4767E+03 & Direct-PRF & 0\\
010724544-02 & 010724533-pri & 2:1 & 88.7 & 20 & 11 & 9.04 & 5.97 & 1.2828E+03 & Direct-PRF & 0\\
010724551-01 & 010724450-01 & 1:1 & 109.8 & 14 & -23 & 13.60 & 2.28 & 1.7143E-01 & Direct-PRF & 1\\
010724569-01 & 010724533-pri & 1:1 & 112.7 & 27 & 10 & 9.04 & 6.45 & 2.0159E+03 & Direct-PRF & 0\\
010724619-01 & 010724569-01 & 1:1 & 54.6 & 0 & -14 & 15.49 & -0.20 & 1.5000E+00 & Direct-PRF & 1\\
010724621-01 & 010724569-01 & 1:1 & 52.7 & 12 & -7 & 15.49 & -0.87 & 3.7059E+00 & Direct-PRF & 1\\
010724635-01 & 010724533-pri & 1:1 & 84.7 & 16 & -15 & 9.04 & 5.51 & 4.3793E+03 & Direct-PRF & 0\\
010732401-01 & 010342041-01 & 1:1 & 2252.9 & 566 & 12 & 14.66 & 0.08 & 1.0644E+02 & Col-Anomaly & 0\\
010735575-01 & 3617.01 & 1:1 & 12.1 & -2 & -2 & 14.57 & -2.86 & 4.5153E+03 & Direct-PRF & 0\\
010736179-01 & V2290-Cyg-pri & 2:1 & 46.5 & 9 & 7 & 13.65 & 2.16 & 5.2158E+03 & Direct-PRF & 0\\
010736179-02 & V2290-Cyg-pri & 1:1 & 46.5 & 9 & 7 & 13.65 & 2.16 & 6.2674E+03 & Direct-PRF & 0\\
010743597-01 & 010743600-01 & 1:1 & 5.6 & 0 & -1 & 17.21 & -1.72 & 7.0889E+02 & Direct-PRF & 0\\
010747439-01 & 2673.01 & 1:1 & 5.8 & 1 & 1 & 16.44 & -1.99 & 3.3853E+01 & Direct-PRF & 0\\
010748393-01 & 010748390-01 & 1:1 & 11.0 & -2 & -2 & 9.17 & 6.22 & 1.4550E+00 & Direct-PRF & 0\\
010749745-01 & 010815379-pri & 1:1 & 80.2 & 20 & 3 & 11.24 & 2.80 & 3.2080E+03 & Direct-PRF & 0\\
010749766-01 & 010815379-pri & 1:1 & 59.9 & 15 & 3 & 11.24 & 3.40 & 2.3588E+03 & Direct-PRF & 0\\
010749841-01 & 010749766-01 & 1:1 & 38.2 & -9 & 3 & 14.64 & -0.14 & 1.4783E+00 & Direct-PRF & 1\\
010777060-01 & 010842687-02 & 1:1 & 51.5 & 11 & 5 & 13.19 & -2.04 & 7.0370E-01 & Direct-PRF & 1\\
010777060-02 & 010842687-01 & 1:1 & 51.5 & 11 & 5 & 13.19 & -2.04 & 1.1176E+00 & Direct-PRF & 1\\
010794405-02 & 010858720-pri & 1:1 & 22.8 & 1 & -6 & 10.97 & 3.74 & 1.0919E+02 & Direct-PRF & 0\\
010794509-01 & 010858720-pri & 1:1 & 169.4 & 43 & 0 & 10.97 & 1.65 & 3.4207E+04 & Direct-PRF & 0\\
010794509-02 & 010858720-sec & 1:1 & 169.4 & 43 & 0 & 10.97 & 1.65 & 4.1809E+04 & Direct-PRF & 0\\
010796473-01 & 010796477-pri & 2:1 & 22.6 & 6 & 1 & 14.11 & 0.91 & 8.3067E+03 & Direct-PRF & 0\\
010801249-01 & 3617.01 & 1:1 & 498.2 & 125 & 0 & 14.57 & -1.20 & 7.5255E+03 & Col-Anomaly & 0\\
010801951-01 & V2290-Cyg-pri & 1:1 & 399.6 & 101 & 0 & 13.65 & 0.86 & 2.9891E+04 & Col-Anomaly & 0\\
010842687-01 & 010777060-02 & 1:1 & 51.5 & -11 & -5 & 11.16 & 2.04 & 8.9474E-01 & Direct-PRF & 1\\
010842687-02 & 010777060-01 & 1:1 & 51.5 & -11 & -5 & 11.16 & 2.04 & 1.4211E+00 & Direct-PRF & 1\\
010858737-01 & 010858720-pri & 1:1 & 88.3 & -14 & 17 & 10.97 & 2.57 & 1.4085E+04 & Direct-PRF & 0\\
010858737-03 & 010858720-sec & 1:1 & 88.3 & -14 & 17 & 10.97 & 2.57 & 2.2995E+04 & Direct-PRF & 0\\
010858785-01 & 010858720-pri & 1:1 & 74.4 & 4 & 18 & 10.97 & 4.90 & 4.4757E+03 & Direct-PRF & 0\\
010858785-02 & 010858803-02 & 1:1 & 23.0 & -5 & -3 & 15.61 & 0.26 & 3.1538E+00 & Direct-PRF & 1\\
010858803-01 & 010858720-pri & 1:1 & 91.1 & 9 & 21 & 10.97 & 4.64 & 5.2626E+03 & Direct-PRF & 0\\
010858803-02 & 010858720-sec & 1:1 & 91.1 & 9 & 21 & 10.97 & 4.64 & 5.6085E+03 & Direct-PRF & 0\\
010877024-01 & 010934755-pri & 1:1 & 382.1 & 96 & 0 & 14.40 & -0.89 & 1.2923E+04 & Col-Anomaly & 0\\
010879208-01 & 010879213-01 & 2:1 & 7.3 & 1 & 1 & 18.79 & -2.89 & 6.0355E+02 & Direct-PRF & 0\\
010920420-01 & 010861842-pri & 2:1 & 290.1 & 73 & 0 & 14.29 & -1.77 & 1.6490E+04 & Col-Anomaly & 0\\
010920420-02 & 010861842-pri & 2:1 & 290.1 & 73 & 0 & 14.29 & -1.77 & 1.6490E+04 & Col-Anomaly & 0\\
010924340-01 & 010924462-pri & 2:1 & 182.0 & 46 & -1 & 13.40 & 0.54 & 6.8800E+03 & Col-Anomaly & 0\\
010924340-02 & 010924462-pri & 2:1 & 182.0 & 46 & -1 & 13.40 & 0.54 & 9.2973E+03 & Col-Anomaly & 0\\
010924400-01 & 010924340-01 & 1:1 & 86.7 & -22 & 1 & 13.94 & -1.64 & 2.6316E+00 & Direct-PRF & 1\\
010924400-02 & 4326.01 & 1:1 & 86.7 & -22 & 1 & 13.94 & -1.64 & 9.8000E+00 & Direct-PRF & 1\\
010924437-01 & 010924462-pri & 2:1 & 24.5 & -2 & 5 & 13.40 & 1.07 & 1.0750E+04 & Direct-PRF & 0\\
010925113-01 & 010925104-01 & 1:1 & 6.2 & -1 & -1 & 13.74 & 1.27 & 5.6932E+00 & Direct-PRF & 0\\
010931512-01 & 010931507-01 & 1:1 & 5.0 & 2 & 0 & 13.78 & -0.56 & 3.0278E+00 & Direct-PRF & 0\\
010960993-01 & 3564.01 & 1:1 & 4.8 & -1 & 0 & 14.50 & -3.10 & 2.5636E+01 & Direct-PRF & 0\\
010972902-02 & 010858720-sec & 1:1 & 1112.4 & -280 & 1 & 10.97 & 3.79 & 2.4205E+04 & Col-Anomaly & 0\\
010972902-03 & 010858720-pri & 1:1 & 1112.4 & -280 & 1 & 10.97 & 3.79 & 1.7104E+04 & Col-Anomaly & 0\\
010989166-02 & 009851142-pri & 43:1 & 7066.1 & 5 & 3 & 7.63 & 6.52 & 1.5133E+02 & Cross-Talk & 0\\
010992011-01 & 7398.01 & 1:1 & 20.3 & -4 & 1 & 10.28 & 4.37 & 5.4512E+01 & Direct-PRF & 0\\
010992011-02 & 010991989-sec & 1:1 & 20.3 & -4 & 1 & 10.28 & 4.37 & 5.6818E+01 & Direct-PRF & 0\\
011044770-01 & 3327.01 & 1:1 & 11.0 & 2 & 0 & 15.47 & -2.09 & 1.2108E+02 & Direct-PRF & 0\\
011044770-02 & 011044779-02 & 1:1 & 11.0 & 2 & 0 & 15.47 & -2.09 & 1.1293E+02 & Direct-PRF & 0\\
011046870-01 & 1418.01 & 1:1 & 10.2 & 2 & 1 & 15.73 & -0.67 & 4.4955E+01 & Direct-PRF & 0\\
011076276-01 & 7407.01 & 1:1 & 28.5 & -6 & 5 & 14.21 & 0.91 & 3.2563E+03 & Direct-PRF & 0\\
011098004-02 & 011098013-01 & 1:1 & 6.9 & 1 & 0 & 11.12 & 0.75 & 3.0600E+00 & Direct-PRF & 0\\
011137065-01 & 1157.01 & 1:1 & 5504.5 & 682 & 13 & 13.96 & 0.85 & 2.7378E+01 & Col-Anomaly & 1\\
011154093-01 & 011154110-pri & 1:1 & 12.6 & 2 & -2 & 13.37 & 2.05 & 1.3511E+02 & Direct-PRF & 0\\
011154102-01 & 011154110-pri & 1:1 & 8.6 & 3 & 0 & 13.37 & -0.42 & 7.4413E+01 & Direct-PRF & 0\\
011200415-01 & 3724.01 & 1:1 & 7.6 & 1 & -1 & 16.80 & -4.75 & 3.6915E+02 & Direct-PRF & 0\\
011200767-01 & 011200773-01 & 1:1 & 6.3 & -2 & 1 & 13.67 & -0.30 & 2.3453E+01 & Direct-PRF & 0\\
011200767-02 & 011200773-02 & 2:1 & 6.3 & -2 & 1 & 13.67 & -0.30 & 2.1412E+01 & Direct-PRF & 0\\
011200773-02 & 3667.01 & 1:2 & 6.3 & 2 & -1 & 13.37 & 0.30 & 1.2565E+00 & Direct-PRF & 0\\
011243547-01 & 011401845-pri & 1:1 & 1079.4 & 271 & 1 & 14.36 & 0.40 & 6.2182E+03 & Col-Anomaly & 0\\
011251058-01 & 7428.01 & 1:1 & 226.8 & 57 & 1 & 13.39 & -0.21 & 5.2323E+03 & Col-Anomaly & 0\\
011303815-01 & 3744.01 & 1:1 & 10.0 & 1 & 2 & 15.77 & -0.50 & 8.1290E+01 & Direct-PRF & 0\\
011341164-01 & 004756776-05 & 1:6 & 39157.3 & -136 & -359 & 11.29 & 1.08 & 2.2105E+00 & Reflection & 1\\
011341314-01 & 011235323-02 & 1:1 & 866.0 & 218 & 0 & 13.49 & -0.69 & 4.8395E+02 & Col-Anomaly & 0\\
011401822-01 & 011401845-pri & 1:1 & 25.7 & -3 & 6 & 14.36 & 1.63 & 2.1714E+03 & Direct-PRF & 0\\
011401869-01 & 011401845-pri & 1:1 & 30.3 & 5 & -5 & 14.36 & 1.18 & 6.7279E+03 & Direct-PRF & 0\\
011455491-01 & 011455484-pri & 1:1 & 6.9 & 0 & -2 & 16.15 & -2.70 & 1.0333E+03 & Direct-PRF & 0\\
011455491-02 & 011455484-sec & 1:1 & 6.9 & 0 & -2 & 16.15 & -2.70 & 1.0333E+03 & Direct-PRF & 0\\
011456382-01 & 4845.01 & 1:1 & 21.0 & 0 & 5 & 15.37 & -3.62 & 1.7609E+00 & Direct-PRF & 1\\
011456405-01 & 2771.01 & 1:1 & 21.0 & 0 & -5 & 11.75 & 3.62 & 4.2264E+00 & Direct-PRF & 0\\
011560382-01 & 011560447-pri & 1:1 & 99.0 & -22 & 12 & 10.83 & 4.52 & 3.1361E+03 & Direct-PRF & 0\\
011560397-01 & 011560447-pri & 1:1 & 93.5 & -23 & 6 & 10.83 & 2.87 & 1.1832E+04 & Direct-PRF & 0\\
011560431-03 & 011560447-pri & 1:1 & 43.1 & -11 & 0 & 10.83 & -1.14 & 1.0412E+04 & Direct-PRF & 0\\
011567149-01 & 011618883-sec & 1:1 & 72.8 & -14 & -11 & 13.38 & 0.78 & 9.5842E+03 & Direct-PRF & 0\\
011612241-03 & V850-Cyg-pri & 1:1 & 9254.2 & -1 & -7 & 11.20 & 2.89 & 6.0189E+03 & Cross-Talk & 0\\
011616596-01 & 011616594-pri & 1:2 & 28.4 & 4 & -6 & 11.17 & 1.45 & 5.8236E+03 & Direct-PRF & 0\\
011616631-01 & 011616663-01 & 1:1 & 40.1 & -2 & -10 & 14.97 & 0.88 & 7.9310E-01 & Direct-PRF & 1\\
011616641-01 & 011616594-pri & 1:2 & 77.1 & 2 & 20 & 11.17 & 3.19 & 5.2508E+03 & Direct-PRF & 0\\
011616663-01 & 7463.01 & 1:1 & 40.1 & 2 & 10 & 15.85 & -0.88 & 1.3043E+00 & Direct-PRF & 1\\
011673674-01 & 011673686-pri & 1:1 & 16.5 & 4 & -1 & 11.69 & 1.97 & 7.8625E+00 & Direct-PRF & 0\\
011673674-02 & 011673686-pri & 1:2 & 16.5 & 4 & -1 & 11.69 & 1.97 & 3.5158E+02 & Direct-PRF & 0\\
011673686-02 & 133.01 & 1:2 & 16.5 & -4 & 1 & 13.65 & -1.97 & 4.1867E+00 & Direct-PRF & 0\\
011752908-01 & 011752906-01 & 1:1 & 5.1 & 1 & 1 & 15.25 & 0.30 & 2.3913E+00 & Direct-PRF & 0\\
011763903-01 & 7477.01 & 1:1 & 10.1 & 2 & 2 & 13.72 & 0.40 & 1.7083E+00 & Direct-PRF & 0\\
011774387-01 & 011774383-pri & 1:1 & 5.1 & -1 & 0 & 19.17 & -3.54 & 9.0196E+01 & Direct-PRF & 0\\
011824218-01 & 437.01 & 1:1 & 6.3 & 2 & 0 & 14.50 & -0.77 & 1.3170E+01 & Direct-PRF & 0\\
011855538-01 & 012004679-pri & 1:2 & 1115.0 & 280 & 1 & 13.23 & -1.00 & 1.3040E+04 & Col-Anomaly & 0\\
011858748-01 & 3633.01 & 1:1 & 11.6 & -3 & 0 & 16.48 & -0.97 & 6.6702E+02 & Direct-PRF & 0\\
011872139-01 & 011922782-pri & 1:2 & 609.0 & 153 & 2 & 10.46 & 2.85 & 9.6125E+03 & Col-Anomaly & 0\\
011873171-01 & 011873166-pri & 1:2 & 26.1 & -4 & -4 & 13.47 & 2.12 & 1.8844E+03 & Direct-PRF & 0\\
011911580-01 & 003644542-sec & 3:1 & 41461.2 & -18 & 44 & 8.35 & 5.55 & 2.5221E+02 & Reflection & 0\\
011911580-02 & 3511.01 & 3:1 & 41461.2 & -18 & 44 & 8.35 & 5.55 & 3.0234E+02 & Reflection & 0\\
011912911-01 & 011913071-pri & 1:1 & 255.6 & 54 & 35 & 9.53 & 5.99 & 1.2857E+03 & Direct-PRF & 0\\
011912916-01 & 011913071-pri & 1:1 & 236.0 & 44 & 39 & 9.53 & 6.29 & 7.4704E+02 & Direct-PRF & 0\\
011912932-01 & 011913071-pri & 1:1 & 209.5 & 37 & 37 & 9.53 & 4.79 & 2.1000E+03 & Direct-PRF & 0\\
011912941-01 & 011913071-pri & 1:1 & 189.7 & 28 & 38 & 9.53 & 5.60 & 1.6017E+03 & Direct-PRF & 0\\
011912987-01 & 011913071-pri & 1:1 & 122.5 & 17 & 26 & 9.53 & 4.04 & 2.1236E+03 & Direct-PRF & 0\\
011913012-01 & 011913071-pri & 1:1 & 90.4 & 15 & 17 & 9.53 & 5.23 & 4.6782E+02 & Direct-PRF & 0\\
011913012-02 & 011913071-sec & 1:1 & 90.4 & 15 & 17 & 9.53 & 5.23 & 6.5775E+02 & Direct-PRF & 0\\
011913013-01 & 011913071-pri & 1:1 & 91.7 & 17 & 15 & 9.53 & 7.91 & 3.7967E+01 & Direct-PRF & 0\\
011913013-02 & 011913071-sec & 1:1 & 91.7 & 17 & 15 & 9.53 & 7.91 & 6.1046E+01 & Direct-PRF & 0\\
011913052-01 & 011913071-pri & 1:1 & 103.7 & 25 & -5 & 9.53 & 4.31 & 1.3404E+03 & Direct-PRF & 0\\
011913072-01 & 011913071-pri & 1:1 & 102.6 & -22 & 14 & 9.53 & 4.88 & 2.5890E+03 & Direct-PRF & 0\\
011913073-01 & 011913071-pri & 1:1 & 34.9 & 7 & -5 & 9.53 & 3.96 & 3.9293E+02 & Direct-PRF & 0\\
011913073-02 & 011913071-sec & 1:1 & 34.9 & 7 & -5 & 9.53 & 3.96 & 5.4941E+02 & Direct-PRF & 0\\
011922648-01 & 7495.01 & 1:1 & 158.8 & 40 & 3 & 10.46 & 4.07 & 3.3753E+03 & Direct-PRF & 0\\
011922678-01 & 011922782-pri & 1:2 & 106.3 & 20 & -18 & 10.46 & 3.05 & 4.3528E+03 & Direct-PRF & 0\\
011922722-01 & 011922782-pri & 1:2 & 76.8 & 5 & -18 & 10.46 & 3.30 & 2.6216E+03 & Direct-PRF & 0\\
011923074-01 & 011922782-pri & 1:2 & 351.0 & -88 & 0 & 10.46 & 4.26 & 3.7820E+03 & Direct-PRF & 0\\
011968514-01 & 3587.01 & 1:1 & 8.4 & 1 & -2 & 14.44 & -2.99 & 8.5665E+02 & Direct-PRF & 0\\
012004656-01 & 012004679-pri & 1:2 & 38.5 & -7 & 7 & 13.23 & 2.29 & 3.3807E+03 & Direct-PRF & 0\\
012004680-01 & 012004679-pri & 1:2 & 38.7 & 8 & 5 & 13.23 & 2.07 & 4.4745E+03 & Direct-PRF & 0\\
012023078-01 & 012023089-pri & 1:1 & 9.8 & 1 & -2 & 15.63 & -2.98 & 3.4762E+02 & Direct-PRF & 0\\
012062667-01 & 3746.01 & 1:1 & 6.8 & 1 & -2 & 17.38 & -4.71 & 5.8005E+02 & Direct-PRF & 0\\
012066583-01 & 012066629-01 & 1:1 & 49.5 & -9 & -9 & 15.07 & -1.55 & 3.2222E+00 & Direct-PRF & 1\\
012066629-01 & 012066583-01 & 1:1 & 49.5 & 9 & 9 & 13.52 & 1.55 & 3.1034E-01 & Direct-PRF & 1\\
012071037-01 & 7511.01 & 1:1 & 30.7 & -6 & 6 & 13.53 & 0.57 & 7.3335E+03 & Direct-PRF & 0\\
012106929-01 & 3895.01 & 1:1 & 12.0 & -1 & -2 & 18.36 & -4.56 & 1.2763E+02 & Direct-PRF & 0\\
012106929-02 & 012106934-02 & 1:1 & 12.0 & -1 & -2 & 18.36 & -4.56 & 4.6969E+01 & Direct-PRF & 0\\
012107008-01 & 359.01 & 1:1 & 96.7 & -21 & 12 & 13.80 & 0.90 & 4.0000E+00 & Direct-PRF & 1\\
012107021-01 & 3895.01 & 1:1 & 121.0 & 2 & 31 & 18.36 & -5.34 & 2.3723E+02 & Direct-PRF & 1\\
012108293-01 & 012108333-pri & 1:1 & 50.3 & -1 & 13 & 13.23 & 1.61 & 5.9288E+03 & Direct-PRF & 0\\
012108312-01 & 012108333-pri & 1:1 & 21.4 & -1 & 5 & 13.23 & 1.12 & 4.0207E+03 & Direct-PRF & 0\\
012108364-01 & 012108333-pri & 1:1 & 52.4 & -1 & -13 & 13.23 & 2.60 & 3.8022E+03 & Direct-PRF & 0\\
012109421-01 & 7514.01 & 1:1 & 76.8 & -5 & 18 & 13.77 & -0.31 & 4.6786E+01 & Direct-PRF & 1\\
012157971-01 & 012157987-pri & 1:1 & 26.5 & -1 & 7 & 12.21 & 1.45 & 3.9558E+03 & Direct-PRF & 0\\
012157983-01 & 012157987-pri & 1:1 & 25.1 & 6 & -1 & 12.21 & 1.56 & 3.6088E+03 & Direct-PRF & 0\\
012164770-01 & 012164751-01 & 1:1 & 20.6 & 5 & 1 & 14.19 & 0.46 & 2.1786E+03 & Direct-PRF & 0\\
012257851-01 & 012257908-pri & 1:2 & 99.2 & -2 & 25 & 10.43 & 4.94 & 3.0977E+03 & Direct-PRF & 0\\
012257886-01 & 012257908-pri & 1:1 & 53.4 & -4 & 12 & 10.43 & 4.75 & 1.1788E+03 & Direct-PRF & 0\\
012316431-01 & 3575.01 & 1:1 & 14.4 & 4 & 0 & 16.11 & -1.94 & 2.9519E+02 & Direct-PRF & 0\\
012316431-02 & 012316447-02 & 1:1 & 14.4 & 4 & 0 & 16.11 & -1.94 & 2.2965E+02 & Direct-PRF & 0\\
012353633-01 & 012554536-pri & 1:1 & 1587.3 & 399 & 0 & 12.82 & 0.36 & 2.0919E+04 & Col-Anomaly & 0\\
012418891-01 & 7533.01 & 1:1 & 73.4 & -11 & 15 & 12.40 & 3.45 & 3.0507E+03 & Direct-PRF & 0\\
012459808-01 & 7525.01 & 1:1 & 749.3 & 188 & 0 & 13.53 & -0.99 & 3.4224E+03 & Col-Anomaly & 0\\
012506342-01 & 012506351-pri & 1:2 & 15.9 & 0 & 4 & 13.18 & 2.53 & 2.0500E+02 & Direct-PRF & 0\\
012554510-01 & 012554536-pri & 1:1 & 45.3 & -6 & 9 & 12.82 & 0.84 & 2.7892E+04 & Direct-PRF & 0\\
012643589-01 & 3626.01 & 1:1 & 7.5 & -1 & 2 & 16.44 & -2.69 & 6.5671E+01 & Direct-PRF & 0\\
012644774-01 & 1611.01 & 1:1 & 16.1 & -3 & -3 & 11.76 & 3.14 & 1.2362E+02 & Direct-PRF & 0\\
012644774-02 & 012644769-sec & 9:1 & 16.1 & -3 & -3 & 11.76 & 3.14 & 1.3407E+01 & Direct-PRF & 0\\


==> hzCandidates.tex <==
We take a closer look at some of the HZ candidates. All of those in this list have a 1 sigma error bar that places them below 1.8 Rearth and less than 2.0 Searth according to the MCMC fits, has an relative error in Rp less than 33 per cent and has a score cut larger than 0.6.

\paragraph K08279.01 on \opstce\,009011955-01 
This TCE is dispositioned as PC with a score of 0.7 but when inspected manually, it is clearly caused by Rolling band. The fit gives a radius of 5.22, but it has large uncertainties which give it some possibility of being terrestrial. However this is clearly an FP. 

\paragraph K08174.01 on \opstce\,008873873-01
This candidate is new to DR25 and has five transits, three of which show a significant reduction in flux. It is measured to have a radii smaller than the Earth's and receives slightly less insolation flux than the Earth. It is around a 5300\,K star. It has low MES. It likely has an anomolously small radius.

\paragraph K08007.01 on \opstce\,010403228-03
This candidate is new to DR25 and has a score of 0.802. There are only five quarters of observations for this star (Q8 and Q14--Q17), so this 67\,d period TCE only has 4 transits. None of these transits show a clear signal, so this is a marginal PC.

\paragraph K08000.01 on \opstce\,010331279-01
This candidate is new to DR25 and has five transits that do not lie in data gaps (score=0.974). It has a period of 225\,d and a MES of 8.7. It circles a star that is 5663. It's planet radii ranges from 1.52 to 2.07 Rearth. 

\paragraph K07923.01 on \opstce\,009084569-02
This candidate is new to DR25 and has 5 transits. Only one or two of these transits truly look transit-shaped. Marshall only preferred a transit shape for one, but not with enough significance to actually throw away most of those transits. Likely this is an FP.

\paragraph K07894.01 on \opstce\,008555967-01
This candidate is new to DR25 and has four transits. The Q5 transit looks more like a step-up than a transit, though Marshall preferred the sigmoid-box model for that transit. It has a MES of 8.5 and a period of 347.976\,days. Our MCMC model gives this a radius of 1.79 (-0.15 +0.49) and an insolation flux of 0.97 (-0.27, +0.87), i.e. likely a super-Earth with an insolation flux similar to the Earth's.

\paragraph K07749.01 on \opstce\,005888187-01
This candidate is new to DR25 and has 10 transits. It has a MES of 8.2 and a period of 133\,d. While it is a low signal to noise candidate, there is not reason to question it. It would have a radius of 1.89 and insolation flux of 2.38 around a 5202\,K star (Between and K and G dwarf)

\paragraph K07711.01 on \opstce\,004940203-01
This candidate is new to DR25 and has four transits. Each transit has no issues and three were passed cleanly by Marshall.  This planet candidate is in a 302\,d orbit with a MES of 8.4 and score of 0.99.  It  lies around a 5734\,K star and has an insolation flux of 0.87 (-.22,+0.66). The radii is 1.47 (-.12, +0.34).

\paragraph K07706.01 on \opstce\,004940203-01
This candidate is new to DR25 and has 23 good transits.  The star shows large flux variations likely due to spots, but the transit duration is significantly shorter than these spot variations and so likely the detrending is creating the signal. It has a period of 42.0495\,d and MES of 7.4 with a score of 0.84. It circles a 4281\,K star. It's radius s 1.63 (-.16, +0.08) with an insolation flux of 2.0 (-0.68 +0.55).


This is the list of new Candidates with score values less than 0.6.  These have a lower reliability (~40 per cent)

\paragraph K08290.01 on \opstce\,010459805-01
This FP has a score of 0.113. Two of its four transits are possible SPSDs (Q0 and Q7) and the remaining signal is not enough to convince one there is a transit here.

\paragraph K08278.01 on \opstce\,008873674-01
This is dispositioned as an FP with a score of 0.448. This fails because Marshall removes two of the transits (Q6 and Q15) because they are more consistent with no transit. This causes the calculated MES to drop a bit below 7.1. Given that it has 7 observed transits, by manual inspection it would be a marginal candidate. If so it has a radius of 1.82 and an insolation flux of 1.95 which places it as a potential super Earth in the habitable zone of this G type star.

\paragraph K08272.01 on \opstce\,008022520-01
This candidate has a score of 0.117 meaning that several metrics were on the verge of failing it. It has three transits of which one is truly transit shaped in the DV detrending, the alternate detrending looks pretty good.

\paragraph K08259.01 on \opstce\,010459805-01
This PC with a score of 0.33 has four transits. Q8 is has most of the signal and is associated with noise in the sky causing the transit to be quite noisy. The other three events are not convincing. This is likely an FP.

\paragraph K08253.01 on \opstce\,005098334-01
This PC has a score of 0.07. It has three transits, but none really look like transits. This is likely an FP.

\paragraph K08246.01 on \opstce\,004446859-01
This PC with a score of 0.223 has four transits on a pretty clean light curve. Other than the low score there is no reason to fail this candidate. The candidate orbits a 6067\,K G-type star at a 425\,d period orbit. It is 1.61 (-0.37, +0.45) radius and the insolation flux is 1.48.

\paragraph K08242.01 on \opstce\,003629119-01
This PC with a score of 0.184 is very low signal-to-noise but otherwise has no reason to fail it.  It has a radius of 1.82 and an insolation flux of 0.78. This is an FP.

\paragraph K08227.01 on \opstce\,011558217-01
This FP has a score of 0.221. This correctly fails because the events are different in shape and depth.

\paragraph K08085.01 on \opstce\,002284957-01
This PC has a score 0.421. From manual inspection it is clear that two of the transit events are actually SPSDs. The other two transit events are identified correctly by Marshall to be better fit by an offset only. This is likely an FP.

\paragraph K08077.01 on \opstce\,012266099-01
This PC has a score of 0.341. This is a marginal, low snr PC. At 4840\,K and 1.9 radii and 2.7 insolation flux, but the large error bars cause it to have some possibility of being in the HZ.

\paragraph K08048.01 on \opstce\,012266099-01
This PC has a score of 0.332. It is a marginal, low snr PC, but otherwise fine. It has a radii of 1.52 and insolation flux of 0.88 around a cool F-dwarf star (6156\,K)

\paragraph K07992.01 on \opstce\,010214341-01
This PC has a score of 0.124 with four transits. The transit in Q13 is associated with a sky flare and Q7, which contains most of the remaining flux, is not transit shaped. This is likely an FP. 

\paragraph K07953.01 on \opstce\,009650579-01
This PC has a score of 0.339 and three transits. None of the transits are very convincing, likely this is an FP.

\paragraph K07932.01 on \opstce\,009278575-01
This PC has a score of 0.229 and three transits. None of the transits are very convincing, like this is an FP. The strongest transit in Q12 is associated with noisy data points and a discontinuity in the sky time series.

\paragraph K07938.01 on \opstce\,009469494-01
This PC has a score of 0.510. It has an extremely large error bar in insolation flux that yields some possibility that it could lie in the habitable zone. A manual inspection shows that this is a highly variable star and the transits artifacts of less than optimal detrending. Likely this is an FP.

\paragraph K07930.01 on \opstce\,009210820-01
This PC has a score of 0.469 and is a low signal-to-noise transit with only 3 transits. Manual inspection yields no reason to doubt this candidate. Its radius is 50 percent larger than the earth's and circles a 5031\,K K-dwarf at a period similar to the Earth's causing it have an insolation flux similar to Mars.

\paragrph K07882.01 on \opstce\,008364232-01
This PC has a score of 0.552 and circles a star that is 4348\,K, a mid K-dwarf with a period of 65\,d. It has a MES of 7.2, making it very low signal to noise and thus marginally passes the Robovetter.  Manual inspection reveals that there is no reason to doubt this signal.

\paragraph K07798.01 on \opstce\,006952971-01
This PC has a score of 0.474. It is dominated by what looks like noise or a discontinuity in Q16 and the TCE is likely an FP.

\paragraph K07723.01 on \opstce\,005276332-01
This PC has a score of 0.262. It has four transits, one which was thrown out as a step-up by Marshall (Q10) and one that is on the edge of a gap (Q2). Likely this is an FP.

\paragraph K07716.01 on \opstce\,005097856-01
This PC has a score of 0.234. This is an extremely marginal PC but there is not obvious reason to fail it.  It is a 1.52 radius planet with an insolation flux of 0.39 around at 5700\,K G-dwarf star. The orbital period is 483\,d.

\paragraph K02853.02 on \opstce\,010387742-02
This FP has a score of 0.217 with 5 transit events.  One is a likely SPSD (Q5). Marshall flags Q11 and Q14 as offset only. Likely this is an FP.

These are not new to DR25.

\paragraph K07223.01 on \opstce\,009674320-01 
This candidate is was found first in the DR24 catalog and has 5 transits, 3 of which passed the Robovetter's metrics. It has a period of 317.091\,d and mes of 10.3247 and a score of 0.947. The 1.65 radii (-0.12 +0.27) planet circles a 5366\,K star with an insolation flux of 0.54 (-0.13 +0.29), making the planet a bit cooler than the Earth.



==> lpp.tex <==
%% Text describing LPP and how it works.

We implemented the LPP transit-like metric described by \citet{Thompson2015b} to separate those TCEs that show a transit-like shape from those that do not. This technique bins the folded light curve and then uses a machine learning technique that uses a dimensionality reduction algorithm called Locality Preserving Projections (LPP) to group transits of a similar shape.  In attempting to find a metric that best separates the known candidates from the false positives, we deviated from the method described \citet{Thompson2015b} in a few key ways.  This retraining was directed at solving the problem that the metric was highly dependent on both period and MES. The threshold that divides the transit-like from the not-transit-like events increases at periods less than $\sim$ 10??\,days. This is caused by the fact these TCEs transit for a large fraction of the orbital period and because transit injection does not include a large number of this type of event.  The trend with MES is difficut to overcome. It is routed in the fact that when the binned light curve has a lower signal to noise, it is less likely for two light curves to be identical to each other, creating more scatter in the final metric.


More specifically we made the following changes when implementing the LPP transit-metric. First, we trained the LPP algorithm using the pixel-level transit injections plus those planet candidates from DR24 that were found as TCEs in DR25.  Transit injection had very few short period injections, which can look distinctly different, even in the highly controlled binned space used by LPP. Since this population defines what a transit-like event looks like, it is important to have a wide variety of known transits, thus we included the DR24 candidates in the training sample.  Second, we changed how the data were binned. To remove some of the MES dependence TCEs with lower MES are given wider bins for those near the transit center. Also, we found that we got better performance by having a total ??97 bins (x for wide and y for central bins) and reducing them to 20?? dimensions with LPP.  Third, we normalized the LPP values by the 75 percentile of the N?? training set TCEs that are closest in period.  In this way we remove the period dependence on the LPP metric.  See Figure~{fig:lpp}.

The matlab code used to calculate this metric is available at the following repository:

